Making Decisions under Outcome Performativity

Decision-makers often act in response to data-driven predictions, with the goal of achieving favorable outcomes. In such settings, predictions don't passively forecast the future; instead, predictions actively shape the distribution of outcomes they are meant to predict. This performative prediction setting raises new challenges for learning "optimal" decision rules. In particular, existing solution concepts do not address the apparent tension between the goals of forecasting outcomes accurately and steering individuals to achieve desirable outcomes. To contend with this concern, we introduce a new optimality concept -- performative omniprediction -- adapted from the supervised (non-performative) learning setting. A performative omnipredictor is a single predictor that simultaneously encodes the optimal decision rule with respect to many possibly-competing objectives. Our main result demonstrates that efficient performative omnipredictors exist, under a natural restriction of performative prediction, which we call outcome performativity. On a technical level, our results follow by carefully generalizing the notion of outcome indistinguishability to the outcome performative setting. From an appropriate notion of Performative OI, we recover many consequences known to hold in the supervised setting, such as omniprediction and universal adaptability.

==> arxiv 2/calibration.tex <==

\section{Connections to Multicalibration}

So far, we have studied how  extensions of  outcome indistinguishability definitions enable the design of omnipredictors for performative settings. 
In the world of supervised learning, \cite{oi} established tight connections between outcome indistinguishability and various notions of multicalibration \cite{hkrr}.
Given the complementary relationship between these two concepts in the supervised world, it is natural to speculate that generalizing multicalibration to the outcome performative setting might be fruitful.
% whether these remain similarly related notions once we go beyond supervised learning.
% And if not, whether a more multicalibration-based perspective on outcome performativity would yield a more efficient approach towards omniprediction.

In this section, we begin to examine these questions and 
discuss analogues of multiaccuracy and multicalibration for the performative setting. 
We start by showing that multiaccuracy naturally, and efficiently, extends to performative contexts, and provides an effective way to achieve performative outcome indistinguishability in a loss-independent fashion. 
Conversely, we illustrate how naive translations of multicalibration to performative prediction result in definitions whose complexity blows up exponentially in the number of predictions $\card{\Ych}$.
We conclude with some discussion of alternatives to calibration-style guarantees that could, in principle, be used to obtain efficient omnipredictors.


\paragraph{On Multiaccuracy.}
\theoremref{thm:omni} shows how $(\cL,\Hcal, \epsilon)$-performative omniprediction arises as a consequence of $(\cL, \Hcal, \epsilon)$-performative OI and $(\cL, \epsilon)$-decision OI, where the OI distinguishers explicitly account for the collection of loss functions $\cL$.
Here, we show an efficient approach for obtaining POI for the class of all bounded input-oblivious loss functions.

We say that a loss function is \emph{input-oblivious} if it only depends on the input $x \in \Xcal$ via the decision $h(x)$. That is, for all $x$ and $x'$ and pairs $(\yhat, y)$, $\ell(x,\yhat, y) = \ell(x', \yhat,y)$. Equivalently, these functions have domain $\cYh \times \cY$ instead of $\cX\times \cYh \times \cY$.
We use 
\begin{align*}
\mathcal{L}_\mathrm{io} = \set{\ell:\Ych \times \set{0,1} \to [0,1]}
\end{align*} 
to denote the class of all bounded input-oblivious loss functions.
Our first result for this section proves that a performative analogue of multiaccuracy \cite{hkrr,kim2019multiaccuracy}  implies POI for $\cL_\mathrm{io}$.
%Originally introduced as a basic notion of multi-group fairness in the supervised setting, the idea of multiaccuracy naturally extends to the performative setting.
\begin{definition}[Multiaccuracy]
For a distribution $\D$, hypothesis class $\Hcal$, and $\eps \ge 0$,
a predictor $\pt:\Xcal \times \Ych \to [0,1]$ is $(\Hcal,\eps)$-multiaccurate under outcome performativity over $\D$ if for all $h \in \Hcal$ and $\yhat \in \Ych$
\begin{gather*}
    \big|\E_{\substack{x \sim \calD \\ \ys \sim \ps(x,\yhat)}} [\ys \cdot \1\{h(x) = \yhat\}] - \E_{\substack{x \sim \calD \\ \yt \sim \pt(x,\yhat)}}[\yt \cdot \1\{h(x) = \yhat\}] \big|
  \leq \eps.
\end{gather*}
\end{definition}
Here, we require that the expectation of our modeled outcome $\yt \sim \pt(x,h(x))$ is accurate after deploying each $h \in \Hcal$, even when restricting our attention to the individuals $x \in \Xcal$ such that $h(x) = \yhat$.
While seemingly simpler than performative OI, we show that multiaccuracy in fact implies performative OI for all input-oblivious losses.
\begin{lemma}
\label{lem:MA2POI}
If $\pt:\Xcal \times \Ych \to [0,1]$ is $(\Hcal,\eps)$-multiaccurate, then $\pt$ is $(\cL_\mathrm{io},\Hcal,2\eps)$-performative OI.
\end{lemma}
\begin{proof}
The proof shows an approximate equality between the loss $\ell \in \mathcal{L}_\mathrm{io}$ of any $h \in \Hcal$ under $\yt \sim \pt(x,h(x))$ and $\ys \sim \ps(x,h(x))$. For $\cY = \{0,1\}$,
\begin{align*}
\E_{\substack{x \sim \calD \\ \yt \sim \pt(x,\yhat)}}[\ell(h(x),\yt)]
&= \sum_{\yhat \in \Ych} \Pr_{\cD}[h(x) = \yhat] \cdot \E_{\substack{x \sim \calD \\ \yt \sim \pt(x,\yhat)}}[\ell(\yhat,\yt) ~\vert~ h(x) = \yhat]\\
&= \sum_{\yhat \in \Ych} \Pr_{\cD}[h(x) = \yhat] \cdot \E_{\substack{x \sim \calD \\ \yt \sim \pt(x,\yhat)}}\left[\yt \cdot \ell(\yhat,1) + (1-\yt) \cdot \ell(\yhat,0) ~\vert~ h(x) = \yhat\right]\\
&\leq \sum_{\yhat \in \Ych} \Pr_{\cD}[h(x) = \yhat] \cdot \E_{\substack{x \sim \calD \\ \ys \sim \ps(x,\yhat)}}\left[\ys \cdot \ell(\yhat,1) + (1-\ys) \cdot \ell(\yhat,0) ~\vert~ h(x) = \yhat\right] + 2 \eps\\
&= \sum_{\yhat \in \Ych} \Pr_{\cD}[h(x) = \yhat] \cdot \E_{\substack{x \sim \calD \\ \ys \sim \ps(x,\yhat)}}[\ell(\yhat,\ys) ~\vert~ h(x) = \yhat] + 2 \eps\\
&=\E_{\substack{x \sim \calD \\ \ys \sim \ps(x,\yhat)}} [\ell(h(x),\ys)] + 2 \eps.
\end{align*}
The the third line follows under the assumption that $\pt$ is $(\Hcal,\eps)$-multiaccurate and the bound on the magnitude of $\card{\ell(\yhat,b)} \le 1$ for all $\yhat \in \Ych$ and $b \in \set{0,1}$. Given that an identical argument can be used to show the opposite inequality, we conclude that $\pt$ is indeed POI.
\end{proof}
Inspecting the performative multiaccuracy condition, we can see that it is similarly possible to reduce the problem of auditing for multiaccuracy to supervised learning.
This auditing procedure can be viewed as a special case of the auditing step from Section~\ref{sec:learning} or as a generalization of previous auditing procedures from work on multiaccuracy in the supervised learning setting \cite{hkrr,kim2019multiaccuracy}. In more detail, the relevant auditing problem for performative multiaccuracy is to determine whether there exists an $h \in \cH$ and $\yhat \in \cYh$ such that
\begin{gather*}
         \big|\E_{\substack{x\sim \cD \\ \ys \sim \ps(x,\yhat)}}[(\ys - \pt(x,\yhat)) \cdot \1\{h(x) = \yhat\}] \big|> \eps.
\end{gather*}
As before, this auditing step reduces to a cost-sensitive classification problem (\definitionref{definition:csc}). Auditing over a hypothesis class $\cH$ can be done with $2|\cYh|$ many calls to a cost-sensitive learner $\cscalg$ with tolerance parameter $\cO(\eps)$. We omit a formal statement of this result since it follows the exact pattern from \propref{prop:csc_auditing}.


In other words, in order to achieve $(\cL,\Hcal,O(\eps))$-POI for any class of input-oblivious losses $\cL \subseteq \cL_\mathrm{io}$, it suffices to audit for and enforce $(\Hcal,\eps)$-multiaccuracy.
In this sense, for input-oblivious losses, there is a single auditing procedure that works for all losses, so we can replace $\card{\cL}$-factors by $|\cYh|$ factors in the auditing complexity for performative OI. 
%\jcpnote{maybe we should include a formal statement?}



\paragraph{On Multicalibration.}
\label{sec:calibration}

Going beyond multiaccuracy, the original work of \cite{omni} established omniprediction in the supervised setting as a consequence of multicalibration.
As such, we might wonder whether there exists an analogous notion of multicalibration for performative prediction that enables a similar result.
Defining an efficient notion of calibration under performativity (let alone, multicalibration), turns out to be a subtle task.

In supervised learning, calibration requires that the expectation of $\pt$ is accurate, even when we partition the inputs $x \in \Xcal$ based on the predicted value $\pt(x) = v$.
Specifically, the constraints quantify over each supported $v \in \supp(\pt)$:
\begin{gather*}
    \E_{\substack{x \sim \D\\\ys \sim \ps(x)}}[\ys \cdot \1\{\pt(x) = v\}] \approx \E_{\substack{x \sim \D\\\yt \sim \pt(x)}}[\yt \cdot \1\{\pt(x) = v\}] = v \cdot \Pr[\pt(x) = v].
\end{gather*}
Such calibration-style constraints suffice to establish omniprediction because for any loss $\ell$, the optimal decision $\ft_\ell(x)$ is completely determined by $\pt(x)$.

In performative prediction, quantifying over the supported values of $\pt$ requires considering the decisions $\yhat \in \Ych$ as well.
In particular, the optimal decision $\ft_\ell(x)$ is a function of the vector of predictions $\tilde{q}(x) \in [0,1]^{\card{\Ych}}$, which gives the predicted probability $\yt \sim \pt(x,\yhat)$ for each $\yhat \in \Ych$ (recall the $q(\cdot)$ notation from \propref{prop:iteration_bound}).
Thus, using the naive translation of the calibration constraints for omniprediction, we must partition $\Xcal$ based on the vector-valued predictions,
$\tilde{q}(x) = \overrightarrow{v}$.
The cardinality of this calibration partition of $\Xcal$ scales exponentially in the number of decisions $\card{\Ych}$, even for binary outcomes $\cY$.

Still, we may consider more efficient calibration-style conditions that suffice to imply omniprediction in the performative setting.
Rather than aiming for full performative calibration, we focus on adapting the notion of decision calibration \cite{zhao2021calibrating} to the performative setting.
Decision calibration was introduced to avoid  exponential blow-up in the calibration constraints due to multi-class prediction.
We show that the notion can equally be adapted to the performative setting to deal with blow-up due to many actions $\yhat \in \Ych$.
We define decision calibration with respect to the class of input-oblivious losses.
\begin{definition}[Decision Calibration]
For a distribution $\D$ and $\eps \ge 0$,
a predictor $\pt:\Xcal \times \Ych \to [0,1]$ is $\eps$-decision calibrated under outcome performativity over $\D$ if for every loss $\ell \in \cL_\mathrm{io}$, and for all $\yhat \in \Ych$,
\begin{gather*}
   \big| \E_{\substack{x \sim \D\\\ys \sim \ps(x,\ft_\ell(x))}}[\ys \cdot \1\{\ft_\ell(x) = \yhat\}] - \E_{\substack{x \sim \D\\\yt \sim \pt(x,\ft_\ell(x))}}[\yt \cdot \1\{\ft_\ell(x) = \yhat\}] \big| \leq \eps.
\end{gather*}
\end{definition}
With this definition in place, the proof of Lemma~\ref{lem:MA2POI} can be adapted to show that decision calibration suffices to establish performative decision OI.
\begin{lemma}
\label{lem:DC2DOI}
If $\pt:\Xcal \times \Ych \to [0,1]$ is $\eps$-performative decision calibrated, then $\pt$ is $(\cL_\mathrm{io},2\eps)$-performative decision OI.
\end{lemma}
As an immediate corollary of ~\theoremref{thm:omni} and Lemmas~\ref{lem:MA2POI} \& \ref{lem:DC2DOI}, we obtain sufficient conditions for omniprediction with respect to all bounded input-oblivious losses.
\begin{corollary}
Suppose $\pt:\Xcal \times \Ych \to [0,1]$ is $(\Hcal,\eps)$-multiaccurate and $\eps$-decision calibrated under outcome performativity.
Then, $\pt$ is a $(\cL_\mathrm{io},\Hcal,4\eps)$-performative omnipredictor.
\end{corollary}
In other words, if we can obtain multiaccuracy and decision calibration under performativity, then we have a direct pathway to obtain omniprediction for all bounded, input-oblivious losses.

\paragraph{On Decision Calibration.}
Note, however, that unlike the case of multiaccuracy, the decision rules that arise in the decision calibration condition are loss-dependent.
That is, the optimal decision rules $\ft_\ell$ depend on $\ell \in \cL_\mathrm{io}$.
%In this sense, decision calibration strengthens the requirements compared to $\cL$-decision OI for $\cL \subseteq \cL_\mathrm{io}$.

Motivated by the strong guarantee, we consider the feasibility of auditing for decision calibration.
Note that for any $\ell \in \cL_\mathrm{io}$, the loss is defined by the loss for each outcome $y \in \set{0,1}$ and decision $\yhat \in \Ych$.
Thus, to audit decision calibration over all input-oblivious losses, it suffices to audit whether there exist a $\yhat \in \Ych$ and $w_{a,0},w_{a,1} \in [-1,1]$ such that:
\begin{gather*}
    \big|\E_x[\left(\pt(x,\yhat) - \ys\right) \cdot \1\{\argmin_{a \in \Ych}\set{ w_{a,1} \cdot \pt(x,a) + w_{a,0} \cdot (1-\pt(x,a))} = \yhat\}] \big| > \eps
\end{gather*}
where the weights $w_{a,0}$ and $w_{a,1} \in [-1,1]$ represent the choice of $\ell(a,0)$ and $\ell(a,1)$ corresponding to the choice of $a \in \Ych$.
% \jcpnote{do you mind taking a pass on this last paragraph part and saying something that this is more speculative?}

Naively, searching for such a violated loss might require time exponential in $\card{\Ych}$.
For instance, by explicitly enumerating over some appropriately-fine net of $[-1,1]^{2\card{\Ych}}$, then we can simply consider ``every'' possible loss.
Improving the computational complexity of such a search is an interesting question, which may benefit from the techniques utilized in \cite{zhao2021calibrating}.

Even without an improvement in the runtime complexity of learning, note that once an auditor succeeds, and we have a violated loss function, there is an efficient update to the prediction function.
In particular, we simply need to record the chosen $2 \cdot \card{\Ych}$ parameters $\set{w_{a,0},w_{a,1}}$ and the $\yhat \in \Ych$, then execute the update from POI-Boost.
In all, we can conclude that performative omnipredictors for $\cL_\mathrm{io}$ exist in complexity independent of the complexity of $\cL_\mathrm{io}$.
\begin{corollary}
Suppose $\Hcal$ is a hypothesis class with size-$s$ circuits.
Then, for any $\eps > 0$, there exist an $(\cL_\mathrm{io},\Hcal,\eps)$-performative omnipredictor implemented by a circuit of size  $\poly(s, \card{\Ych})/\eps^2$.
\end{corollary}
% \mpk{Does this look right?  I guess it's not that impressive, as already the size didn't depend on $\card{\cL}$.}
This preliminary analysis leaves open the possibility of learning performative omnipredictors via techniques that are independent of the loss class, as in the original work on $(\cL_\mathrm{cvx},\Hcal)$-omniprediction from $\Hcal$-multicalibration.
We leave a more thorough investigation of these ideas to future work.


% \mpk{Implementing the search is an interesting problem.  Naively, also exponential in $\card{\Ych}$, e.g., by explicitly enumerating over some net of $[-1,1]^\card{\Ych}$.
% But, in terms of the complexity of the resulting predictor, we only have to encode the weights $w_{a,0},w_{a,1}$ and $\yhat$.
% So, complexity scales as $\card{\Ych}$.
% }

% Thus, for binary outcomes, the auditing problem only requires solving a maximization problem over three parameters (one discrete choice of $\yhat \in \Ych$, and two choice of weights $w_0,w_1 \in [-1,1]$).
% Thus, given access to appropriate numerical search methods, we can audit for decision calibration.
% For instance, one naive strategy would take an appropriate net over $[-1,1]^2$, then explicitly enumerating over the choice of $w_0,w_1$.
% Given a fixed $w_0,w_1$, estimating the miscalibration 




% \paragraph{Decision OI and Calibration.}
% \mpk{
% Note:  decision calibration is equivalent to the following technical condition.

% Does there exist a $\yhat \in \Ych, w_0,w_1 \in [-1,1]$ such that:
% \begin{gather*}
%     \E_x[\pt(x,\yhat) - \ps(x,\yhat) ~\vert~ \argmin_{a \in \Ych}\set{ w_1 \cdot \pt(x,a) + w_0 \cdot (1-\pt(x,a))} = \yhat] > \eps
% \end{gather*}
% i.e., does there exist some $\ell \in \cL_1$ and $\yhat \in \Ych$ such that conditioning on the event that $\ft_\ell(x) = \yhat$ maintains accurate expectations of probabilities.

% Note:  this means we can probably run explicit searches over $\poly(1/\eps)$ many choices of $w_0,w_1$, then compute the minimizers, and evaluate the conditional expectations for $\card{\Ych}$ choices of $\yhat$.

% So, auditing is reasonably efficient.  e.g., linear in $\card{\Ych}$, not exponential!
% }



==> arxiv 2/indistinguishability.tex <==


\newpage


\begin{figure}[t]
\setlength{\fboxsep}{2mm}
\begin{boxedminipage}{\textwidth}
\begin{center}
{\centering{\underline{Indistinguishability Boosting}}}
\end{center}

\vspace{2mm}
{\bf Input:} Set of losses $\cL$, hypotheses $\cH$, distribution $\cD$, tolerance $\alpha > 0$\\
\vspace{-2mm}

{\bf Initialize:} $p^{(1)}(x,\yhat) \in \Delta(\cY)$ for all $x$ and $\yhat$ \\

{\bf For:} $t = 1,2, \ldots$
\begin{itemize}
	\item {\bf If:} there exists $\bar{h} \in \cH \cup \{f_{\ell, t}: \ell \in \cL \}$ and $\bar{\ell} \in \cL$ such that
	\begin{align}
	\equationlabel{eq:constraint}
		| \underbrace{\E_{\substack{x \sim \cD \\ \yt \sim \pt(x,\bar{h}(x))}}[\bar{\ell}(x, \bar{h}(x),\yt)] - \E_{\substack{x \sim \cD \\ \ys \sim \ps(x,\bar{h}(x))}}[\bar{\ell}(x, \bar{h}(x),\ys)]}_{\nabla} | \geq \alpha
	\end{align}
	{\bf Then:} update the model $p^{(t)}$, for all $x, \yhat$
	\begin{align}
	\label{eq:predictor_update_rule}
		p^{(t+1)}(x,\yhat) \leftarrow \Pi \left( p^{(t)}(x,\yhat) - \eta^{(t)} \left[\bar{\ell}(x, \bar{h}(x), 1) - \bar{\ell}(x, \bar{h}(x),0) \right] \ind\{h(x) = \yhat\} \right)
	\end{align}
% TO INCLUDE general categorical case update rule

%	\begin{align}
%	\label{eq:predictor_update_rule_2}
%		p^{(t+1)}(x,\yhat) \leftarrow p^{(t)}(x,\yhat) - \eta^{(t)} \begin{bmatrix}
%			\ell(x, h(x), y_1) \\ 
%			\dots\\
%		    \ell(x, h(x), y_k)
%		\end{bmatrix} \ind\{h(x) = \yhat\}
%	\end{align}
	where $\eta_t = - \sign(\nabla) \; / \; \lmax$

	\item {\bf Else:} terminate and return $p^{(t)}$
\end{itemize}
\vspace*{2mm}
\end{boxedminipage}

\caption{\label{fig:algorithms} Algorithm for generating performatively outcome indistinguishable predictors. Correctness and runtime are analyzed in \propref{prop:loss_calibration_analysis}. For the sake of clarity, here we present the simplest version of the algorithm where $\cYh = \{0,1\}$ is binary and the search outlined in \equationref{eq:constraint} is proper. Both of these conditions can be relaxed as we explore in \sectionref{sec:search}.}
\end{figure}














\section{Performative Outcome Indistinguishability}

Our approach towards achieving decision rules which are simultaneously optimal for a wide variety of losses and marginal distributions over features is centered around achieving the following indistinguishability definition. 

Performative outcome indistinguishability, as we define it below, is a property of a model of nature $\pt$, which captures the probabilities of outcomes in $\cY$, for every individual $x$ and (performative) prediction $\yhat$. 
Intuitively, the condition asserts that, when viewed from the perspective of a particular set of test functions and decision rules, the expected values of these functions under nature and the learner's model of nature are approximately indistinguishable.

\begin{definition}[Performative Outcome Indistinguishability]
Suppose $\cL$ is a collection of loss functions and $\cH$ is a hypothesis class.
For a given tolerance $\eps \geq 0$, a predictor $\pt$ is $(\cL,\cH,\eps)$-performatively outcome indistinguishable (or POI for short) if for all $\ell \in \cL$ and for all $h \in \cH$,
\begin{align}
    \card{\E_{\substack{x \sim \D\\\yt \sim \pt(x,h(x))}}[\ell(x, h(x),\yt)] - \E_{\substack{x \sim \D\\\ys \sim \ps(x,h(x))}}[\ell(x, h(x),\ys)]} \le \eps.
\end{align}
Furthermore, we say that $\pt$ is $(\cL,\cH,\eps)$-reflexively POI if it is $(\cL,\cH',\eps)$
-calibrated for 
\begin{align}
\cH' = \cH \cup \{\ft_{\ell}: \ell \in \cL \}.
\end{align}
\end{definition}

Relative to initial work on outcome indistinguishability (OI) in supervised learning which defines indistinguishability in terms of an abstract class of binary-valued distinguishers, our definition of performative outcome indistinguishability is somewhat more pragmatic. 
It ensures that nature and the learner's model are close in terms of the downstream metrics (the expected risks for a choice of loss and hypothesis) which will ultimately decide whether a predictor is useful or not for a particular application.

Like previous definitions however, this indistinguishability condition can be efficiently achieved assuming the learner can solve a particular search problem, closely related to weak agnostic learning. 
As we now show, one can extend the algorithm from [??? \jcpnote{@mpk}], to nonparametrically construct a predictor $\pt$ which achieves this definition. 
For the sake of simplifying the exposition, we again focus on the case where $\cY$ is binary. Extensions to the general case where $\cY$ is categorical are straightforward (see Appendix ???).

\begin{proposition}
\proplabel{prop:loss_calibration_analysis}
The Indistinguishability Boosting algorithm described in Figure 1 terminates in at most $  \lmax^2 |\cYh| \;/\; \alpha^2$ many iterations and returns a predictor $\pt$ that is
$(\cL, \cH, \alpha)$-self-calibrated. 
\end{proposition}
\begin{proof}
The fact that $\pt$ is reflexively-POI follows directly from the termination criteria. 
To prove the algorithm terminates, the key insight is that if the indistinguishability constraint is violated for any $l$ or $h$, then we will have made nontrivial progress on a common potential function. 
Since this potential is bounded from above and below, and bounded progress is guaranteed with every update, the total number of updates must be bounded. 
We now make this argument formal.
First, note that for any predictor $p$, loss $\ell$, and hypothesis $h$,
\begin{align*}
	\E_{\substack{x \sim \D\\ y \sim p(x,h(x))}} \ell(x, h(x), y) &= \E_{x} \E_{y\mid x} \ell(x, h(x), y) \\
	&= \E_x \ell(x, h(x), 1)p(x,h(x)) + \ell(x, h(x),0)(1 - p(x, h(x))) \\ 
	&= \E_{x}\ell(x, h(x),0) + \left(\ell(x, h(x), 1) - \ell(x, h(x), 1)\right) p(x,h(x)).
\end{align*}
Hence, the difference between any two predictors $p$ and $p'$ (and in particular for $p^{(t)}$ and $\ps$) can be expanded as:
\begin{align*}
	\E_{\substack{x \sim \D\\ \yt \sim \pt(x,h(x))}} \ell(x, h(x), \tilde{y}) - \E_{\substack{x \sim \D\\ \ys \sim \ps(x,h(x))}} \ell(x, h(x), y_*) &= \E_{x} \left(\ell(x, h(x),1) - \ell(x, h(x), 0)\right)\left(\pt(x, h(x)) - \ps(x, h(x))\right) \\ 
	& = \underbrace{\sum_{\yhat} \E_x \left(\ell(x,\yhat,1) - \ell(x,\yhat', 0)\right)\left(\pt(x, \yhat) - \ps(x, \yhat)\right) \ind\{h(x) = \yhat\}}_{\defeq \nabla_t} 
\end{align*}
Now, consider the potential:
\begin{align*}
 \sum_{\yhat} \E_x \left(p^{(t+1)}(x,\yhat) - \ps(x,\yhat)\right)^2 = 	\sum_{\yhat} \E_x \left(\Pi \left(p^{(t)}(x,\yhat)  - \eta \left[\ell(x, h(x), 1) - \ell(x, h(x),0) \right] \ind\{h(x) = \yhat\} \right) -
 \ps(x,\yhat)\right)^2.
\end{align*}
Because projection can only decrease the distance to $\ps$, if an update is performed, the difference between potentials at adjacent time steps,
\begin{align*}
	\sum_{\yhat} \E_x \left(p^{(t+1)}(x,\yhat) - \ps(x,\yhat)\right)^2 - \sum_{\yhat} \E_x \left(p^{(t)}(x,\yhat) - \ps(x,\yhat)\right)^2,
\end{align*}
is upper bounded by 
\begin{align*}
-2 \eta \underbrace{\sum_{\yhat}\E_x(\ell(x,\yhat, 1) - \ell(x, \yhat, 0))  \left(p^{t}(x,\yhat) - \ps(x, \yhat)\right) \ind\{h(x) = \yhat\}}_{\nabla_t} + \eta^2 \underbrace{ \sum_{\yhat}\E_x(\ell(x,\yhat, 1) - \ell(x, \yhat, 0))^2 \ind\{h(x) = \yhat\}}_{\defeq B}.
\end{align*}
From this rewriting, since $\nabla_t \geq \alpha$ by the search criterion in \equationref{eq:constraint} and $|B| \leq \lmax^2$, the difference between potentials satisfies:
\begin{align*}
	\sum_{\yhat} \E_x \left(p^{(t+1)}(x,\yhat) - \ps(x,\yhat)\right)^2 - \sum_{\yhat} \E_x \left(p^{(t)}(x,\yhat) - \ps(x,\yhat)\right)^2 = -2 \eta_t \Delta_t + \eta^2 B \leq -\alpha^2 / \lmax^2
\end{align*}
Hence, the potential must decrease by at least $\alpha^2 / \lmax^2
$ per iteration. Since the potential is lower bounded by 0, upper bounded by $|\cYh|$, and we improve by $\alpha^2 / \lmax^2$ each time, the algorithm is guaranteed to terminate in at most $\lmax^2 |\cYh| / \alpha^2$ many iterations.
\end{proof}

\subsection{Statistical Complexity of Performative Outcome Indistinguishability}

The previous proposition shows that one can efficiently construct a POI predictor $\pt$ with at most a moderately small number of calls to an algorithm which implements the search step outlined in \equationref{eq:constraint}. This begs the question, what are the statistical and computational complexities of solving this search problem? 

Here, we focus on the statistical considerations and delay the discussion on computation for \sectionref{sec:search}. Interestingly, this weak learning problem can be solved using a single exploratory dataset in which predictions are chosen randomly for every $x$:

\begin{proposition}
There exists an algorithm  which given $n \geq \mathcal{O}(\lmax |\cYh|\log(|\cH| |\cL| / \delta)/ \alpha^2)$ samples drawn according to $x\sim \cD, \yhat \sim \unif(\cYh), \ys \sim \ps(x,\yhat)$
implements the search step outlined in \equationref{eq:constraint} with probability $1-\delta$  and runs in time $\mathcal{O}(|\cH| |\cL| n)$.
\end{proposition}

\begin{proof}
The algorithm just runs a for loop and computes the empirical mean of the performative risk for each $h$ and $\ell$. 
Crucially, this can be done off of a single exploratory dataset.
By \lemmaref{lemma:static}, for any hypothesis $h$ and loss $\ell$, the performative risk of $h$ over $\ell$ can be written as the expected risk of a modified objective over distribution that is independent of $h$:
\begin{align*}
\E_{\substack{x \sim \calD_x \\ \ys \sim \ps(x,h(x))}} \ell(x, h(x), \ys) = |\calYhat| \E_{\substack{x \sim \calD_x \\ \yhat \sim \Unif(\calYhat) \\ \ys \sim \ps(x,\yhat)}} \ell(x, \yhat, \ys )\ind \{h(x) = \yhat\}.
\end{align*}	
Since $|\cYh| \cdot \ell(x, \yhat, y)$ is uniformly bounded by $|\cYh| \cdot \lmax$, Hoeffding's inequality guarantees that given $n \geq |\cYh| \cdot  \infn{\cL} / (2\alpha^2) \log(2 /\delta)$ many samples, the empirical mean of the right hand side (over $n$ samples) is $\alpha$ close to its expectation. To get uniform convergence over all $\ell \in \cL$ and $h \in \cH$ it suffices to apply a union bound.
\end{proof}

From this result, we see that at least naively, a total of $\mathcal{O}(\lmax^3 |\cYh|^2 \log(|\cH| |\cL| / \delta)\;/\; \alpha^4)$ many ``RCT'' samples, where $\yhat \sim \unif(\cYh)$ for every $x$, are sufficient to compute a predictor $\pt$ which is $(\cL, \cH, \epsilon)$ performatively outcome indistinguishable. 

\jcpnote{There are of course better ways of getting this concentration analysis to go through (e.g Bernstein's, VC dimension, etc.). Getting the sharpest concentration result doesn't seem to me the main focus on this paper, but we should make a remark to that end.}





==> arxiv 2/intro.tex <==
\section{Introduction}


Data-driven predictions inform policy decisions that directly impact individuals.
Proponents argue that by understanding patterns from the past, decisions can be optimized to improve future outcomes, to the benefit of individuals and institutions \cite{kleinberg2015prediction}.
In the US educational system, for instance, early warning systems (EWS) have become a key tool used by states to combat low graduation rates \cite{balfanz2019early,survey}. 
The rationale for using such systems is clear.  Given a predictor that, for each student, estimates the likelihood of graduation, school districts can identify high-risk students at a young age, directing resources to improve individuals' outcomes, and in turn, the districts' graduation rates.
Despite compelling arguments, reliably predicting life outcomes remains a largely-unsolved problem in machine learning.
% \mpk{why commented?}

% One of the key issues in utilizing predictions to inform decisions is that, often, predictions do not just forecast the world around them, they actively shape it. 
% \mpk{scope.  \emph{An issue?  A challenge?}  predictions influence what? decisions? outcomes? the world?}
A key challenge in utilizing predictions to inform decisions is that, often, predictions influence the outcomes they're meant to forecast.
In the education example above, districts consider predictions of graduation with the \emph{intention} of effecting graduation outcomes.
% for high-risk students.
% when the EWS determines that a given student is unlikely to graduate, the student may qualify for extra support, which ideally helps them to graduate.
In this situation---where predictions determine interventions, which influence outcomes---accuracy can be a paradoxical notion.
If a predictor correctly identifies high risk individuals as likely to suffer negative outcomes, after successful interventions, the individuals' outcomes will be positive and the initial predictions will appear inaccurate.
To apply data-driven tools effectively, decision-makers must resolve an apparent tension between the objectives of \emph{forecasting} individuals' outcomes reliably and \emph{steering} individuals to achieve better outcomes.

% This situation highlights an apparent tension in the goals of data-driven policy
% highlights an apparent tension between two goals of data-driven policy:  accurately forecasting individuals' outcomes and steering individuals to achieve better outcomes.



% These issues \mpk{NOT these \emph{issues}.  The issue of predictions influencing distribution on examples.} were brought to light in the recent work of \cite{performative} on \emph{performative prediction}.
Recent work of \cite{performative} introduced \emph{performative prediction} to contend with the fact that predictions not only forecast, but also shape the world.
Informally, a prediction problem is performative if the act of prediction influences the distribution on individual-outcome pairs.
From early warning systems, to online content recommendations, to public health advisories: across many contexts, individuals respond to predictions in a manner that changes the likelihood of possible outcomes (successful graduation, increased click rate, or decreased disease caseload).
%% commented, discussed later.
% On a technical level, the performative prediction framework generalizes many well-studied problems including supervised learning \cite{shalev2014understanding}, strategic classification \cite{hardt2016strategic}, and causal inference \cite{pearl2009causality,imbens2015causal}.







% \mpk{Performative prediction....

% This tension was brought to light in the computer science community recently in the work of \cite{performative} on \emph{performative prediction}.
% A prediction problem is \emph{performative} if the choice of predictions can influence the distribution on outcomes.
% They highlight how this phenomenon is largely overlooked in the ML/CS communities, and argue that the settings where performativity is at play are widespread.
% Performativity comes up in strategic classification settings, and social dynamics.
% \cite{many,works}
% }

% \begin{itemize}
%     \item Original framing:  very general model of distributional shift
%     \item Allowed to shift---in $\Xcal$ and $\cY$---in response to the decision rule as a whole.  May model broad policy decisions.
%     \item Frames the goals of performative prediction through the loss minimization paradigm;  in particular, a hypothesis is performative optimal if [blah]
% \end{itemize}

In their original work on the subject, \cite{performative} frame the goal of performative prediction through loss minimization.
In this framing, the ultimate goal is to learn a \emph{performatively optimal} decision rule.
A decision rule $h_\mathrm{po}$ is performatively optimal if it achieves the minimal expected loss (within some class of decision rules $\Hcal$) over the distribution that it induces,
\begin{gather}
\equationlabel{eq:po}
    h_\mathrm{po} \in \argmin_{h \in \Hcal} \E_{(x,y) \sim \D(h)}[\ell(x,h(x),y)].
\end{gather}
Here, $\D(h)$ is the distribution over $(x,y)$ pairs observed as response to deploying $h$.

For generality's sake, performative prediction makes minimal restrictions on how the distribution may respond to a chosen decision rule.
In particular, the choice to deploy a hypothesis $h$, may change the joint distribution $(x,y) \sim \D(h)$ over individual-outcome pairs, essentially arbitrarily.\footnote{\cite{performative}  assume only a Lipschitzness condition, where similar hypotheses $h$ and $h'$ give rise to similar distributions $\D(h)$ and $\D(h')$, measured in Wasserstein (earth mover's) distance.}
This generality enables us to write a broad range of prediction problems---including supervised learning \cite{shalev2014understanding}, strategic classification \cite{hardt2016strategic}, and causal inference \cite{miller2020strategic}---as special cases of performative prediction.
In all, \cite{performative} establishes a powerful framework for reasoning about settings where the distribution of examples responds to the predictions.


% In the original work, \cite{performative} propose a broad framing of the problem where performativity, the impact of predictive models on their environment, is a function of the predictor $h$.
% That is, every decision rule $h$, mapping individuals $x$ to predictions $\yhat$, induces a potentially distinct distribution $\cD(h)$ over the joint distribution of individuals and outcomes $(x, y)$.
% One of the main goals in this setting is to find \emph{performatively optimal} decision rule $h_\mathrm{po}$.
% These are models which achieve the best possible expected risk over the distribution they induce: 
% \begin{gather*}
%     h_\mathrm{po} \in \argmin_{h \in \Hcal} \E_{(x,y) \sim \D(h)}[\ell(x,h(x),y)].
% \end{gather*}


While powerful, the framework has two noticeable limitations.
First, achieving performative optimality is hard.
Without any assumptions on the distributional response $\D(\cdot)$, achieving performative optimality requires exhaustive search over the hypothesis class $\Hcal$.
Furthermore, even under strong structural assumptions on the distributional response and choice of loss $\ell$, it is known that convex optimization does not suffice to achieve optimality \cite{performative, miller2021outside}.
Stated another way: the generality of performative prediction does not come for free.
To date, all existing methods for performative optimality require strong specification assumptions on the outcome distribution and distributional response.

The second limitation arises due to formulating performative prediction as a loss minimization problem:  the loss $\ell$ is fixed, once and for all.
In performative prediction, different losses can encode drastically different objectives:  losses are used not only to promote accuracy of predictions, but also to encourage favorable outcome distributions.
Consider a loss designed for accurate forecasting, e.g., the squared error $(\yhat - y)^2$.
In this case, the optimal decision rule will prioritize accuracy without regard for the ``quality'' of the outcome distribution.
% In fact, the decision rule may be chosen to steer individuals towards a \emph{predictable} outcome distribution, rather than a desirable distribution.
On the other hand, consider a loss designed to steer towards positive outcomes, $1-y$.
Here, there is no notion of accuracy (the loss ignores the prediction $\yhat$), but instead, the objective is to nudge the distribution of outcomes towards $y = 1$.
% the predictions may no longer give calibrated forecasts.


Encoding the decision-making objective through a single loss function forces the learner to choose the ``correct'' objective at train time.
% , obscuring the tension between the goals of accurate forecasting and steering to desirable outcomes.
Downstream decision-makers, however, may reasonably want to explore different objectives according to their own sense of ``optimality''.
% and understand \emph{why} the resulting decision rule is optimal.
In the existing formulations for performative prediction, exploring different losses requires re-training from scratch.
In this work, we investigate an alternative formulation that enables decision-makers to efficiently explore optimal decision rules under many different objectives.

% Here, we investigate an alternative abstraction for performative prediction that eliminates the need to fix a single loss function.
% Identifying an abstraction that eliminates the need to fix a single loss function has been an important open direction, stated explicitly in the discussion of \cite{miller2021outside}.
% A skeptical decision-maker may reasonably want to understand \emph{why} the chosen decision rule is optimal, or elect to choose predictions according to their own definition of what is ``optimal''.

% \mpk{
% In performative prediction, each choice of loss function implicitly encodes some tradeoff between forecasting and steering.
% Classical supervised learning losses like the 01 loss, 1{h(x) != y}, direct the learner to choose decision rules which prioritize predictive accuracy above all else.
% Conversely, steering losses, such as l(yhat, y) = 1-y, disregard accuracy completely.
% The optimal predictor for this loss is the one that best steers the distribution towards a particular target.
% Convex combinations of these two losses interpolate between these two, potentially contradictory, objectives.
% The value of a performative omnipredictor is that it explicitly allows the learner to punt on this question of what is the right notion of optimality, as captured by specific choice of loss function.
% Omnipredictions “frontloads” all the learning.
% The goal is to find a single, simple predictor that downstream decision-makers can easily post-process to achieve their own particular notion of optimality from a wide menu of options (losses), without the need to retrain.
% Different losses encode different optimal predictors.  Could be very different in this setting if we're steering towards different types of outcomes.
% Want a new solution concept:  separates the task of learning from decision-making.  Single learner.  Then, decision-maker gets to choose what is ``optimal''.
% }





% While powerful, this initial, function-based viewpoint for performative prediction is somewhat limited in what it can accomplish. Previous work \cite{miller2021outside, performative} has established how optimality can be computationally and statistically difficult to achieve, even under strong, structural assumptions on the mapping between predictions and distributions captured in $\cD(\cdot)$.


% In particular, recognizing that predictions have the power to influence outcomes, a natural desiderata in performative performative is to develop tools which empower system designers to balance between \emph{forecasting} and \emph{steering}. 
% In online content moderation for example, one may want to nudge users towards certain kinds of content versus others. Furthermore, the decision of \emph{where} to steer outcomes is highly dependent on social context. 
% School districts all using the same early warning system may have different priorities on which students to prioritize. 
% This tension regarding how to balance between different objectives is core to the kinds of problems that performative prediction seeks to address. However, all existing works in this area assume the loss function $\ell$ is fixed, once and for all.
% By encoding the decision-making objective through a single loss function, these results obscure the central tension between forecasting and steering.






%Beyond the computational and statistical challenges of achieving performative optimality, there are also evident limitations to the definition itself.
%A \jcpnote{all accuracy like losses are the same}
%
%For instance, consider a loss designed for accurate forecasting (say, the squared error).
%In this case, the optimal decision rule may steer individuals towards a \emph{predictable} outcome distribution, rather than a desirable distribution.
% \jcpnote{Juanky inserts quick example?}
%On the other hand, if we choose a loss designed to steer towards positive outcomes, the predictions may no longer give calibrated forecasts.
%A skeptical decision-maker may reasonably want to understand \emph{why} the chosen decision rule is optimal.
%These shortcomings in the notion of optimality raise the question of whether there is a different abstraction that naturally accommodates exploration of different objectives by downstream decision-makers.











% The characterization gives credence to a common learning paradigm:  a decision maker observes data, trains and deploys a hypothesis $h$, then retrains using data observed from $\D(h)$.
% While syntactically similar, stability and optimality are very different solution concepts.
% Unlike performative stability, performative optimality is not obviously achieved by any simple method like iterative retraining.
% As a consequence, \cite{performative} show that the loss achieved by performative stable points can be arbitrarily worse than the performative optimal.
% This separation motivates investigations into methods that go beyond retraining, towards achieving globally optimal loss.














% \mpk{
% In the original work, \cite{performative} identifies two solution concepts for performative prediction problems: \emph{stability} and \emph{optimality}.
% A decision rule $h_\mathrm{ps}$ is performative stable if $h_\mathrm{ps}$ is amongst the best predictors under the induced distribution when $h_\mathrm{ps}$ is ``deployed''.
% % in other words, the predictor is a ``stationary'' solution.
% Formally, for hypothesis class $\Hcal$ and loss function $\ell$, performative stability is defined as a ``stationarity'' condition:
% \begin{gather*}
%     h_\mathrm{ps} \in \argmin_{h \in \Hcal} \E_{\D(h_\mathrm{ps})}[\ell(h(x),y)]
% \end{gather*}
% where $\D(h_\mathrm{ps})$ is the distribution over $(x,y)$ pairs under the predictions given by $h_\mathrm{ps}$.
% The main results of \cite{performative} characterize performative stability as the set of predictors achieved through iterative retraining.
% The characterization gives credence to a common paradigm:  a decision maker observes data, trains and deploys a hypothesis $h$, then retrains using data observed from $\D(h)$.
% Once these dynamics stablize, the resulting predictor satisfies performative stability.

% Performative optimality, on the other hand, is a global condition that requires a hypothesis $h_\mathrm{po}$ to achieve the minimum loss $\ell$ amongst all hypotheses $h \in \Hcal$.
% \begin{gather*}
%     h_\mathrm{po} \in \argmin_{h \in \Hcal} \E_{\D(h)}[\ell(h(x),y)]
% \end{gather*}
% While syntactically similar, stability and optimality are very different solution concepts.
% To start, note that optimal hypotheses may not be stable hypotheses.
% Despite its global optimality,  $h_\mathrm{po}$ may be locally suboptimal; that is, $h_\mathrm{po}$ may not be a loss minimizer under $\D(h_\mathrm{po})$.
% \begin{gather*}
% h_\mathrm{po} \not \in \argmin_{h \in \Hcal}\E_{\D(h_\mathrm{po})}[\ell(h(x),y)]
% \end{gather*}
% In particular, optimality is not obviously achieved by any simple method like iterative retraining.
% As a consequence, \cite{performative} show that the loss achieved by performative stable points can be arbitrarily worse than the performative optimal.
% This separation motivates investigations into methods that go beyond retraining, towards achieving globally optimal loss.
% To date, the only known methods for obtaining performative optimality require strong assumptions about the underlying distribution on outcomes \cite{miller2021outside}.

% }



% \mpk{



% While performative prediction raises important issues, the performative prediction abstraction does not adequately address the central tension between forecasting and steering.

% Existing works do not address the central tension between the goals of forecasting and steering.
% Indeed, all existing works on performative prediction assume the loss function---which encodes the objective---is fixed in advance.
% Fixing a loss function obscures the competing goals of performative prediction.


% Existing works assume that the loss function $\ell$ is fixed in advance.
% This is troubling for a few reasons.

% On a more fundamental level, optimizing a given loss function may not do what we intend.


% On a practical level, different clients may have different loss functions, which necessitates training a different model for each client.
% \begin{itemize}
%     \item To date, methods for obtaining optimality are limited.  Require making very strong assumptions about the true outcome model.
%     \item Worse yet, 
% \end{itemize}


% To date, the only known methods for obtaining performative optimality work under very strong assumptions about the way that nature governs outcomes under performativity \cite{juankyEtAl}.

% Even if we could achieve optimality in the framing of \cite{performative}, one downside is that the framing fixes a loss function.
% In particular, the framework forces you to choose between objectives up front.
% For instance, if the goal is the give most accurate predictions (insert Juanky example of bad steering).
% Effectively, this decision rule steers individuals towards a predictable outcome distribution, not a beneficial one.
% Alternatively, we may optimize a loss designed to steer individuals towards good outcomes, but then be unsure of the rationale for using the decision rule.
% These choices, which are made by the developers of the prediction model, are fixed in advance, hiding the central tension between forecasting and steering from the client of the model.
% An ideal EWS would allow districts to explore and optimize a loss suited to their needs without retraining.  Does it exist?
% }



% Predictions inform policy
% \begin{itemize}
%     \item Idea:  predictions give us a sense of likelihoods of outcomes
%     \item We can use these estimates to choose policy that leads to favorable outcomes, for institutions and individuals
% \end{itemize}
% But often, predictions actually influence the outcomes they're meant to predict
% \begin{itemize}
%     \item Can be direct or indirect
%     \item Example, Education EWS:  prediction that student is likely to struggle graduating may be criterion to give special programming
%     \item That is, predictions often influence \emph{decisions}, which themselves influence outcomes
%     \item STEERING
% \end{itemize}
% Formalized in Performative Prediction:
% \begin{itemize}
%     \item (Perdomo et al.) study the issue of prediction under performativity
%     \item Two key solution concepts:
%     \begin{itemize}
%         \item Stability -- efficiently achieved via iterative retraining
%         \item Optimality -- no known efficient algorithms; worst-case:  seems to require exhaustive exploration of the space of decision rules (or strong assumptions on how Nature behaves)
%     \end{itemize}
%     \item In general, stability and optimality are very different solutions (incomparable qualitatively and quantitatively)
% \end{itemize}
% Challenges:
% \begin{itemize}
%     \item Absent strong assumptions on outcome distribution, no methods for obtaining optimality
%     \item Existing work focuses on optimizing a fixed loss function.  But losses---especially in the performative context---may serve very different complementary roles.
%     \item Losses:
%     \begin{itemize}
%         \item for giving accurate estimates of probabilities of outcomes (probability of graduation)
%         \item for steering the outcomes in a certain direction (promoting graduation)
%         \item really would love all in one:  understand probability of outcomes under a given policy. and be able to explore/optimize, with reliable estimates of losses under different policies.
%     \end{itemize}
% \end{itemize}


\subsection{Decision-Making under Outcome Performativity}
%In this work, we revisit the question of efficiently obtaining performative optimality under realistic assumptions.

% In this work, w
To begin, we introduce a special case of the performative prediction setting, which we call \emph{outcome performativity}.
Outcome performativity focuses on the effects of local decisions on individuals' outcomes, rather than the effect of broader policy on the distribution of individuals.
For instance, our example of graduation prediction is modeled well by outcome performativity.
For a given a student, the EWS prediction they receive affects their future graduation outcome, but does not influence their demographic features or historical test scores.
%beyond individual-level effects, the warning system does not meaningfully influence on the population (e.g., the distribution on demographic features is unaffected).
% Historical features are unaffected by prediction, and the only thing that affects the future graduation outcome is the EWS prediction a student receives.
In other words, we narrow our attention to the performative effects of decisions $h(x)$ on the conditional distribution over outcomes $y$, rather than the effects of the decision rule $h$ on the distribution as a whole $\D(h)$.
This reframing of performativity still captures many important decision-making problems, but gives us additional structure to address some of the limitations in the original formulation.


% \paragraph{Outcome Performativity.}
% Our first contribution is conceptual.
% We introduce a specialization of the performative prediction framework which we call \emph{outcome performativity} that we believe provides a more accurate representation of various consequential decision-making problems.
%\purple{commented out the first sentence, think it made things seem a bit repetitive}
%As the name suggests, in outcome performativity, we assume that performative effects are limited to the conditional distribution over outcomes and that this influence occurs independently over individual units $x \in \Xcal$. 


%In this way, outcome performativity focuses on the effects of local decisions on individuals' outcomes, rather than the effect of broader policy on the distribution of individuals.
%For instance, our example of graduation prediction is captured well by outcome performativity:  a given student's graduation is directly influenced by the EWS prediction they receive, but is largely unaffected by the EWS predictions on other students.
% A given student's EWS prediction directly influences their likelihood of graduation; the student's graduation, however, is largely unaffected by the EWS predictions on other students.
On a technical level, outcome performativity imagines a data generating process over triples $(x,\yhat, \ys)$ where $x \sim \D$ is sampled from a \emph{static} distribution over inputs, then a prediction or decision $\yhat \in \Ych$ is selected (possibly as a function of $x$), and finally the true outcome $\ys \in \cY$ is sampled conditioned on $x$ and $\yhat$.
We focus on binary outcomes $\cY = \set{0,1}$.\footnote{In general, outcome performativity could be defined for larger outcome domains.  Handling such domains is possible, but technical.  We restrict our attention to binary outcomes to focus on the novel conceptual issues.}
In this setting, the outcome performativity assumption posits the existence of an underlying probability function,
\begin{align*}
\ps:\Xcal \times \Ych \to [0,1],	
\end{align*}
where for a given individual $x \in \Xcal$ and decision $\yhat \in \Ych$, the true outcome $\ys$ is sampled as a Bernoulli with parameter $\ps(x,\yhat)$.
We refer to the true outcome distribution $\ps$ as \emph{Nature}.

% Given an individual's features $x \in \X$ and  a decision $\yhat \in \Ych$, we assume the true distribution on outcomes is fixed.
% In this view, the inputs $x \in \X$ represent reliable (rather than manipulable) features of individuals.
By asserting a fixed ``ground truth'' probability function, the outcome performativity framework does not allow for arbitrary distributional responses and limits the generality of the approach. For instance, outcome performativity does not capture strategic classification.
But importantly, by refining the model of performativity, there is hope that we may sidestep the hardness results for learning optimal performative predictors.
% Modeling the ``ground truth'' as a map from individual-decision pairs to probabilities 
% Concretely, the outcome performativity assumption motivates a new paradigm for learning optimal predictors: to learn a function $\pt:\Xcal \times \Ych \to [0,1]$ that mimics $\ps$ in a manner that allows for optimal downstream decisions.


%% juanky's text
% This matches the natural flow of time for various prediction problems.
% We observe individual students in middle school, make predictions at the start of high school, and observe graduation outcomes several years later.
% This is in contrast to the general performative prediction setting where a decision maker deploys a decision rule $h$ and observes samples $(x,y)$ sampled from some a priori arbitrary distribution $\cD(h)$.
% In this setting, the marginal distribution over individuals $x$ can be impacted by $h$, as in strategic classification.
% We explicitly rule out this type of feedback in outcome performativity. 

















% \mpk{I suggest moving some of this to the next section.


% A careful examination of the mechanism by which performativity arises reveals a promising perspective.  
% Thinking back to the education example, the influence of predictions on the data distribution is not really a consequence of the decision rule $h$, but of the prediction $h(x)$.
% The decision of a teacher to intervene on a student is determined by the prediction $\yhat$ itself of whether a student is high or low risk, not by the functional form of whatever decision rule generated the prediction. 
% Furthermore,  predictions are observed by teachers, not students, and generated only after individual features are measured. Therefore, these predictions $
% \yhat$ cannot impact the distribution over individual students $x$, only the likelihood of outcomes $y$ which lie in the future relative to $x$ and $\yhat$.
% While these might seem like obvious or mundane observations, they motivate a specialization of the performative prediction framework which we call \emph{outcome performativity} in which significantly stronger results are possible.

% The main goal of this work is to develop theory that directly addresses these concerns. We illustrate that by carefully framing the outcome performativity problem, we can develop predictors which empower optimal-decision making for many different populations and for a wide variety of objectives. We now discuss these ideas in more detail.

% }


















\begin{figure}
\begin{center}
\begin{tikzpicture}[scale=0.2]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [black] (30.7,-27.5) circle (3);
\draw (30.7,-27.5) node {$x$};
\draw [black] (38.7,-18.7) circle (3);
\draw (38.7,-18.7) node {$\yhat$};
\draw [black] (46.2,-27.5) circle (3);
\draw (46.2,-27.5) node {$\ys$};
\draw [black] (32.72,-25.28) -- (36.68,-20.92);
\fill [black] (36.68,-20.92) -- (35.77,-21.18) -- (36.51,-21.85);
\draw [black] (33.7,-27.5) -- (43.2,-27.5);
\fill [black] (43.2,-27.5) -- (42.4,-27) -- (42.4,-28);
\draw [black] (40.6,-21.3) -- (44.19,-25.27);
\fill [black] (44.19,-25.27) -- (44.02,-24.34) -- (43.28,-25.02);
\end{tikzpicture}
\end{center}
\caption{Causal graphical representation of the outcome performativity data generating process.}
\end{figure}
% We now move onto to presenting how this viewpoint enables the development of \emph{performative omnipredictors}: decision rules that are simultaneously optimal for a wide variety of objectives.


    % \begin{itemize}
        % \item outcome performativity is a well-motivated special case of performative prediction
        % \item treats the input distribution as a distribution of individuals $x \in \Xcal$.
        % \item outcome performativity only occurs as a change in \emph{outcome distribution}.
        % \item Technically, this is equivalent to positing the existence of some $\ps:\Xcal \times \Ych \to [0,1]$ where for a given individual $x \in \Xcal$ and decision $\yhat \in \Ych$, $\ps(x,\yhat)$ is the true probability with which the outcome $\ys$ is sampled.
        % \item This abstraction---modeling the ``ground truth'' as a map from individual-decision pairs to probabilities---motivates a new learning objective, to learn a function $\pt:\Xcal \times \Ych \to [0,1]$ that mimics $\ps$ in a manner that allows for optimal downstream decisions.
        % \item Conceptually, explicitly modeling the effect of a selected decision on the distribution over outcomes is natural, but is a departure from all earlier works on performative prediction, which focused on methods of direct loss minimization over decision rules.
    % \end{itemize}



\newcommand{\fs}{f^*}
\paragraph{Performative Omniprediction.}
We begin by observing that under outcome performativity, the true probability function $\ps$ suggests an optimal decision rule $\fs_\ell:\Xcal \to \Ych$ for any loss $\ell$.
In our setting, $\ps$ governs the outcome distribution, so given an input $x \in \Xcal$, the optimal decision $\fs_\ell(x)$ is determined by a simple, univariate optimization procedure over a discrete set $\Ych$:
\begin{gather}
\equationlabel{eq:opt_dr}
    \fs_\ell(x) \in \argmin_{\yhat \in \Ych}\E_{\ys \sim \ps(x,\yhat)}[\ell(x,\yhat,\ys)].
\end{gather}
Note that the decision rule $\fs_\ell(x)$ minimizes the loss pointwise for $x \in \Xcal$. Consequently, averaging over any static, feature distribution $\D$, the decision rule $\fs_\ell$ is performative optimal
%\footnote{Indeed, note that $\fs_\ell$ competes with the global minimizer over $h \in \Hcal$ of the outcome performative loss, and is not merely a stable decision rule.} 
for \emph{any} hypothesis class $\Hcal$, loss $\ell$, and marginal distribution $\cD$:
\begin{gather*}
    \E_{\substack{x \sim \D\\\ys \sim \ps(x,\fs_\ell(x))}}[\ell(x,\fs_\ell(x),\ys)] \le \min_{h \in \Hcal} \E_{\substack{x \sim \D\\\ys \sim \ps(x,h(x))}}[\ell(x,h(x),\ys)].
\end{gather*}
While the existence of $\ps$ implies the existence of optimal decision rules under outcome performativity, we make no assumptions about the learnability of $\ps$.
In general, the function $\ps$ may be arbitrarily complex, so learning (or even representing!) $\ps$ may be infeasible, both computationally and statistically.
Still, the above analysis reveals the power of modeling the probability function $\ps:\Xcal \times \Ych \to [0,1]$.
The optimal probability function $\ps$ encodes the optimal decision rule $\fs_\ell$ \emph{for every loss function } $\ell$.
%Furthermore, the decision rule $\fs_\ell$ is simple to deploy, it only requires a simple post-processing of $\ps$. 
% that is, the predictor $\ps$ encodes the optimal decision rule $\fs_\ell$ \emph{for every loss function } $\ell$.
This perspective raises a concrete technical question:  short of learning $\ps$, can we learn a probability function $\pt:\Xcal \times \Ych \to [0,1]$ that suggests an optimal decision rule, via simple post-processing, for many different objectives?
% given a loss $\ell$, suggests a decision rule $\ft_\ell:\Xcal \to \Ych$ that is performative optimal with respect to a given hypothesis class $\Hcal$?
% If we could access it, then we could use it to find optimal decision rules for many objectives.

% \mpk{updated text}
Recent work of \cite{omni} studied the analogous question in the context of supervised learning (without performativity), formalizing a solution concept which they call \emph{omniprediction}.
Intuitively, an omnipredictor is a single probability function $\pt$ that suggests an optimal decision rule for many different loss functions $\cL$.
The work of \cite{omni} and follow-up work of \cite{gopalan2022loss} demonstrate---rather surprisingly---that omniprediction in supervised learning is broadly a feasible concept.
For a variety of choices of loss classes $\cL$ (e.g., Lipschitz losses or convex losses), it is possible to learn an efficient predictor $\pt$ that gives optimal decisions for any loss $\ell \in \cL$.
% Hence, we could empower decision makers to optimize with regards to a loss of their choosing and balance between steering and forecasting as they see fit. 




% \begin{itemize}
%     \item Of course, $\ps$ is inaccessible.  Could be statistically unlearnable, and very complicated.
%     \item But is there an efficient way to mimic the optimality behavior?
%     \item Note:  the arguments for optimality applied to any loss $\ell$.  Can we mimic this?  Can we hope to learn a $\pt$ that would give us access to $\ft_\ell$ that would similarly behave as optimal decision rules?
%     \item This question was asked in the supervised learning setting!
%     \item This derivation of an optimal decision rule $\fs_\ell$ suggests some reason for optimism.
%     \begin{itemize}
%         \item First, suggests that if we know our loss function, there is a concrete target optimal predictor.  We know how to say what the best is.
%         \item Second, more intriguingly, the approach hardly depends on the loss.  We only need the loss at the very end.  So, in our paradigm of learning $\pt$ to approximate $\ps$, then post-processing for optimal decision rule, in principle, we may be able to mimic optimal decisions for many losses.
%     \end{itemize}
% \end{itemize}


% raises two intriguing possibilities:
% (1) for a fixed loss, at least in principle, we know what our target should be; (2) the way we got the optimal decision rule was \emph{for every loss}, start with $\ps$, then post-process to $\fs_\ell$.





In this work, we generalize omniprediction to the outcome performative setting.
As a solution concept, \emph{performative omniprediction} directly addresses the limiting assumption in performative prediction that the loss $\ell$ is known and fixed.
Given a performative omnipredictor, a decision-maker can explore the consequences of optimizing for different losses, balancing the desire for forecasting and steering, as they see fit.
Technically, given a predictor $\pt$, we define $\ft_\ell:\Xcal \to \Ych$ to be the optimal decision rule,
% in analogy with $\fs_\ell$, where $\ft_\ell(x)$ is the optimal decision, 
 that acts as if outcomes are governed by $\pt$.
\begin{gather*}
    \ft_\ell(x) \in \argmin_{\yhat \in \Ych}\E_{\yt \sim \pt(x,\yhat)}[\ell(x,\yhat,\yt)]
\end{gather*}
We emphasize that, for any loss $\ell$, the decision rule $\ft_\ell(x)$ is an efficient post-processing of the predictions given by $\pt(x,\yhat)$ for $\yhat \in \Ych$.
A performative omnipredictor is a model of nature $\pt:\cX \times \cYh \rightarrow [0,1]$ that induces a corresponding decision rule $\ft_\ell$ that is performatively optimal over a collection of losses $\ell \in \cL$.
\begin{definition*}[Performative Omnipredictor]
For a collection of loss functions $\cL$, hypothesis class $\Hcal$, and $\eps \ge 0$, a predictor $\pt:\Xcal \times \Ych \to [0,1]$ is an $(\cL,\Hcal,\eps)$-performative omnipredictor  for an input distribution $\cD$ if for every $\ell \in \cL$, the decision rule $\ft_\ell$ is $\eps$-performative optimal over $\Hcal$.
\begin{gather}
\equationlabel{eq:omni_guarantee}
    \E_{\substack{x \sim \D\\\ys \sim \ps(x,\ft_\ell(x)))}}[\ell(x,\ft_\ell(x)), \ys)] \le \argmin_{h \in \Hcal} \E_{\substack{x \sim \D\\\ys \sim \ps(x,h(x))}}[\ell(x, h(x),\ys)] + \eps
\end{gather}
\end{definition*}
% This ambitious notion is particularly well-motivated in the performative world.
% While notions of predictive optimality are qualitatively similar in supervised learning\footnote{Predictors which optimize different losses, e.g. squared vs cross-entropy, often produce very similar outputs.},
While an intriguing prospect, omniprediction is particularly ambitious in the performative world.
Whereas most supervised learning losses have the same moral goal (to accurately forecast the outcome), losses in the performative world can encode entirely contradictory objectives.
For instance, we can define a pair of losses $\ell_0$ and $\ell_1$ that reward decisions that steer outcomes to be $0$ and $1$, respectively.
% The performatively optimal predictors for different loss functions can be drastically different.
% For example, in news recommendation systems, reasonable people can have completely opposed opinions as to what kinds of articles we should steer people towards.
A performative omnipredictor must contend with these contradictions, providing optimal decision rules under performative effects.
% Given a performative omnipredictor, a decision-maker can easily explore different objectives with the certainty that the final decision rule will be optimal, even taking into account performative feedback effects.
% In short, they are empowered to directly contend with tradeoffs between forecasting and steering.

% But is the definition too strong?
% Do efficient omnipredictors exist or does omniprediction require learning $\ps$?
% \mpk{
% Even in the supervised learning setting, the existence of efficient omnipredictors is not at all obvious.
% The main result of \cite{omni} demonstrates the feasibility of (supervised) omnipredictors over any hypothesis class $\Hcal$, for the class $\cL_\mathrm{cvx}$ of all convex and Lipschitz loss functions.
% This sweeping result draws a connection between optimal decision-making and the notion of \emph{multicalibration} from the algorithmic fairness literature \cite{hkrr}.
% }




% Understanding the feasibility of performative omniprediction is even more subtle.
% In the supervised setting, the choice of loss function $\ell \in \cL$ exactly determines the optimal post-processing of the predictions given by $\pt$ to a decision rule.
Concretely, under outcome performativity, there is a certain circularity in naively determining the optimal decision $\ft(x)$ from a prediction $\pt(x,\yhat)$.
% In particular,
Choosing an ``optimal'' decision $\ft(x)$ causes a shift in the distribution on the outcome $\ys \sim \ps(x,\ft(x))$, which may imply a different ``optimal'' decision, which seems to lead to a continuing cycle of dependency.
In this way, any performative omnipredictor $\pt$ must encode the optimal decision rule $\ft_\ell$ for each $\ell \in \cL$, \emph{anticipating the shift} induced by the choice of $\ft_\ell$.
In this work, we ask whether---despite this key challenge---efficient performative omnipredictors exist, and if so, can we learn them?






    % \begin{itemize}
        % \item Note that given $\ps$, we can obtain performative optimal decisions under \emph{any} loss!  For a given $x$, we can search over $\yhat \in \Ych$:  outcomes are generated as $\ys \sim \ps(x,\yhat)$, so we can choose the decision that minimizes the expectation $\E_{\ys \sim \ps(x,\yhat)}\ell(x,\yhat,\ys)$.
        % \item Solution concept:  omnipredictor.  Omniprediction was recently introduced in the supervised learning world, but is particularly well-motivated in the performative world.  Allows us to consider multiple losses, which encode different objectives (e.g., forecasting and steering).
        % \item While we posit that $\ps$ exists, we make no assumptions about its complexity.  In other words, the existence of $\ps$ does not obviously imply the existence of \emph{efficient, learnable} performative optimal decision rules.
        % \item Our main result shows that learning efficient omnipredictors is possible, even under outcome performativity.
        % \item \textbf{THEOREM:}  For any collection of losses, hypothesis class, and $\eps > 0$, there exists an $(\cL,\Hcal,\eps)$-performative omnipredictor with complexity $c(\cL,\Hcal) \cdot \poly(1/\eps)$.
        % \mpk{how does the complexity of $\cL$ come in actually?}
    % \end{itemize}
    

\subsection{Our Contributions}

Our first contributions are conceptual, introducing the outcome performativity setting and the notion of performative omnipredictors.
As an abstraction, outcome performativity strikes a balance 
with enough generality to model many real-world phenomena and enough structure to give effective solutions.
For settings where the distributional response occurs predominantly as outcome performativity, the framework is well-scoped to contend with the challenges of performative prediction.
In particular, performative omnipredictors provide an effective solution concept to address the tension between different objectives under performativity.

% \mpk{New text}
With these conceptual contributions in place, we turn to the feasibility of omniprediction under outcome performativity.
While outcome performativity introduces a number of new challenges, we show how to apply many techniques established for omniprediction in the supervised learning setting to recover analogous guarantees under performativity.
On a technical level, we follow the \emph{Loss Outcome Indistinguishability} approach of \cite{gopalan2022loss}, demonstrating how---with the right conceptual framing---arguments for the existence of supervised omnipredictors can be translated into guarantees for the performative setting.



\paragraph{Efficient Performative Omnipredictors Exist.}
Our first technical contribution demonstrates existence of efficient performative omnipredictors.
We prove that for any class of losses $\cL$ and any hypothesis class $\Hcal$, there exists a performative omnipredictor $\pt$ of complexity that scales polynomially with the complexity of computing the losses and hypotheses.
\begin{result}
\label{result:omni}
Suppose $\D$ is a fixed distribution over $\Xcal$.
Let $\cL \subseteq \set{\ell:\Xcal\times \Ych \times \cY \to [0,1]}$ be a set of bounded loss functions, and let $\cH \subseteq \set{h:\Xcal \to \Ych}$ be a hypothesis class of decision rules. 
If the functions in $\cL$ and $\cH$ can be computed by circuits of size $s$, then there exists a $(\cL,\Hcal,\eps)$-performative omnipredictor of circuit complexity $\poly(s, |\cYh |) / \eps^2$.
\end{result}
Importantly, this result holds \emph{for any} class of bounded losses.
The collection $\cL$ may include losses for forecasting and steering, or may include losses that steer towards different outcomes.
Still, the predictor $\pt$ will encode a performative optimal decision rule for each such loss $\ell \in \cL$.
Furthermore, the complexity of this predictor scales gracefully with the complexity of the losses and hypotheses and the available decisions, \emph{independent of the complexity of Nature} $\ps$.
Even if the true probability function $\ps$ is intractably-complex, there exists a simple function $\pt$ that mimics the omniprediction behavior, provided the losses and hypotheses are sufficiently simple.

% This result is quite general in the sense that we make no assumptions, e.g. convexity, on the functions in $\cL$. We only assume that they are bounded. For typical problems with binary outcomes $\cY$, we think of the space of decision $\cYh$ as a small constant. Hence, the overall complexity of the omnipredictor $\pt$ is reasonably small, even if nature's model of nature $\ps$ is intractably complex.


\paragraph{Learning Performative Omnipredictors Reduces to Supervised Learning.}

In fact, the proof of existence is constructive.
We establish the feasibility of performative omnipredictions by devising a boosting-style learning algorithm, inspired by the original algorithm for learning (non-performative) omnipredictors  \cite{hkrr,oi,omni,gopalan2022loss}.
% by examining the output of a boosting-style algorithm for learning performative omnipredictors.
As in the supervised case, we show that learning omnipredictors reduces to an \emph{auditing} task.
%This is surprising because while in supervised learning there is only a single distribution over pairs $(x,y)$, in performative prediction there are \emph{many}.
Despite the fact that in performative prediction, different decision rules induce different distributions, we show that given appropriately randomized data, this auditing task can be solved using only \emph{supervised learning} primitives implementable in finite samples.
That is, under outcome performativity, there is a surprising reduction from the task of learning optimal performative predictors to the task of non-performative supervised learning.

Formally, we assume that the learner has access to a collection of data triples $(x,\yhat,y) \sim \D_\mathrm{rct}$ where inputs are sampled from the data distribution $x \sim \D$, decisions $\yhat$ are assigned uniformly at random, and the outcome $\ys \sim \ps(x,\yhat)$ is sampled from Nature, for the given individual and randomly-assigned decision.
Given an efficiently bounded number of samples access from this distribution, we show how to learn performative omnipredictors assuming access to a supervised learner for the hypothesis class $\Hcal$.
We formalize this learning assumption in terms of cost-sensitive classification \cite{elkan2001foundations}.
% Instead, the success of the POI-boost algorithm is contingent on the ability to solve basic supervised learning problems like cost-sensitive classification. 

\begin{result}[Informal]
\label{result:learning}
Assume sample access to $\D_\mathrm{rct}$  and
suppose that $\cA$ is a cost-sensitive learning algorithm for the hypothesis class $\Hcal$.
% that the one can assign predictions $\yhat$ randomly to individuals $x$ and that $\cA$ is an efficient cost-sensitive learning algorithm for the hypothesis class $\cH$.
There is a polynomial-time algorithm, that, for any set of bounded losses $\cL$, returns a $(\cL, \cH, \epsilon)$-performative omnipredictor using at most $\poly(1/\epsilon,\; |\cYh|,\;\log |\cH|,\; \log|\cL|)$ many samples from $\D_\mathrm{rct}$ while also making $|\cL|\cdot \poly(1/\eps,\; |\cYh| )$ oracle calls to $\cA$.
\end{result}
The guarantees of this algorithm represent a significant point of departure from previous work on performative prediction.
Specifically, previous algorithms for learning performatively optimal models (for a single loss) hinged on the condition that predictions had very mild, and highly-structured (e.g. linear) impact on the induced data distributions  as in \cite{miller2021outside,jagadeesan22a}.
Conversely, within the outcome performativity restriction, we make no assumptions on the way predictions influence outcomes.
Further, the omnipredictor output in the guarantee of Theorem~\ref{result:learning} has complexity scaling as stated in Theorem~\ref{result:omni}.
In other words, our learning algorithm makes no ``realizability'' assumptions and outputs an efficient predictor, regardless of the complexity of Nature.

% From this, we see that at least statistically, we can find omnipredictors that are optimal for an exponentially large collection of losses $\cL$ and decision rules $\cH$. However, computationally, this requires linearly searching over all objectives in $\cL$. Seeing as how writing down an exponentially large collection of objectives for typical outcome performative problems like EWS likely requires significant creative effort, this linear dependence is unlikely to be a bottleneck in practice.
% In theory, we show how it can be avoided in certain special cases by exploring connections to the multicalibration literature \cite{hkrr}.
%%% move reference to this stuff to the technical overview
 
\paragraph{Universally-Adaptable Omnipredictors.}
Outcome performativity focuses attention on performative shifts in the outcome distribution as a function of the chosen decision $\yhat \in \Ych$.
In particular, it excludes performative effects in the distribution over individuals $\Xcal$.
Despite this limitation, our final result shows that we can learn performative omnipredictors that are robust to \emph{exogenous} (non-performative) shifts in the distribution over individuals.

Adapting the notion of universal adaptability, introduced in the context of statistical estimation by \cite{ua}, we show how to learn \emph{univerally-adaptable} performative omnipredictors.
% Lastly, by appropriately augmenting the class of loss functions $\cL$, we can in fact significantly strengthen this omniprediction result.
% Assuming that the conditional distribution over outcomes $\ps$ is invariant, we can efficient learn decision rules which are again optimal for many objectives, but now also remain optimal under \emph{exogenous} (non-performative) shifts in the marginal distribution over individuals.
% We refer to these models as universal omnipredictors in light of the work by \cite{ua} which prove similar results in the context of statistical inference problems. 
% Relative to the previous omniprediction definition,
Whereas performative omnipredictors guarantee optimality on a fixed marginal distribution $\D$ over individuals, 
universally-adaptable omnipredictors give the same optimality guarantee, simultaneously, over a rich class of input distribution shifts $\D_\cW$.
% universally-adaptable omnipredictors have the same guarantee outlined in \equationref{eq:omni_guarantee}, except that this optimality condition now holds, not just for a fixed marginal distribution $\cD$ over individuals, but on a rich class of potential distribution shifts $\D_\cW$.
Each distribution in $\cD_\omega\in \cD_{\cW}$ corresponds to the reweighting of probabilities in $\cD$ by some importance weight function $\omega$ in some pre-specified class $\cW$.
\begin{result}[Informal]
Let $\cL$ be a set of bounded loss functions,  $\cH$ a hypothesis class of decision rules, and let $\cW \subseteq \{\omega: \cX \rightarrow [0,\omax]\}$. 
If the functions in $\cL$, $\cH$, and $\cW$ can be computed by circuits of size $s$, then there exists a predictor $\pt$, computable by a circuit of size at most $\poly(s, |\cYh |) \cdot \omax^2/ \eps^2$, that is a $(\cL,\Hcal,\eps)$-performative omnipredictor for every distribution over individuals $\cD_\omega \in \cD_\cW$.
\end{result}
The result follows by augmenting the class of loss functions $\cL_\cW$ to account for shifts under $\cW$, and again, applying the constructive learning algorithm from Theorem~\ref{result:learning}.
% To efficiently, learn these predictors, we only need to augment the class of loss functions $\cL$ on which we run the POI-boost algorithm by $\cW$.
We emphasize that the learner only needs to account for the class of shifts at \emph{training} time.
At evaluation time, the decision-maker need not know anything about the underlying distribution over individuals.
Indeed, the decision-maker can simply use $\pt$ as before, post-processing to decisions $\ft_\ell(x)$ for any $\ell \in \cL$ on an input-by-input basis.
% have knowledge of what the marginal distribution over individuals might be.
% By guaranteeing robustness to a broad class of distribution shifts, we hope these results empower decision makers to deploy models according to their own objectives which are optimal over their own populations.



% \jcpnote{this last bit on universal adaptability needs more work, not super happy about it}
%        Shifts are specified by a class of importance weights $\cW$, where $\D_\omega$ is reweighted by some $\omega \in \cW$.

%
%adapting a guarantee recently studied in statistical inference problems, we show how to obtain \emph{universally adaptable} omnipredictors.
%        \item Intuitively, UA performative omnipredictors $\pt$ give the omnipredictor guarantee, not just on the original distribution over individuals, but on a rich class of potential distribution shifts.
%        Shifts are specified by a class of importance weights $\cW$, where $\D_\omega$ is reweighted by some $\omega \in \cW$.
 
%  \jcpnote{I'm a bit stuck on how to write this. Will come back}
%\begin{result}
%Omniprediction implies universality for chosen losses approtiately
%\end{result}


% We think of this result as a form of ``computational satisficing'' \cite{simon1956rational}.  The learner is asked to write down, ahead of time,











\subsection{Our Techniques:  Performative Outcome Indistinguishability}
We begin our technical overview with a simple motivating example.
Consider the following performative prediction problem.

\begin{example*}
Let individuals and decisions be encoded as signed booleans $\Xcal = \set{\pm 1}$ and $\Ych = \set{\pm 1}$, assuming $\D$ is uniform over $\Xcal$.
Suppose that Nature's outcome distribution over $\cY = \set{0,1}$ is governed by the conditional probability function
\begin{gather*}
    \ps(x,\yhat) = 1/2 + \beta x \yhat 
\end{gather*}
for any $0 < \beta < 1/2$.
Consider the goal of learning an $(\cL,\Hcal)$-performative omnipredictor for the following collection of losses and hypotheses:
\begin{itemize}
    \item $\cL = \set{\ell_0,\ell_1}$ contains two opposing steering losses, which steer outcomes towards $0$ and $1$, respectively.
    \begin{align*}
        \ell_1(x,\yhat,\ys) = 1-\ys&&\ell_0(x,\yhat,\ys) = \ys
    \end{align*}
    \item $\Hcal = \set{h_+,h_-}$ contains two decision rules over $\Xcal$ that either returns $x$ or its negation.
    \begin{align*}
        h_+(x) = x&& h_-(x) = -x
    \end{align*}
\end{itemize}
\end{example*}

We begin by considering some naive attempts to achieve the goal of performative omniprediction.
Note that $\Hcal$ actually contains an optimal decision rule for each loss in $\cL$.
In particular, for losses that steer to $0$ versus $1$, the optimal decisions minimize (or maximize) the probability that $\ys = 1$.
The decision rule $h_+$ maximizes the probability $\ps(x,h_+(x)) = 1/2 + \beta$ for all $x$, whereas $h_-$ minimizes the probability $\ps(x,h_-(x)) = 1/2-\beta$.
To obtain the omniprediction guarantee, then, we must learn a probability function that encodes the best decision under $\ell_0$ and $\ell_1$.
% it is clear that we cannot simply choose a fixed decision rule:  because they steer in opposite directions, any fixed decision rule will fail to be optimal for at least one of $\ell_0$ or $\ell_1$.

As such, a natural approach would be to fit a function $p:\Xcal \times \Ych \to [0,1]$ that approximates the underlying probability $\ps$, which we can then post-process for a loss $\ell$ as in \equationref{eq:opt_dr} .
To fit $p$, we can simply do supervised learning directly over triples $(x,\yhat,\ys)$, where $\yhat$ is chosen uniformly at random.
We argue that without specification (realizability) assumptions, this approach also fails.
Consider, for instance, fitting $p$ using logistic regression
\begin{align*}
	p(x,\yhat) = \frac{1}{1 + \exp(-(ax + b\yhat + c))},
\end{align*}
where $a,b,c$ are parameters of the model.
In our example, when we select $\yhat$ at random, the outcome $\ys$ is uncorrelated with each of $x$ and $\yhat$ on their own.
Thus, the optimal setting of these parameters is $a = b = c = 0$.\footnote{More concretely, since $\E[x\yhat] = \E[x\ys] = 0$, one can check that $a=b=c=0$ solves the first-order optimality conditions for the logistic regression objective $\E_{x,\yhat, \ys} -[y \log \sigma(ax +b\yhat +c) + (1-y)\log(1- \sigma(ax +b\yhat +c))]$ for $\sigma(z) = 1 / (1 + \exp(-z))$.}
% The relevant model fitting procedure is a convex optimization problem and we can check that $a^* = b^* = c^* = 0$
% solves the standard logistic regression objective. \footnote{More specifically, it solves
% $\argmin_{a,b,c} \E_{x,\yhat, y} \log(1 + \exp(-y(ax + b\yhat +c))).$}
%\end{align*}
% Since all the parameters are 0, we get that
Consequently, the logistic model is a constant: $p(x, \yhat) = 1/2$ for all $x \in \Xcal$ and $\yhat \in \Ych$.
Such constant predictions are completely uninformative. Clearly, they cannot suggest the optimal decision rule for any loss, let alone every loss in our collection.
The negative result here, follows because the model class for $p$ was misspecified to fit $\ps$.
In this example, of course, we simply need to run regression with quadratic terms to be well-specified.
However, without any assumptions about the complexity of $\ps$, we cannot rely on approaches that require specifying Nature's model exactly, which might have unbounded complexity.

% Instead, we turn to methods that involve  $\Hcal$ over different losses encoded in $\cL$.
% For instance, suppose we consider the loss under a decision rule in our class, say $h_+$.
% This decision rule will look great for $\ell_1$, but terrible for $\ell_0$.
% An important observation is that this difference in performance arises because of differences in the underlying outcome probabilities $\ps(x,h_+(x))$.
% That is, the hypotheses and losses in our class provide useful information to \emph{distinguish} between Nature's probabilities and our current model of the probabilities.






% \mpk{
% Example:
% \begin{itemize}
%     \item Simple distribution $x \sim \pm 1$
%     \item (fairly) simple outcome distribution $\ys \sim 1/2 + x\yhat \eps$
%     \item Hypothesis class of decision rules:  $\Hcal = \set{x,-x}$ (really simple!)
%     \item Collection of loss functions:  $\cL = \set{\ys,-\ys}$ (both steering, both simple, but contradictory)
% \end{itemize}
% Zeroth attempt: choose a single optimal decision rule
% \begin{itemize}
%     \item works well for a single loss
%     \item but clearly fails for omniprediction
%     \item obviously a toy example, but point is, direct optimization is doomed to fail
% \end{itemize}
% First attempt:  directly learn an estimate of the probability $p:\Xcal \times \Ych \to [0,1]$
% \begin{itemize}
%     \item may work well under well-specified (realizable) setting
%     \item but we make no assumptions for $\ps$
%     \item For instance, if we use linear/logistic regression to learn over $(x,\yhat,\ys)$ triples, we learn the constant function $p(x,\yhat) = 1/2$
%     \item These predictions give no information, so clearly can't suggest the optimal decision rule
% \end{itemize}
% Observation:  hypotheses and losses give us important information about how to improve our predictions.
% \begin{itemize}
%     \item even though we have no bound on the complexity of $\ps$, we may assume that $\Hcal$ is known and learnable (after all, a hypothesis class)
%     \item for instance, what if we use $h(x) = x$ to make decisions
%     \item this will look really good for $\ell_1$ and bad for $\ell_0$
%     \item but this difference arises because of a difference in the underlying $\ps(x,h(x))$ values
%     \item Intuitively, this is useful information to \emph{distinguish} between our current model and the true Nature.
% \end{itemize}
% }


% Our technical approach towards learning omnipredictions is centered on extending ideas from the outcome indistiguishability literature \cite{oi,gopalan2022personal}. However, 
% having posited the existence of a model of nature $\ps:\cX \times\cYh \rightarrow[0,1]$, one might wonder whether this machinery is really necessary. 
% Perhaps the most natural solution strategy one might consider for the problem is to directly learn $\ps$ via model-fitting and then make decisions while treating this approximation of $\ps$ as if it were the true model. 
% This ``Fit-then-Optimize'' or ``Certainty Equivalence'' approach, however, is very brittle and in general comes with no downstream guarantees of performance.  

% \begin{example}[Limits of Fit-then-Optimize]
% Consider the following simple example. Features, predictions, and outcomes are all binary $\cX = \cYh = \cY = \{\pm 1\}$ and the learner has access to a maximally informative exploratory distribution over $\ps$ where features $x$ and predictions $\yhat$ are both drawn uniformly at random. That is, $x\sim \Unif(\{\pm 1\})$ and $\yhat \sim \Unif(\{\pm 1\})$. Outcomes $\ys$ are performative and drawn from the conditional distribution, $\ps(x, \yhat) =\frac{1}{2} + x\yhat \epsilon$, for some $|\epsilon| < 1/2$. Now, assume we try to learn $\ps$ using standard tools like logistic regression, 
% \begin{align*}
% 	\pt(x,\yhat) = \frac{1}{1 + \exp(-y(ax + b\yhat + c))},
% \end{align*}
% where $(a,b,c)$ are the parameters of the model. The relevant model fitting procedure is a convex optimization problem and we can check that $a^* = b^* = c^* = 0$ solves the standard logistic regression objective. \footnote{More specifically, it solves
% $\argmin_{a,b,c} \E_{x,\yhat, y} \log(1 + \exp(-y(ax + b\yhat +c))).$}
% %\end{align*}
% Since all the parameters are 0, we get that the fitted model $\pt(x, \yhat) = 1/2$ for all $x,\yhat$ and is completely uninformative. Consequently, for any loss $\ell$ that is not constant over its domain, e.g. $\ell(x,\yhat, \ys) = \ys$, choosing predictions according to the induced decision rule
% \begin{align*}
%     f_{\ell,\ptilde}(x) = \argmin_{\yhat \in \cYh} \E_{\yt \sim \pt(x,\yhat)}[\ell(x, \yhat,\yt)] 
% \end{align*}
% has no guarantees of optimality with respect to even a single loss function and the simplest of hypothesis classes $\cH$, e.g. $\cH = \{\sign(x), -\sign(x)\}$. 
% \end{example}

% The key feature of this example is that our guess for the model class for $\pt$ is misspecified.\footnote{
%  The simple logistic regression model does not capture the interaction term $x \yhat$ that leads to $\yhat$ having different performative effects for different individuals. In the model fitting step, these effects ``cancel out'' so that the resulting optimal parameters for the fitted model are uninformative and hence any downstream guarantees are vacuous.}  
%  Hence, any subsequent optimization procedures that involve $\pt$ have no guarantees of performance.  
% %\footnote{If $x=1$, then switching $\yhat$ from -1 to 1 increases the likelihood that $y=1$. On the other hand, if $x=-1$, switching $\yhat$ from -1 to 1 decreases the likelihood that $y$ is positive.} 
% This naive model fitting approach might work if we assume that that nature is \emph{realizable}; that is, $\ps$ is contained in the class of models that we are fitting. 
% However, by assuming realizability, any results that follow would almost certainly scale with the complexity of $\ps$.

% In this work, we approach the problem with a more agnostic learning philosophy. 
% Nature is likely  complicated and learning it exactly seems unlikely. 
% Using the indistinguishability machinery, we can instead opt for a computational approximation which is \emph{efficient}, as well as \emph{sufficient}, for the sake of deriving decision rules with strong optimality guarantees. 


\paragraph{Performative Outcome Indistinguishability.}

% Rather than focusing on direct optimization, we adopt a recent paradigm for learning based on computational indistinguishability.
Recently, \cite{oi} introduced the notion of Outcome Indistinguishability (OI) as a new solution concept for supervised learning.
In contrast to the traditional framing of learning through loss minimization, OI defines the goal of learning through the lens of indistinguishability.
In this view, a predictive model should provide outcomes that cannot be distinguished from true outcomes from Nature.
In the world of supervised learning, OI and the closely-related notion of multicalibration \cite{hkrr} have seen broad application, including in deriving supervised omnipredictors \cite{omni,gopalan2022loss}.
% Originally motivated as a notion of fairness in predicting individual probabilities, OI and the closely related notion of multicalibration \cite{hkrr} have seen broader application across modern prediction problems \cite{omni,ua,jung2021moment}.

Towards our goal of performative omniprediction, we adapt the paradigm of learning via outcome indistinguishability to the outcome performative setting.
In particular, we leverage the variant of outcome indistinguishability explored in a recent work of \cite{gopalan2022loss}.
In the supervised learning setting, \cite{gopalan2022loss} builds a set of indistinguishability conditions called Loss OI, which they show implies omniprediction.
We show that these conditions and the argument are even more general than originally conceived, and can be applied to the outcome performative setting.

Intuitively, we say a predictor $\pt:\Xcal \times \Ych \to [0,1]$ is \emph{performative outcome indistinguishable} if outcomes drawn according to the model $\yt \sim \pt(x,h(x))$ are indistinguishable from Nature's outcomes $\ys \sim \ps(x,h(x))$ \emph{under the distribution induced by a decision rule} $h$.
To make this notion precise, we need to specify what we mean by indistinguishability and pin down the decision rules we care to reason about.

To encode omniprediction through performative OI, our goal will be to devise a set of tests of a predictor $\pt$ that---if passed---guarantee for every loss $\ell \in \cL$, the decision rule $\ft_\ell$ is as good as any $h \in \Hcal$.
Formally, we start by building a class of tests from a collection of losses $\cL$ and a hypothesis class $\Hcal$.\footnote{Throughout, we use the notational shorthand $A \approx_\eps B$ to denote that $A \in [B-\eps,B+\eps]$.}
\begin{definition*}[Performative OI]
For an input distribution $\D$, collection of losses $\cL$, hypothesis class $\Hcal$, and $\epsilon \ge 0$, a predictor $\pt:\Xcal \times \Ych \to [0,1]$ is $(\cL,\Hcal,\epsilon)$-performative outcome indistinguishable (POI) over $\D$ if for all $\ell \in \cL$ and all $h \in \Hcal$,
\begin{gather*}
   \E_{\substack{x \sim \D\\\ys \sim \ps(x,h(x))}}[\ell(x,h(x),\ys)] \approx_\eps  \E_{\substack{x \sim \D\\\yt \sim \pt(x,h(x))}}[\ell(x,h(x),\yt)].
\end{gather*}
\end{definition*}
We emphasize how this performative OI condition is a natural notion of \emph{outcome} indistinguishability.
In particular, we note \emph{where} the predictor $\pt$ occurs in the POI conditions:  it is only used to sample outcomes according to $\pt$ in the modeled world.
Importantly, the decisions $h(x)$ are used in the sampling of $\yt \sim \pt(x,h(x))$.
Using $h(x)$ as the decision associated with $x$ to sample each outcome $y$ (under Nature and the model) ensures that $\pt$ 
% Note that the POI conditions ensure that the outcomes from Nature and the model are sampled conditioned on the decision $h(x)$ specified by the given hypothesis.
% If a predictor $\pt$ satisfies performative OI, then it provides
encodes a reliable estimate of the loss $\ell$ if the decision rule $h$ is deployed.
Performative OI ensures that $\pt$ ``knows'' these values for each loss in the collection $\ell \in \cL$ and each hypothesis in our class $h \in \Hcal$.

While this OI condition ensures that $\pt$ captures the behavior of the hypotheses in $\Hcal$, it says nothing about the losses under its own decision rules $\ft_\ell$.
Reasoning about these decision rules is essential for performative omniprediction.
As such, we introduce an additional OI condition, which we call performative \emph{decision} OI, to ensure OI under the decision rules suggested by $\pt$.
\begin{definition*}[Performative Decision OI]
For an input distribution $\D$, collection of loss functions $\cL$, and $\epsilon \ge 0$, a predictor $\pt:\Xcal \times \Ych \to [0,1]$ is $(\cL,\epsilon)$-performative decision outcome indistinguishable (DOI) over $\D$ if for all $\ell \in \cL$,
\begin{gather*}
    \E_{\substack{x \sim \D\\\ys \sim \ps(x,\ft_\ell(x))}}[\ell(x,\ft_\ell(x),\ys)] \approx_\eps \E_{\substack{x \sim \D\\\yt \sim \pt(x,\ft_\ell(x))}}[\ell(x,\ft_\ell(x),\yt)].
\end{gather*}
\end{definition*}
Here, $\pt$ is still used to sample outcomes $\yt$, but is also used to determine the decision rule $\ft_\ell$, for each $\ell \in \cL$.
Syntactically, changing from $h \in \Hcal$ to $\ft_\ell$ is a small change, but it has significant impacts on the nature of the performative DOI condition---both in terms of its costs and the strength of its guarantees.
Critically, for a given loss $\ell$, the decision rule $\ft_\ell$ is (by definition) optimal for outcomes sampled from $\yt \sim \pt(x,\ft_\ell(x))$.
As such, indistinguishability is a powerful tool here: if the losses are indistinguishable on  modeled outcomes (where $\ft_\ell$ is optimal) and on Nature's outcomes, then $\ft_\ell$ should be optimal for Nature.

We formalize this intuition, demonstrating that, as in the supervised setting, performative OI and decision OI suffice to establish omniprediction.
Consider the loss $\ell \in \cL$ obtained by any $h \in \Hcal$ on true outcomes.
We show that the loss of $\ft_\ell$ is upper bounded by that of $h$.
\begin{proposition*}[Informal]
If a predictor $\pt$ is $(\cL,\Hcal)$-POI and $\cL$-DOI, then $\pt$ is an $(\cL,\Hcal)$-performative omnipredictor.
\end{proposition*}

\noindent\emph{Proof sketch.}~ Once the appropriate OI conditions are written down, deriving performative omniprediction is almost immediate.
\begin{align*}
    \E_{\substack{x \sim \D\\\ys \sim \ps(x,\ft_\ell(x))}}[\ell(x,\ft_\ell(x),\ys)] &\approx \E_{\substack{x \sim \D\\\yt \sim \pt(x,\ft_\ell(x))}}[\ell(x,\ft_\ell(x),\yt)]\\
    &\le \E_{\substack{x \sim \D\\\yt \sim \pt(x,h(x))}}[\ell(x,h(x),\yt)]
    \approx \E_{\substack{x \sim \D\\\ys \sim \ps(x,h(x))}}[\ell(x,h(x),\ys)]
\end{align*}
The first equality follows by $\cL$-DOI, the second equality follows by $(\cL,\cH)$-POI, and the middle inequality follows by the fact that $\ft_\ell$ is optimal over modeled outcomes. \hfill \qedsymbol
\vspace{8pt}

In other words, we have managed to reduce the task of learning performative omnipredictors to learning models satisfying performative OI conditions.
Clearly, Nature's model $\ps$ is ``indistinguishable'' from Nature (similarly, it is clear that $\ps$ is a performative omnipredictor), but the question remains whether there exist \emph{efficient} predictors $\pt$ that satisfy the performative OI conditions.
Thus, we turn our attention to learning OI predictors under outcome performativity.

\paragraph{Learning Outcome Performative Predictors.}
Despite essential differences in the notions of OI in the supervised and performative settings, we show that many of the algorithmic techniques that have become standard in the literature on multicalibration and OI can be adapted to work in the outcome performative setting.
In particular, we demonstrate that, quite generically, learning performative OI models reduces to \emph{auditing} for distinguishability.
Concretely, if there exists a loss $\ell \in \cL$ and hypothesis $h \in \Hcal \cup \set{\ft_\ell}$, such that the performative OI conditions are violated for a predictor $\pt$, we can use these ``distinguishers'' to update the model to address the violation.
This observation immediately suggests using a boosting algorithm, in the vein of \cite{hkrr}, to learn performative OI predictors.
Provided that updating based on an $\eps$-violation makes significant ``progress'' towards satisfying performative OI, then the number of auditing steps $T \le O(1/\eps^2)$ will be bounded.

While this learning paradigm of ``audit, then update'' is intuitive, there are nontrivial challenges in maintaining the efficiency of the learned predictors.
Consider, for instance, the performative decision OI constraint.
As highlighted above, the DOI constraints require that we reason about the optimal decision rule according to $\pt$.
In particular, to update based on a violation of DOI on loss $\ell$, we need to incorporate a copy of the function $\ft_\ell(\cdot)$.
This decision rule, however, is a function of $\pt(\cdot, \yhat)$ for every $\yhat \in \Ych$ (as it requires computing the argmin over $\Ych$).
Naively, then, it would seem that in every iteration where we update the model based on some $\ft_\ell$, we need to make $\card{\Ych}$ recursive oracle calls to the existing model.
Without careful consideration, the \cite{hkrr}-style learning algorithm will build a performative OI predictor $\pt$ whose complexity $s$ scales \emph{exponentially} in the number of iterations, $s \ge \card{\Ych}^T$.

To avoid this blow-up, we need to choose a more effective representation of the probability function $\pt(\cdot, \cdot)$.
We observe that, in general, the updates required for the algorithm are \emph{sparse} in $\Ych$.
As a result of this sparsity, we can save on overall computation by implementing $\pt:\Xcal \times \Ych \to [0,1]$ as a map from individuals to vectors of probabilities $\tilde{q}:\Xcal \to [0,1]^\Ych$.
Mathematically, there is a bijection between such functions; computationally, however, the representations behave very differently.
By increasing the amount of work per update by a factor of $\card{\Ych}$, we avoid making $\card{\Ych}$ recursive calls.
This strategy is reminiscent of an approach \cite{dwork2022beyond} used to learn (supervised) OI predictors for outcomes living in a large domain.
With this representation in place, an appropriate analysis reveals that the resulting predictors can be implemented in complexity that scales only \emph{polynomially} in the number of iterations and decisions.


% \mpk{While this framework is nice and obvious in a sense, there are some challenges.
% In particular, there is a question of how to represent prediction functions in a way that obtains efficient omnipredicotrs.
% Consider for instance the Decision OI conditiosn.
% As highlighted above, the constraints require taht we reason about (and encode implicitly) the optimal decision rule $\ft_\ell(\cdot)$.
% This decision rule is a function of $\pt(\cdot, \yhat)$ for every $\yhat \in \Ych$.
% Naively, then, it would seem that in every iteration of boosting, we might need to make $\card{\Ych}$ calls to our current model.
% Using this approach would lead to an \emph{exponential} growth in the circuit size in the number of iterations $\ge \card{\Ych}^T$.
% }



After addressing representation issues, we study sufficient conditions to implement the auditing task efficiently, from a polynomially bounded number of samples.
Achieving performative optimality, in general, requires exploration of the consequence of using different decision rules $h \in \Hcal$, as these decision rules effect the distribution on outcomes.
Nevertheless, we show that it suffices for this exploration to be done ``offline'' via randomized assignment of decisions $\yhat \in \Ych$.
In particular, if we collect triples $\set{(x,\yhat,\ys)}$ through a randomized control trial, assigning $\yhat$ uniformly at random for each $x \in \Xcal$, and observing $\ys \sim \ps(x,\yhat)$, we avoid the need to deploy each $h \in \Hcal$.

Given access to such RCT data, we give a reduction from the task of auditing for performative OI to the task of \emph{supervised learning} for the hypothesis class $\Hcal$.
This reduction from auditing to learning is familiar in the OI framework \cite{hkrr,oi}, but critically, we go from a performative prediction task to a non-performative task.
In all, our reductions show that if we can learn the best decision rule from $\Hcal$ in a supervised learning setting, then we can learn performative omnipredictors with respect to $\Hcal$, assuming access to appropriately sampled data.



\paragraph{Universal Adaptability under Outcome Performativity.}
The OI viewpoint enables a similarly straightforward analysis of distributional robustness, via universal adaptability.
Universal adaptability is a notion introduced by \cite{ua} in the context of statistical estimation.
In the original context, a predictor is universally adaptable if it provides an efficient way to estimate statistics across many underlying input distributions.

We translate the notion of universal adaptability to the outcome performative prediction setting.
In our context, we parameterize universal adaptability by a class of importance weight functions $\cW \subseteq \set{\Xcal \to \R_{\ge 0}}$.
For a base input distribution $\D$, we define a corresponding collection of shifted distributions $\D_{\cW}$ to be the set of distributions reachable after reweighting by some $\omega \in \cW$.
\begin{gather*}
    \D_{\cW} = \set{\D_\omega : \omega \in \cW, \supp(\D_\omega) \subseteq \supp(\cD)}  \text{ and } \forall x \in \supp(\D_\omega):~~ \D_\omega(x) = \omega(x) \cdot \D(x) 
\end{gather*}
The key observation is that for any hypothesis $h$, loss function $\ell$, and importance weight function $\omega$, the expected loss over $\D_\omega$ is equal to an expected loss over $\D$, for a loss defined in terms of $\ell$ and $\omega$. \begin{align*}
	\E_{\substack{ x\sim \cD_{\omega} \\ \yt \sim \pt(x, h(x))}} [\ell(x, h(x), \yt)] = \E_{\substack{ x\sim \cD \\ \yt \sim \pt(x, h(x))}} [\ell(x, h(x), \yt) \cdot \omega(x)]
\end{align*} 
Importantly, this equality relies on the fact that 
the outcome probability functions $\ps$ and $\pt$ are defined conditional on $x$ and $\yhat$, and thus are invariant across shifts in the input distribution.
% the expected performative risk of a model $\pt$ averaged over a distribution of individuals $\cD_{\omega}$, is exactly equal to the expected risk of $(h, \ell \cdot \omega)$ averaged over the distribution $\cD$:

Using the result that indistinguishability implies omniprediction, by simply enforcing that $\pt$ satisfy the POI and DOI conditions relative to $\ps$ under this enriched class of loss functions $\ell \cdot \omega$, we can neatly ensure that $\pt$ is again POI and DOI, not just over $\cD$, but over every marginal distribution $\cD_\omega$. Consequently, $\pt$ must a be an omnipredictor under all of these $\cD_\omega$. The simplicity of this analysis attests to the versatility of the OI perspective and the value it provides in domains beyond supervised learning. 
%Further exploring the consequences of OI in other domains is an exciting direction for future work.



















% Instead, we turn to methods that involve  $\Hcal$ over different losses encoded in $\cL$.
% For instance, suppose we consider the loss under a decision rule in our class, say $h_+$.
% This decision rule will look great for $\ell_1$, but terrible for $\ell_0$.
% An important observation is that this difference in performance arises because of differences in the underlying outcome probabilities $\ps(x,h_+(x))$.
% That is, the hypotheses and losses in our class provide useful information to \emph{distinguish} between Nature's probabilities and our current model of the probabilities.
% Our technical approach towards learning omnipredictions is centered on extending ideas from the outcome indistiguishability literature \cite{oi,gopalan2022personal}.



% In particular, our technical approach towards learning omnipredictors is centered on achieving the following two indistinguishability definitions.





% On the other hand, Performative Decision OI states that $\pt$ must be indistinguishable from $\ps$ across all losses $\cL$, even if we act upon the predictions of our model. 
% In light of the shortcomings of the ``Fit-then-Optimize'' example, this definition directly anticipate the fact that we will eventually use the model $\pt$ as part of an optimization problem. It asks that we remain indistinguishable from nature, even if we act on the basis of this optimization procedure. 

% Both of these definitions are efficiently achievable, if two simple conditions holds. The first condition is a necessary statistical requirement that the learner have access to an appropriate ``exploratory'' distribution over pairs $(x,\yhat)$. Since predictions $\yhat$ impact outcomes $\ys$, if the learner only has samples from a distribution where every individual is assigned the same prediction $\yhat_1$, there is no hope to derive guarantees of optimality with respect to decision rules that assign a different prediction $\yhat_2$ to a nontrivial subset of the population. In this work, we assume that the learner has access to ``RCT''-style data where predictions $\yhat$ are made uniformly at random for every individual $x$. \footnote{However, similar results go through if $\yhat$ are not drawn for the uniform distribution, but from any distribution that places nontrivial mass on every element in $\cYh$.} 

% The second condition is computational in nature. We assume that the learner has access to an algorithm that can efficiently solve basic, well-studied supervised learning primitives, like cost-sensitive classification. Importantly, neither one of these assumptions says anything about nature being ``simple'' or low complexity. Our guarantees hold regardless of the strength of performative effects and without regard to the complexity of $\ps$.

% Under these conditions, we can learn predictors $\pt$ which satisfy both of the indistiguishability conditions above, with sample and runtime complexity that only depend on the richness of functions in $\cL$ and $\cH$. We believe that one of the key strengths of our approach is that it enables a particularly clean analysis of omniprediction. Inspired by concurrent work on omniprediction in the supervised learning setting \cite{gopalan2022personal}, the proof that any POI and DOI predictor is also an omnipredictor take 3 lines. \jcpnote{may add proof depending on space, but don't think it's necessary.}







%We think of these definitions of ``computational satisficing'' \cite{simon1956rational} in which we write down, ahead of time, a contract. This contract specifies a list of test functions, in this case defined in terms of losses $\ell$ and decision rules $h$, for which we want our model $\pt$ to be indistinguishable with respect to nature's model $\ps$. 
%The analogy to satisficing comes in because these definitions are: 1) efficiently computable and 2) sufficient for the sake of deriving omnipredictors. 













% Performative Optimality:
% \begin{itemize}
%     \item We show how to obtain performative optimality efficiently, under plausible (and necessary) settings
%     \mpk{NOTE:  even the \emph{existence} of such predictors (in such an efficient construction) is very surprising.  Also, NOTE: the predictor complexity does not depend on any distributional assumptions.}
%     \item We assume that performativity occurs in the \emph{outcomes}, but that units (i.e. individuals' features) are fixed
%     \item \textbf{Theorem:}  Under outcome performativity, there is a sample-efficient algorithm that learns a performatively optimal decision rule, and time-efficient given an oracle for supervised learning.
%     \item \textbf{Proposition:}  Without these assumptions, impossible to obtain sample efficiency (let alone time) \mpk{true?}
% \end{itemize}

% Omniprediction:
% \begin{itemize}
%     \item One-shot approach to learning is especially desirable under performativity:  any changes you make to the predictions themselves may change the distribution over outcomes
%     \item Concept recently introduced in supervised learning literature:  omnipredictor
%     \item Motivates a new abstraction for predictors:
%     \begin{itemize}
%         \item learn a single predictor that allows clients to explore different predictions and policies (for forecasting or steering)
%         \item Predictor must take in decision as an input!
%         \item Pretty fundamentally different abstraction than what has been studied in performativity thus far
%     \end{itemize}
%     \item \textbf{Definition:}  Performative Omnipredictor---optimal policy for a given loss dervied from an omnipredictor is performatively optimal
%     \item \textbf{Theorem:}  There exists an efficient algo for learning performative omnipredictors.  (Again, reduction to supervised learning.)
% \end{itemize}

% Performative Outcome Indistinguishability:
% \begin{itemize}
%     \item Our results go through the OI learning paradigm
%     \item Idea:  learn a predictive model that mimics the behavior of Nature.
%     \item OI is an effective abstraction for performative prediction:
%     \begin{itemize}
%         \item explicitly account for the ``behavior'' under a certain decision $\yhat$.  That is, our predictive model takes the same ``inputs'' as Nature's model (including decision)
%         \item focus our attention on losses that may be relevant for prediction, but also for steering
%     \end{itemize}
%     \item In supervised learning world, there's a tight connection between OI and calibration.  In performative world, we see that it's not as simple.
% \end{itemize}



\subsection{Related Work and Discussion}

Our work lies at the intersection of several areas including performative prediction, the outcome indistinguishability  and multicalibration literature, as well as other fields studying algorithmic decision-making such as contextual bandits. We briefly discuss how our results relate to previous work within these areas and conclude with some speculation regarding broader implications of our conclusions.

\paragraph{Performative Prediction.} The performative prediction framework was introduced by \cite{performative} who defined the main solution concepts and analyzed the convergence of repeated risk minimization to \emph{performatively stable} points. A decision rule $h_{\mathrm{ps}}$ is performatively stable if it is a fixed point of risk minimization,
\begin{align*}
	h_{\mathrm{ps}} \in \argmin_{h \in \cH}\E_{(x,\ys)\sim \cD(h_{\mathrm{ps}})} [\ell(x, h(x), \ys)].
\end{align*}
Subsequent work by \cite{mendler2020stochastic,drusvyatskiy2022stochastic,brown2022performative,cutler2021stochastic}
studied stochastic optimization algorithms for finding stable points in a variety of settings. 
However, these stable solutions need not be performatively \emph{optimal} as per the definition outlined in \equationref{eq:po}. 
In fact, \cite{miller2021outside} proved that performatively stable models can achieve \emph{arbitrarily worse} loss than performative optimal points.
This observation motivated the design of algorithms for findings performatively optimal decision rules for a fixed loss $\ell$\cite{miller2021outside,izzo2021learn,izzo2022learn,narang2022multiplayer,jagadeesan22a}. 
These algorithms work in the general performative prediction setup where
% the deployment of 
the model $h$ can affect the \emph{joint} distribution over pairs $(x,y)$, but make make very strong specification assumptions on how each $h$ influences the distribution, and restrict to loss functions satisfying smoothness and strong convexity.
% In particular, they generally assume that the data generating process is parametrized by a linear function of the decision rule's parameters that has small norm.
% Furthermore, they generally impose strict regularity conditions on the loss $\ell$ (e.g. smoothness \& strong convexity).
% On the other hand, we place very mild restrictions on the loss function (e.g boundedness) and no restriction on the impact of predictions on the distribution, other than the outcome performativity assumption.

In contrast, our results rely only on the outcome performativity assumption and mild boundedness assumptions.
The recent  work of \cite{mendler2022predicting} has also considered the outcome performativity setting, aiming to understand when performative effects are identifiable from observational data.
Short of identifiability, it remains an interesting direction for future research to give learning algorithms for performative omnipredictors from observational data.
% We note that a similar outcome performativity assumption is also used by \cite{mendler2022predicting} as a means of understanding when performative effects are identifiable based off observational data.
% Unlike this line of work, we find a single decision rule that is optimal for a wide variety of losses. We make no assumptions regarding how predictions influence outcomes, other than the condition that they only influence outcomes,  not the distribution over individuals $x$.

Beyond these optimization results, previous work in performative prediction has acknowledged
% that the goals of prediction can extend past accurate forecasting.
the tension in performative prediction between accurate forecasting and steering.
Concretely, \cite{miller2021outside} discuss how the choice of loss function in performative prediction should balance predictive accuracy with any externalities that arise from the impacts of prediction on the observed distribution.
In a different direction, \cite{hardt2022performative} uses performativity as a lens with which to study notions of market power in economics.
As part of their analysis, they provide a decomposition of the performative risk of a classifier into terms that represent forecasting and steering.
While we consider how the choice of loss function determines the high-level objective, \cite{hardt2022performative} considers how, even for a fixed loss function, the performative risk can be decomposed into terms associated with forecasting and steering.
% In light of these previous results, our work directly tries to address the tension between forecasting and steering by developing solution concepts and algorithmic tools that allow decision-makers to choose from a variety of possible objectives.




\paragraph{Reinforcement Learning and Contextual Bandits.} As discussed in \cite{performative}, performative prediction, and in particular outcome performativity, can be cast as reinforcement learning (RL) or contextual bandits problems. 
Individuals $x$ correspond to the contexts, decisions $\yhat$ correspond to actions, and the loss $\ell(x,\yhat, \ys)$ is captured by the reward $r(x,\yhat)$.
Due to the breadth of their definitions, most ML problems can be written as RL problems. 
% However, by adopting such a general perspective, we loose sight of many of the rich details which make performative prediction an valuable framework to study social prediction problems. 

Still, important issues that arise in outcome performativity---like the tension between forecasting and steering and the desire for omnipredictors---are best seen by focusing on the specific interactions between predictions $\yhat$ and outcomes $y$.
The variety of losses that can exist for a given outcome are obscured by encapsulating all feedback within an abstract reward function $r(x,\yhat)$.
Moreover, on a technical level, performativity has a richer feedback structure that can be used to design more efficient algorithms as illustrated by \cite{jagadeesan22a}.

% \jcpnote{for michael?}
\paragraph{Multicalibration and  Outcome Indistinguishability.}
Originally developed by \cite{hkrr} as a notion of fairness in prediction, multicalibration has seen considerable interest and application in the broader context of supervised learning.
At a high-level, multicalibration requires predictions to be \emph{calibrated}, not just overall, but even when restricting our attention to structured subpopulations.
The goal of multicalibration and other related notions of ``multi-group'' fairness \cite{kearns2018preventing,kim2018fairness,kim2019multiaccuracy,jung2021moment} is to ensure that learning occurs within important subpopulations that might otherwise be ignored.

Intuitively, the requirements of multicalibration represent a kind of indistinguishability:  calibration requires that the predicted probabilities ``look like'' real probabilities.
\cite{oi} formalizes this intuition, introducing the notion of Outcome Indistinguishability, which generalizes multicalibration.
They show tight computational equivalences between multi-group fairness notions and variants of OI.
Subsequently, OI and multicalibration have been applied in diverse contexts beyond fairness, such as distributional robustness through universal adaptability \cite{ua} and omniprediction \cite{omni}.

\paragraph{Omniprediction.}
Our work draws directly from the work on omnipredictors \cite{omni,gopalan2022loss}.
Even in the supervised learning setting, the existence of efficient omnipredictors is not at all obvious.
The main result of \cite{omni} demonstrates the feasibility of omnipredictors over any hypothesis class $\Hcal$, for the class $\cL_\mathrm{cvx}$ of all convex and Lipschitz loss functions.
This sweeping result follows by showing that a $\Hcal$-multicalibrated predictor is a $(\cL_\mathrm{cvx},\Hcal)$-omnipredictor.

A key follow-up work of \cite{gopalan2022loss} shows that omniprediction is even more general than initially thought.
This work initiates the study of omniprediction through the lens of outcome indistinguishability.
By the equivalence of OI with multicalibration, it has been clear since the work of \cite{omni} that OI captures loss minimization and omniprediction in the context of supervised learning, albeit indirectly.
\cite{gopalan2022loss} revisits the question of omnipredictors, directly through the lens of OI, studying a refined notion, which they call Loss OI.
They derive a general recipe for omnipredictors for any class of losses $\cL$, from calibration and multiaccuracy over a class derived from $\cL$ and $\Hcal$.

On a technical level, our analysis follows the OI-based approach of \cite{gopalan2022loss}.
Indeed, our proof that Performative OI and Performative Decision OI imply Performative Omniprediction follows the strategy laid out to obtain supervised omnipredictors from Loss OI.
Despite the fact that outcome performativity requires us to reason about distributional shifts induced by the predictions, the same indistinguishability framework proves effective for learning omnipredictors in our setting.

While syntactically similar to prior formulations of OI, our notion of performative OI is the first to consider outcome indistinguishability for non-supervised learning distributions.
Our objective, in this work, was to derive a notion of performative OI sufficient to imply performative omniprediction.
No doubt, further generalizations of the original OI hierarchy \cite{oi} to the (outcome) performative setting---and beyond---may prove useful.


% But is the definition too strong?
% Do efficient omnipredictors exist or does omniprediction require learning $\ps$?






% OI:  \cite{oi}.
% \mpk{later, cite \cite{dwork2022beyond} to say that we had to deal with something similar there to contend with large outcome domain.}

% Comes out of the literature on MC:
% \cite{hkrr}

% These notions have been generalized beyond their original formulations (follow up \cite{dwork2022beyond}, moment multicalibration \cite{jung2021moment}, confidence intervals \cite{gupta2022online}, low-degree MC \cite{gopalan2022low})
% But all of these work in a standard supervised or online learning setting.


% \paragraph{A ``boring'' paradigm for learning.}

% Outcome indistinguishability begins to look like a ``proof system'' for learning.
% \begin{itemize}
%     \item Define your favorite property $\Pi$
%     \item Prove that the optimal predictor $\ps$ satisfies $\Pi$
%     \item Determine tests $\mathcal{T}$ required to ``fool'' the proof
%     \item Learn a predictor $\pt$ that is $\mathcal{T}$-outcome indistinguishable
% \end{itemize}
% If the proof can't distinguish between $\ps$ and $\pt$, then $\pt$ must satisfy property $\Pi$.
% This work pushes OI beyond it's original formulation in significant ways.
% Shows that this paradigm of learning is more general than the standard agnostic supervised learning setup, in which it has been applied successfully.


% While syntactically similar to prior formulations of OI, our notion of performative OI is the first to consider outcome indistinguishability for non-supervised learning distributions.
% Our objective, in this work, was to derive a notion of performative OI sufficient to imply performative omniprediction.
% No doubt, further generalizations of the original OI hierarchy \cite{oi} to the (outcome) performative setting---and beyond---may prove useful.
% % Concretely, consider the role of hypotheses $h \in \Hcal$.
% % In the supervised setting, hypotheses are used to distinguish the conditional distribution on $\ys \vert x$ from $\yt \vert x$.
% % In the performative setting, the choice of decision $h(x) = \yhat$ also influences the outcome distribution.


% Many of the algorithmic and analytic techniques we employ are familiar from prior works.
% The formulaic nature of applying the OI machinery at times feels repetitive, but also feels in line with Barak's measure of scientific success (``when we eliminate the need for creativity and make boring what was once exciting'') \cite{barak}.
% Our work gives further credence to the idea of OI as a learning paradigm that can be effective at modeling exciting modern learning desiderata.
% % From its original formulation as a fairness notion, to distributional robustness, now to performativity, it's the right abstraction for many problems.





\subsection*{Organization}
The remainder of the manuscript is organized as follows.
% In Section~\ref{sec:prelims} we set up outcome performativity formally and establish notation used throughout the manuscript.
In Section~\ref{sec:omni}, we define performative omniprediction and performative outcome indistinguishability.
Here, we show how appropriate performative OI conditions suffice to obtain omniprediction.
In Section~\ref{sec:ua}, we establish the universal adaptability properties of performative omnipredictors.
In Section~\ref{sec:learning}, we give a generic learning algorithm for performative omnipredictors, demonstrating concrete instantiations of the algorithm using randomized control trial data.
Finally, in Section~\ref{sec:calibration}, we discuss notions of multicalibration in the context of performative prediction.
We speculate that some notions translate to the performative setting naturally, yielding efficient approaches to performative OI, while other notions seem to resist efficient translation.


\subsection*{Notation Overview}
We denote individual's features by $x \in \cX$ and
the available decisions by $\yhat \in \cYh$.
We assume that $\cX$ and $\cYh$ are discrete sets, and assume $\card{\cYh}$ is finite.
Throughout our presentation, we assume that outcomes $\cY = \set{0,1}$ are binary. The true conditional expectation over Nature's outcomes is given by $$\ps: \cX \times \cYh \rightarrow [0,1],$$
where for every individual $x \in \Xcal$ and decision $\yhat \in \Ych$, $\ps(x,\yhat)$ gives the true probability of positive outcome.
$$\ps(x,\yhat) = \Pr[\ys=1\mid x, \yhat]$$
In analogy to $\ps$, we denote the learner's predictor (i.e., the ``model of Nature'') by
$$\pt:\cX \times \cYh \rightarrow [0,1].$$
We use the shorthand $\ys \sim \ps(x,\yhat)$ to denote true outcomes drawn from the Bernoulli distribution with parameter $\ps(x,\yhat)$,
and $\yt \sim \pt(x,\yhat)$ to represent modeled outcomes drawn from the Bernoulli distribution with parameter $\pt(x,\yhat)$.
Throughout, we use $\cD$ to denote a marginal distribution over individual features $x \in \cX$.
To denote the approximate equality of expectations, we use the notational shorthand $A \approx_\eps B$ to denote that $A \in [B-\eps,B+\eps]$.

We take a loss function to be a map from individual-decision-outcome triples to a nonnegative value,
$$\ell:\cX \times \cYh \times \cY \rightarrow \R_{\geq 0}.$$
For a collection of losses $\cL$, we let $\lmax = \sup_{x,\yhat,y} \ell(x,\yhat,y)$.
For a fixed loss $\ell$, we define $\ft_{\ell}: \cX \to \cYh$ to be the optimal post-processing of $\pt$ according to $\ell$. 
More specifically, for every $x \in \cX$,
\begin{align*}
    \ft_{\ell}(x) = \argmin_{\yhat \in \cYh} \E_{\yt \sim p(x,\yhat)}[\ell(x, \yhat,\yt)].
\end{align*}
Note that $\ft_{\ell}$ is defined pointwise, without regard to the marginal distribution over $\cX$.
We use $\cH \subseteq \set{h:\Xcal \to \cYh}$ to represent a set of decision rules (i.e., a hypothesis class) which map individuals to decisions.
Typically, we assume that hypotheses $h \in \Hcal$ have an efficient representation. 

%\mpk{Move this part to the section on UA}
%We use $\cW$ to represent a set of importance weight functions $\omega:\cX \rightarrow \R_{\geq 0}$.
%Again we use $\omax = \sup_{x,\omega} \omega(x)$. 


  


 
% \clearpage
 
 
 
 
 
 
 



==> arxiv 2/learning.tex <==
\section{Learning Algorithms for Performative Omniprediction}
\label{sec:learning}

\begin{figure}[t!]
\setlength{\fboxsep}{2mm}
\begin{boxedminipage}{\textwidth}
\begin{center}
{\centering{\underline{Performative OI Boost (POI-Boost)}}}
\end{center}

\vspace{2mm}
{\bf Input:} Set of losses $\cL$, hypotheses $\cH$, distribution $\cD$, tolerance $\eps > 0$\\
\vspace{-2mm}

{\bf Initialize:} $q^{(1)}(\cdot) \gets [1/2, \dots, 1/2] \in [0,1]^{|\cYh|}$  
%\mpk{notation? establish that  you model $p:\Xcal \to [0,1]^{\Ych}$ as a way to implement $\pt(x,\yhat)$.  Maybe even call the learned mapping $q$?} 
\\

{\bf For} $t = 1,2, \ldots$
\begin{itemize}
	\item {\bf If:} there exists $\mathbf{a)}$  $(h,\ell) \in \cH \times \cL$ \quad or,  \quad   $\mathbf{b)}$ $(h, \ell) \in  \{(f_{\ell, t}, \ell): \ell \in \cL \}$
%	\begin{itemize}
%	\item[a)] $(h,\ell) \in \cH \times \cL$  \null\hfill POI
%	\item[b)] or $(h, \ell) \in  \{(f_{\ell, t}, \ell): \ell \in \cL \}$
%	\end{itemize}
%	\quad \quad  such that:
	\begin{align}
	\equationlabel{eq:constraint}
		| \underbrace{\E_{\substack{x \sim \cD \\ \yt \sim \pt(x, h(x))}}[\ell(x, h(x),\yt)] - \E_{\substack{x \sim \cD \\ \ys \sim \ps(x, h(x))}}[ \ell(x, h(x),\ys)]}_{\mathsf{err}_t} | \geq \eps
	\end{align}
	
	
	{\bf Then:} Update the representation $q^{(t)}$: 
	\begin{align}
	\label{eq:predictor_update_rule}
		q^{(t+1)}(\cdot) \leftarrow \Pi \left(\; q^{(t)}(\cdot) - \eta^{(t)} \; v_{\ell, h}(\cdot) \;\right)
	\end{align}
	where $\eta_t = - \epsilon\cdot \sign(\mathsf{err}_t) \; / \; \lmax$ and 
	\begin{align}
	\equationlabel{eq:gradient_def}
	v_{\ell, h}(\cdot) =	 \begin{bmatrix}
	 (\ell(\cdot, \yhat_1, 1) - \ell(\cdot, \yhat_1, 0))  \;\ind\{h(\cdot) = \yhat_1 \}\\ 
	 \dots  \\
	 (\ell(\cdot, \yhat_k, 1) - \ell(\cdot, \yhat_k, 0)) \; \ind\{h(\cdot) = \yhat_k \}
	 \end{bmatrix}\in \R^{|\cYh|},\quad  \cYh = \{\yhat_1, \dots, \yhat_k\}
	\end{align}

	\item {\bf Else:} terminate and return the function $\pt(x,\yhat) = q^{(t)}(x)[\;\yhat\;]$
\end{itemize}
\vspace*{2mm}
\end{boxedminipage}

\caption{Algorithm for generating performative omnipredictors. 
The algorithm proceeds by repeatedly verifying whether the intermediate predictors $p^{(t)}$ satisfy the POI definition, outlined in $\mathbf{a)}$, as well as the DOI definition, outlined in $\mathbf{b)}$. 
If neither is violated, the procedure terminates. 
Otherwise, the algorithm implicitly updates the representation $q^{(t)}$ of the predictor $p^{(t)}$. Given an input $x$, $q^{(t)}(x)$ is a vector of length $|\cYh|$ whose $\yhat$ entry, $q^{(t)}(x)[\;\yhat\;]$, represents $p^{(t)}(x,\yhat)$. 
The operator $\Pi$ clips entries of its input vector to lie in $[0,1]$. 
%The key insight is that we can build the circuit that computes $\pt$ without explicitly updating every entry $(x,\yhat)$ during training time, while still being able to efficiently compute all outputs at evaluation time. 
For the sake of clarity, here we present the simplest version of the algorithm where the search outlined in \equationref{eq:constraint} is proper, however this condition can be easily relaxed as discussed in \sectionref{subsec:csc}.}
\figurelabel{fig:algorithm} 
\end{figure}

%Having introduced performative OI definition, its variants, and how they lead to omniprediction and universality, we now focus on the statistical and computational complexities of learning models $\pt$ which are performatively indistinguishable.




%Our goal is to establish bounds the statistical and computational complexity of achieving omniprediction for general classes of losses $\cL$ and hypothesis $\cH$. Later on, we examine special cases where more efficient approaches are possible and discuss connections between outcome performativity and multicalibration. 


In this section, we introduce a general purpose algorithm, POI-Boost, which provably returns a performative omnipredictor $\pt$ for any class of hypothesis $\cH$ and collection of losses $\cL$.
Our algorithmic approach is centered on establishing two reductions. First, we prove that, similar to previous work in the OI literature, learning Performative OI predictors reduces to the problem of \emph{auditing} for outcome indistinguishability.

The auditing problems we reduce to involve determining whether the losses under the decision rules in $\Hcal$ and $\set{\ft_\ell}$ are the same for Nature's outcomes and our modeled outcomes \emph{under outcome performativity}.
% Defining these auditing problems, however, requires special care relative to previous analyses of these boosting-style algorithms for supervised learning problems.
While in the supervised learning setting we only need to reason about a single outcome distribution, in our setting, 
% there is only a single distribution that needs to be learned,
% at least naively, in performative prediction there are many.
different different decision rules induce different distributions over outcomes, and we want to audit for indistinguishability over each of these induced distributions.
Despite this challenge, we show that, given access to appropriately randomized data, we can reduce this performative auditing problem to standard supervised learning primitives.
In this second reduction, we make use of computational and statistical assumptions:  access to an appropriate supervised learner (computational) and access to randomized control data (statistical).
% Hence, we a prove a second reduction.
% We show that auditing for test functions that exhibit differences between $\ps$ and $\pt$ somewhat surprisingly also reduces to basic and well-studied supervised learning primitives.
% However, this computational reduction hinges on the necessary, statistical assumption that the learner has access to an appropriate exploratory distribution.

While we instantiate our algorithm with specific computational and statistical assumptions, the framework for learning is completely generic and modular.
In particular, any solution to the auditing problem can be used to implement the algorithm.
It stands to reason that our assumptions could be relaxed in the future, or that in certain settings, incomparable assumptions lead to more effective auditing, which in turn would lead to more efficient learning of performative omnipredictors.

\subsection{Reducing Indistinguishability to Auditing}

We start by establishing our first reduction. We prove that the POI-Boost algorithm (\figureref{fig:algorithm}) returns a performative omnipredictor $\pt$ after a small, polynomial number of calls to an auditing subroutine (described in \equationref{eq:constraint} \& \figureref{figure:auditing}), without yet describing the runtime or sample complexity of the auditing step itself. We address these questions in the next subsection. The algorithm works for any outcome performative problem where the number of predicted labels $\cYh$ is finite and the loss functions are bounded.

\paragraph{Representing Predictors.} For the sake of our analysis, it is helpful to distinguish between the predictor $\pt:\cX \times \cYh \rightarrow [0,1]$ as a function, and the implementation of $\pt$ in code. 
In our learning algorithm, we represent the function $\pt$ in terms of vector-valued functions $\qt: \cX \rightarrow [0,1]^{|\cYh|}$.
Given $x \in \cX$, $\qt(x)$ is a vector of length $|\cYh|$ whose $\yhat$ entry, $q^{(t)}(x)[\;\yhat\;]$, represents $\pt(x,\yhat)$. 

Of course, there is a correspondence between these functions $\pt$ and $\qt$ where each $\pt$ leads to a unique $\qt$ and vice versa. 
The key difference is that $\qt(x)$ returns $\pt(x,\yhat)$ for all $\yhat \in \Ych$ in a single function call, while computing the same information using the direct $\pt$ representation would require $|\cYh|$ functions calls. 
While this might seem like a minor detail, these representations have meaningful differences in terms of the circuit complexity of performative omnipredictors.
Crucially, for any loss $\ell$, to compute $\ft_\ell(x)$, we need the value of of $\pt(x,\yhat)$ for all $\yhat \in \Ych$, and this computation can be performed using a single call to $\qt$.
In other words, we perform $\card{\Ych}$ times the work per call to $\qt$ to avoid $\card{\Ych}$ \emph{recursive} calls to the predictor within the construction.
Avoiding further calls to these functions avoids branching factors and an exponential blowup in the complexity of the resulting predictors as we illustrate.



%[Here, we describe the bijection between $\pt$ space and $\tilde{q}$ space.
%Highlight, specifically, how this enables efficient, direct computation of $\ft_\ell$.
%]

\paragraph{Algorithm Description.} As outlined in \figureref{fig:algorithm}, POI-Boost is an iterative algorithm which nonparametrically constructs a predictor $\pt$, represented in terms of a vector-valued function $\qt$, by stringing together copies of circuits which compute losses $\ell$ and decision rules $h$. 
At each iteration, the algorithm first appeals to auditing subroutines to check if there: is $a)$ a pair $h,l$ for which the current predictor $p^{(t)}$, fails the performative OI guarantee, or $b)$ a loss function $\ell$ for which the decision rule $f_{\ell,t}$ fails the decision OI guarantee. 
If neither condition is violated, then the algorithm terminates since $p^{(t)}$ satisfies both indistinguishability conditions and consequently must be an omnipredictor as per \theoremref{thm:omni}.

On the other hand, if one of these conditions is violated, we perform an update to the representation $q^{(t)}$ of the current predictor $p^{(t)}$. These updates nudge the predictor closer to $\ps$ by essentially performing gradient descent in function space \cite{mason1999boosting}. These updates are done implicitly in the sense that we can update the representation $q^{(t)}$ for all $x$ in $\cX$ simultaneously by simply adding a copy of the circuit computing $v_{\ell,h}: \cX \rightarrow \R^{|\cYh|}$ (\equationref{eq:gradient_def}) which is defined in terms of a loss $\ell$ and decision rule $h$. By bounding the total number of updates via a potential argument, we can ensure that we don't add too many copies of these functions so that the final predictor is computationally efficient. 
%We now make this intuition formal.


%nonparametrically constructs a predictor $\pt$ by repeatedly calling the auditing subroutine to find  test functions, defined in terms of losses $\ell$ and decision rules $h$, for which the expected performative risk between $\pt$ and $\ps$ is significantly different. 
%Using these test functions, we can iteratively . 
%At each update step, we add a copy of a circuit computing the function returned by the auditing step to the overall program that computes $\pt$. 
%Intuitively, whenever we can find a violation, these updates bring us closer to the true model $\ps$. If no violation is found, then we've found a good enough approximation. 


\begin{proposition}
\proplabel{prop:iteration_bound}
The POI-Boost algorithm described in Figure 1 terminates in at most $   |\cYh|  \lmax^2 / \eps^2$ many iterations and returns a predictor $\pt$ that is
$(\cL, \cH, \epsilon)$-performative OI and $(\cL, \epsilon)$-performative decision OI. Consequently, $\pt$ is a $(\cL, \cH, 2\epsilon)$-performative omnipredictor.
\end{proposition}
\begin{proof}
%Throughout the proof we will repeatedly switch between referring to the predictors $p^{(t)}:\cX \times \cYh \rightarrow [0,1]$ and their representations as vectors, $q^{(t)}: \cX \rightarrow [0,1]^{|\cYh|}$, such $p^{(t)}(x,\yhat) = q^{(t)}(x)[\yhat]$.

The guarantee that $\pt$ is performative decision OI and performative OI follow directly from the termination criterion. Therefore, the proposition follows from proving that this termination criteria is met within the stated number of iterations. 

%Here, $q^{(t)}(x) \in [0,1]^{|\cYh|}$ is the vector representation of $p^{(t)}$ such that $p^{(t)}(x,\yhat) = q^{(t)}(x)[\yhat]$ where the bracket notation indicates the $\yhat$ entry of the vector $q^{(t)}(x)$. Likewise, we can write $\ps(x,\yhat) = q^*(x)[\yhat]$ where again $q^*(x)$ is a vector of length $|\cYh|$ with entries in $[0,1]$.  

 
The key insight is that if the indistinguishability constraint in \equationref{eq:constraint} is violated for any $\ell$ or $h$, then updating the representation $q^{(t)}$ ensures that we will have made nontrivial progress on a common potential function. 
Since this potential is bounded from above and below, and we make nontrivial progress with every update, the total number of updates must be bounded. 
In more detail, first, note that for any model $p$, loss $\ell$, hypothesis $h$, and $\cY=\{0,1\}$:
\begin{align*}
	\E_{\substack{x \sim \D\\ y \sim p(x,h(x))}} [\ell(x, h(x), y)] &= \E_{x} \E_{y\mid x} [\ell(x, h(x), y)] \\
	&= \E_{x}[\ell(x, h(x),0) + \left(\ell(x, h(x), 1) - \ell(x, h(x), 0)\right) \cdot p(x,h(x))].
\end{align*}
From this rewriting, and the definition of  $v_{\ell, h}$ in \equationref{eq:gradient_def}, the difference in performative risks between the predictors $p^{(t)}$ and $\ps$ for a pair $\ell, h$ can be expanded as,
\begin{align}
	\E_{\substack{x \sim \D\\ y_t \sim p^{(t)}(x,h(x))}} [\ell(x, h(x), y_t)] - \E_{\substack{x \sim \D\\ \ys \sim \ps(x,h(x))}} [\ell(x, h(x), \ys)]
 =\E_x \langle q^{(t)}(x)- q^*(x),\; v_{\ell,h}(x) \rangle.
	\equationlabel{eq:test_func_diff}
\end{align}

Now consider the potential, written in terms of the representations $q^{(t)}$, $\E_x \norm{q^{(t+1)}(x) - q^*(x)}^2$. By definition of the update rule in the algorithm, this potential is equal to:
\begin{align*}
 	 \E_x \norm{\Pi \left(q^{(t)}(x)   - \eta^{(t)} v_{\ell, h}(x)  \right) -
 q^*(x)}^2.
 \end{align*}
Because the projection (or clipping) operator $\Pi$ can only decrease the distance to $\ps$, if an update is performed, the difference between potentials at adjacent time steps, 
\begin{align*}
 \E_x \norm{q^{(t+1)}(x) - q^*(x)}^2 - \E_x \norm{q^{(t)}(x) - q^*(x)}^2,
\end{align*}
is upper bounded by the sum of  two terms,
% where $v_{\ell, h}$ is defined in \equationref{eq:gradient_def}
\begin{align*}
 &-2 \eta_t \E_x\langle q^{(t)}(x)- q^*(x), v_{\ell, h}(x)\rangle  + \eta_t^2 \E_{x} \norm{v_{\ell, h}(x)}^2.
 \end{align*}
 Using the identity from \equationref{eq:test_func_diff} and the definition of $v_{\ell, h}$ from \equationref{eq:gradient_def}, this is equal to:
 \begin{align*} 
 & -2 \eta_t \mathsf{err}_t + \eta_t^2 \E_{x} [(\ell(x, h(x),1) - \ell(x,h(x),0))^2].
\end{align*}
Because losses lie in $[0,\lmax]$, the second term is less than $\lmax^2\eta_t^2$. 
Furthermore, from the auditing guarantee, $|\mathsf{err}_t| > \epsilon$. By setting the step size $\eta^{(t)}$ to be $-\eps \cdot \sign(\mathsf{err}_t) \; / \; \lmax$, we conclude that the difference in potentials across adjacent time steps satisfies,
\begin{align*}
2 \eta_t \mathsf{err}_t + \eta_t^2 \E_{x} [(\ell(x, h(x),1) - \ell(x,h(x),0))^2] \leq 	-2\eta_t \mathsf{err}_t + \eta_t^2 \lmax^2 \leq -\eps^2 /\lmax^2.
\end{align*}
Since the potential is nonnegative and bounded above by $|\cYh|$, the maximum number of iterations until the termination criterion is met must be at most $|\cYh| \lmax^2 / \eps^2$.
\end{proof}

An important consequence of this result is that it reveals the existence of omnipredictors $\pt$ that admit computationally efficient approximations. 
This result is subtle, even in light of previous work on OI-style boosting algorithms. Intuitively, the final $\pt$ is built out by stringing together copies of functions in $\cH$, $\cL$, and decision rules $f_{\ell,t}$.
Because these decision rules $f_{\ell,t}$ are defined in terms of an optimization procedure involving the intermediate constructions $p^{(t)}$, which themselves depend on previous models $p^{(t-1)}$, a naive implementation of $\pt$ can result in a recursion that induces an exponentially large circuit.
Specifically, the naive implementation would make $\card{\Ych}$ recursive calls to the prior circuit in order to compute $f_{\ell,t}$, resulting in a growth rate of $\card{\Ych}^t$.

However, by carefully ordering the relevant computations and 
``caching'' previous work, we avoid this blow-up.   
The key insight is the following.
By designing a circuit that computes the value of $\pt(x,\yhat)$ for every $\yhat \in \Ych$ simultaneously, we can avoid recursive calls to the circuit.
By maintaining the intermediate computations of $q^{(t)}$, we can avoid a branching factor in the program and preserve efficiency.




% Note that the hypothesis $h^{(t)}$ could belong to the set $\{f_{\ell, t}: \ell \in \cL \}$. Because these decision rules $f_{\ell, t}$ themselves depend on the predictor $p^{(t)}$, and its representation $q^{(t)}$,we need to be careful in how we compute these vectors in order to avoid an exponential blowup in program complexity.
%\mpk{Perhaps have two different cases in the auditing, rather than auditing for $h \in \Hcal \cup \set{f_\ell}$}

%\mpk{Also, for this analysis, having a different notation for $\pt:\Xcal \times \Ych \to [0,1]$ and the function you're building up mapping $q:\Xcal \to [0,1]^\Ych$ would be helpful.}








%Note that $\pt$ is a circuit that consists of $\lmax^2 |\cY| |\cYh| / \eps^2$ many copies of functions in $\cL$ and decision rules in $\cH \cup \{f_{\ell, t}: \ell \in \cL \}$. Therefore, the runtime and memory requirements of $\pt$ are at most a polynomial factor larger than those of the functions in these sets. If these functions are efficiently computable, then so is $\pt$,

\begin{theorem}
\theoremlabel{theorem:circuit_size}
Assume that the functions in $\cH$ and $\cL$ are computable by circuits of size at most $s$, then the predictor $\pt$  returned by the POI-Boost algorithm has size at most $\lmax^2 /\eps^2 \cdot \poly(s, |\cYh|)$.
\end{theorem}
\begin{proof}
The final predictor consists of a summation of the initial prediction, followed by the update from each iteration.
We bound the growth of the circuit computing the predictor by induction.
Formally, let $S_t$ be the circuit size for computing $q^{(t)}$.
Then, we show that $S_{t+1}\leq S_t + \poly(|\cYh|, s)$ for all $t\geq 1$.
Thus, by the overall bound on the iteration complexity, the final predictor can be implemented using a circuit of size $S \le \lmax^2 /\eps^2 \cdot \poly(s, |\cYh|)$.
To begin, the initial constant predictor $q^{(1)}$ can be implemented using a circuit of size at most $S_1 = \card{\Ych} \le  \poly(s,\card{\Ych})$ by hard-coding the constant vector.

By the update rule, each update incorporates a function of the form,
\begin{align}
\equationlabel{eq:intermediate_functions}
g^{(t)}(x) \defeq\eta^{(t)} v^{(t)}_{\ell, h}(x) =	 \eta^{(t)}\begin{bmatrix}
	 (\ell^{(t)}(x, \yhat_1, 1) - \ell^{(t)}(x, \yhat_1, 0))  \;\ind\{h^{(t)}(x) = \yhat_1 \}\\ 
	 \dots  \\
	 (\ell^{(t)}(x, \yhat_k, 1) - \ell^{(t)}(x, \yhat_k, 0)) \; \ind\{h^{(t)}(x) = \yhat_k \}
	 \end{bmatrix}\in \R^{|\cYh|},
\end{align}
where $\ell^{(t)}$ and $h^{(t)}$ define the test function surfaced by the auditing subroutine at time step $t$.
Within these updates, the function $h^{(t)}$ may \emph{a}) come from $\Hcal$ due to a POI violation or \emph{b}) equal $f_{\ell,t}$ for some $\ell \in \cL$ due to a DOI violation.

In the first case where $h^{(t+1)} \in \cH$, $q^{(t+1)}(x)$ can be computed by evaluating evaluating $q^{(t)}(x)$, and then evaluating $h(x)$ and $\ell(x,\yhat, y)$, for every $\yhat$ and $y$.
By assumption, the latter operations require circuits of size at most $\poly(s, |\cYh|)$.
Paired with the inductive hypothesis, the resulting circuit size can be bounded as $S_{t+1} \le S_t + \poly(s,\card{\Ych}) \le (t+1) \cdot \poly(s,\card{\Ych})$.

For the second case, 
we recall the definition of $f_{\ell,t}(\cdot)$, we can express its computation as a minimization over $\Ych$ of expected losses that depend on $q^{(t)}(\cdot)[\yhat]$ for each $\yhat \in \Ych$.
\begin{align*}
	f_{\ell,t}(x) = \argmin_{\yhat \in \Ych}\ \set{\ell(x, \yhat,0) + \left(\ell(x, \yhat, 1) - \ell(x, \yhat, 0)\right) \cdot q^{(t)}(x)[\yhat]}.
\end{align*}
Importantly, to compute each term in the minimization, we only need to compute the vector $q^{(t)}(x)$ once.
% This is the key point.
The remaining terms, $\ell(x, \yhat, 0)$ and $\ell(x, \yhat, 1)$ (for every $\yhat$), can again be  computed by a circuit of size $\poly(|\cYh|, s)$.
Since the minimization itself can be done by linearly enumerating over $\cYh$, we again preserve the invariant that $S_{t+1} \leq S_t + \poly(|\cYh|, s)$.
\end{proof}




\subsection{Reducing Auditing to Supervised Learning}
\sectionlabel{subsec:csc}

\begin{figure}[t]
\setlength{\fboxsep}{2mm}
\begin{boxedminipage}{\textwidth}
\begin{center}
\underline{$\mathrm{Audit}(\cH, \cL, \pt, \eps)$}
\end{center}
\vspace{2mm}
\textbf{If:} there exists $(h,\ell) \in \cH \times \cL $
	\begin{align*}
		   \big|  \E_{\substack{x \sim \cD \\ \yt \sim \pt(x,h(x))}}\ell(x, h(x),\yt) - \E_{\substack{x \sim \cD \\ \ys \sim \ps(x,h(x))}}\ell(x, h(x),\ys) \big| \geq \eps
	\end{align*}
\textbf{Then:} return  $h,l$  \\

\textbf{Else:} return $\mathsf{False} $
\end{boxedminipage}
\caption{The key auditing step in the POI-Boost algorithm. In each iteration of the algorithm, we run two auditing steps: once to check for the POI condition over $\cH \times \cL$ and once to check for the DOI condition over $\{(f_{\ell, t}, \ell): \ell \in \cL \}$. See the proof of  ~\corollaryref{cor:end} for further discussion.}
\figurelabel{figure:auditing}
\end{figure}

Having shown how omniprediction reduces to an auditing problem, we now complete our analysis of the POI-Boost algorithm by showing that auditing itself reduces to cost-sensitive classification over a single, static distribution. In doing so, we address the statistical and computational complexity of solving this auditing step.

%Unlike supervised learning, in performative prediction one needs to engage in active exploration in order to find good decision rules. For example, a dataset in which every individual $x$ receives the same prediction $\yhat_1$ provides no information about what the outcomes $y$ would look like if we choose a decision rule that assigns predictions $\yhat_2$ for a nontrivial subset of the population.

From examining the auditing condition in \figureref{figure:auditing}, perhaps the most obvious strategy is to choose a decision rule $h$, and to collect a dataset of triples $(x, \yhat, \ys)$ where $\yhat=h(x)$ for every $x$ and $\ys \sim \ps(x, h(x))$. If the loss $\ell$ is bounded, a standard application of Hoeffding's inequality shows that empirical risk of the loss concentrates around its expectation:
\begin{align*}
	 \frac{1}{n}\sum_{i=1}^n \ell(x_i, h(x_i), \ys_i) \approx\E_{\substack{x \sim \D\\ \ys \sim \ps(x,h(x))}} [\ell(x, h(x), y_*)].  
\end{align*} 
Therefore, one could implement the auditing step by enumerating over all $h$, deploying $h$ to collect a new dataset every time, and then nonadaptively computing the empirical performative risk of $h$ on every $\ell \in \cL$. This procedure would however require $\tilde{\cO}(|\cH|/\eps^2 \log |\cL|)$ many samples. 

On the other hand, if we have access to randomized predictions $\yhat$, we can estimate the empirical risk of every pair $h, \ell$ off of a \emph{single} distribution by using inverse propensity scoring. The following lemma is  well-known within various communities, and, in particular, the contextual bandits literature (see e.g. \cite{monster,dudik2011}).\footnote{This result can be generalized to the case where for every $x$, $\yhat \sim q(x)$ for some known distribution $q$, where $q\neq \Unif(\cYh)$ but where $q$ has full support over $\cYh$.}

We use the shorthand $(x,\yhat,y) \sim \D_\mathrm{rct}$ to denote the sampling process where inputs are sampled from the base distribution $x \sim \D$, decisions $\yhat$ are assigned uniformly at random, $\yhat\sim \Unif(\cYh)$, and the outcomes are sampled according to Nature's model $\ys \sim \ps(x,\yhat)$.

\begin{lemma}
\lemmalabel{lemma:ip_weighting}
Assume that $\calYhat$ is a finite set. Then, for any hypothesis $h:\cX \rightarrow \cYh$, 
\begin{align*}
\E_{\substack{x \sim \calD_x \\ \ys \sim \ps(x,h(x))}} [\ell(x, h(x), \ys) ]= |\calYhat| \cdot \E_{(x,\yhat, \ys) \sim \rct} [\ell(x, \yhat, \ys )\ind \{h(x) = \yhat\}].
\end{align*}	
\end{lemma}

\begin{proof}
We present the proof for the case where $\calYhat = \{0,1\}$ is binary, but the general case follows the same pattern. We expand out the left hand side as:
\begin{align*}
\E_{\substack{x \sim \calD \\ \ys \sim \ps(x,h(x))}} [\ell(x, h(x), \ys)] & = \E_{\substack{x \sim \calD \\ \ys_{(1)} \sim \ps(x,1), \ys_{(0)} \sim \ps(x,0)}} \left[\ell(x, 1, \ys_{(1)}) \ind\{h(x) = 1\} +  \ell(x, 0, \ys_{(0)}) \ind\{h(x) = 0\} \right]\\
& = \E_{\substack{x \sim \calD \\ \ys_{(1)} \sim \ps(x,1)}} \left[\ell(x, 1, \ys_{(1)}) \ind\{h(x) = 1\} \right] + \E_{\substack{x \sim \calD \\ \ys_{(0)} \sim \ps(x,0)}} \left[\ell(x, 1, \ys_{(0)}) \ind\{h(x) = 0\} \right].
\end{align*}
Reweighting the term on the right hand side, we observe our desired equality:
\begin{align*}
 \E_{\substack{x \sim \calD \\ \yhat \sim \Ber(1/2) \\ \ys \sim \ps(x,\yhat)}} \left[ \ell(x, \yhat, \ys )\ind\{h(x) = \yhat\} \right]&= \frac{1}{2}\E_{\substack{x \sim \calD \\ \ys_{(1)} \sim \ps(x,1)}} \left[\ell(x,1, \ys_{(1)}) \ind\{h(x) = 1\} \right] \\
 &+ \frac{1}{2} \E_{\substack{x \sim \calD \\ \ys_{(0)} \sim \ps(x,0)}} \left[\ell(x,1, \ys_{(0)}) \ind\{h(x) = 0\} \right]. 
\end{align*} 
\end{proof}



There are two main takeaways from this lemma. First, it shows that the statistical complexity of auditing can be exponentially better than the the naive strategy outlined previously.
\begin{corollary}
\corollarylabel{corollary:concentration}
Let $\{(x_i, \yhat_i, \yt_i)\}_{i=1}^n$ be a dataset of $n$ i.i.d samples from $\rct$. If $$n\geq \frac{2\lmax^2 |\cYh|^2 \cdot \log(2|\cH| |\cL| / \delta)}{\eps^2},$$ then with probability $1-\delta$,
\begin{align*}
\max_{h \in \cH,\ell \in \cL} \big|\E_{\substack{x \sim \calD \\ \ys \sim \ps(x,h(x))}} [\ell(x, h(x), \ys)]  - \frac{1}{n} \sum_{i=1}^n |\calYhat| \cdot  \ell(x_i, \yhat_i, \ys_i )\ind \{h(x_i) = \yhat_i\}  \big| \leq \eps.
\end{align*}
\end{corollary} 
 \begin{proof}
From the previous lemma, we have that for any loss $\ell$ and decision rule $h$, 
\begin{align*}
\E_{\substack{x \sim \calD \\ \ys \sim \ps(x,h(x))}} [\ell(x, h(x), \ys)] = |\calYhat|\cdot \E_{(x,\yhat, \ys) \sim \rct} [\ell(x, \yhat, \ys )\ind \{h(x) = \yhat\}].
\end{align*}	 
Because $|\calYhat| \cdot \ell(x_i, \yhat_i, \ys_i )\ind \{h(x_i) = \yhat_i\}$ is uniformly bounded by $\lmax |\cYh|$, we can apply Hoeffding's inequality to argue that the probability that the empirical estimate is far from the true expectation
\begin{align*}
\big|\E_{\substack{x \sim \calD \\ \ys \sim \ps(x,h(x))}} [\ell(x, h(x), \ys)]  - \frac{1}{n} \sum_{i=1}^n |\calYhat| \cdot  \ell(x_i, \yhat_i, \ys_i )\ind \{h(x_i) = \yhat_i\}  \big| > \epsilon
\end{align*}
is bounded as $2\exp\left(\frac{2\eps^2}{n (\lmax \card{\Ych})^2}\right)$.
% get that if $n \geq 2 \lmax^2 |\cYh|^2 / \epsilon^2 \log(2/\delta)$ with probability $1-\delta$, 
The result follows by rearranging for failure probability $\delta$, and taking a union bound over all $h \in \cH$ and $\ell \in \cL$.
%The proof follows directly from the previous lemma and Hoeffding's inequality.
 \end{proof}

Consequently, for a single iteration of the POI-Boost algorithm, the auditing step can be implemented by enumerating over all $\cL$ and $\cH$ and non-adaptively evaluating their empirical risks on a single dataset of size $\tilde{\cO}(\lmax^2 |\cYh|^2 / \eps^2 \log(|\cH| |\cL| ))$.\footnote{An analogous result applies if we replace $\ps$ by $\pt$, which we assume that the learner can easily sample from.} 
Typically, we think of $|\cYh|$ as a small constant and the class of decision rules $\cH$ as a rich collection. From this result, we see that at least statistically, we can hope to design omnipredictors that are optimal with respect to an exponential number of losses and decision rules.

Here, we present the simplest possible analysis of this result and state our bounds for finite classes $\cH$ and $\cL$. It is certainly feasible to achieve sharper results and to state bounds in terms of VC-dimension or other sharper notions of statistical complexity. 
However, the goal of our initial work on outcome performativity is not to establish the tightest bounds, but to provide a broad overview of what is possible. 
We hope future work will provide a precise understanding of the sample complexity of omniprediction in outcome performativity. 

The following proposition summarizes the sample complexity of omniprediction if the auditing steps for the POI and DOI conditions are implemented via a naive learner that linearly enumerates over all $h,\ell$ and evaluates their empirical risk on a single dataset of RCT samples.

\begin{proposition}
\propositionlabel{prop:sc_summary}
Given labeled data $(x, \yhat, \ys) \sim \rct$ drawn from Nature and unlabeled samples $x \sim \cD$, the POI-boost can be implemented using at most: 
\begin{itemize}
	\item $\cO(\lmax^2 |\cYh|^2 \log(\frac{|\cH||\cL|}{\delta}) / \epsilon^2 + \lmax^4 |\cYh|^3 \log(\frac{|\cL| \lmax |\cYh|}{\delta \epsilon}) /\epsilon^4 )$ labeled samples
	\item $\cO(\lmax^4 |\cYh|^3 \log(\frac{|\cH||\cL| \lmax |\cYh|}{\delta \epsilon}) / \epsilon^4)$ unlabeled samples
\end{itemize}
\end{proposition}

\begin{proof}
In each iteration of the POI-boost algorithm, we need to audit for the POI and DOI guarantees (conditions $a$ and $b$). We can implement each of the auditing steps by explicit enumeration. 

For POI, at each iteration $t$ we enumerate over $\cH$ and $\cL$ and evaluate the empirical counterparts of 
\begin{align}
\equationlabel{eq:two_expectations}
\E_{\substack{x \sim \cD \\ \yt \sim p^{(t)}(x,h(x))}}[\ell(x, h(x),\yt)] \quad \text{ and } \E_{\substack{x \sim \cD \\ \ys \sim \ps(x,h(x))}}[\ell(x, h(x),\ys)].
\end{align}
By \corollaryref{corollary:concentration}, the empirical versions of these quantities concentrate around their expectations. To get an $\eps$ approximation, with probability $1-\delta$, we require at most $\cO(\lmax^2 |\cYh|^2 \log(|\cH||\cL| / \delta) / \epsilon^2)$ many samples. At each iteration $t$,  the expectation on the left changes, since we update $p^{(t)}$. However, to evaluate this expectation we only need \emph{unlabeled} samples, since labels $\yt$ come from our own model $p^{(t)}$. On the other hand, the expectation on the right in \equationref{eq:two_expectations} does not depend on $t$, so we need not recompute it at every iteration. Because the total number of iterations is bounded by $\lmax^2 |\cYh| / \epsilon^2$, applying a union bound on $\delta$, to achieve the POI guarantee we only need a total of $\cO(\lmax^4 |\cYh|^3 \log(|\cH||\cL| \lmax |\cYh| \epsilon^{-1} \delta^{-1}) / \epsilon^4)$ unlabeled samples and $\cO(\lmax^2 |\cYh| \log(|\cH||\cL| / \delta) / \epsilon^2)$ labeled samples.

For the DOI guarantee outline in condition $b$, we instead need to approximate 
\begin{align}
\equationlabel{eq:doi_two_equations}
\E_{\substack{x \sim \D\\\yt \sim p^{(t)}(x,f_{\ell,t}(x))}}[\ell(x,f_{\ell,t}(x),\yt)]	\quad \text{ and } \E_{\substack{x \sim \D\\\ys \sim \ps(x,f_{\ell,t}(x))}}[\ell(x,f_{\ell,t}(x),\ys)].
\end{align}
Note that both of these expectations now depend on $t$, because the decision rules $f_{\ell,t}$ can change between iterations. Again, by \corollaryref{corollary:concentration}, if we enumerate over all $|\cL|$ losses and decision rules $f_{\ell,t}$ at each iteration, the empirical counterparts of these expressions on a dataset of size $\cO(\lmax^2 |\cYh|^2 \log(|\cL|/\delta) /\epsilon^2)$ concentrates. Collecting a new dataset at every iteration, we get that the total number of labeled (and unlabeled) samples is bounded by $\cO(\lmax^4 |\cYh|^3 \log(|\cL| |\cYh| \lmax \delta^{-1} \epsilon^{-1}) /\epsilon^4)$.
\end{proof}


\paragraph{Cost-Sensitive Classification.} The second main takeaway from \lemmaref{lemma:ip_weighting} is that auditing can now be rewritten as as the solution to a cost-sensitive multiclass classification problem over $|\cYh|$ many classes. This result completes our analysis showing how omniprediction can be reduced to basic supervised learning problems. 

In light of previous results, the main benefit of this reduction is that it enabled the design of oracle-efficient algorithms which can be faster than the naive learner used in \propositionref{prop:sc_summary}. We start by first defining what we mean by cost-sensitive classification.

\begin{definition}
\definitionlabel{definition:csc}
Let $\cX$ be a feature space, $\cYh$ be a finite set of $k$ classes, and $\cD$ be a distribution over $\cX \times [-1,1]^k$. For $(x,c) \sim \cD$, we say that $c$ is a cost vector whose entries $c(\yhat)$ denote the costs of predicting label $\yhat$ on feature $x$. An algorithm $\cscalg$ is an $\rho$-cost-sensitive  learner for a hypothesis class $\cH$ if for any distribution $\cD$ over $\cX \times [-1,1]^{k}$, promised that there exists $h \in \cH$ such that $\E_{(x,c) \sim \cD} c(h(x)) \leq -\rho$, $\cscalg$ returns a hypothesis $h'$ such that $\E_{(x,c) \sim \cD} c(h'(x)) \leq -\rho/2 $.
\end{definition}

Cost-sensitive classification is a well-studied supervised learning problem for which many, both passive and active learning algorithms, have been designed \cite{beygelzimer2009error,abe2004iterative,langford2005sensitive, krishnamurthy2017active,elkan2001foundations}. 
There are a number of software packages that can be used to solve applied cost-senstive classification problems \cite{catboost}. 
Like many problems in computational learning theory, cost-sensitive classification is known to be hard in the worst-case, but can be solved effectively in practice.
As such, our goal is to design \emph{oracle-efficient} learning algorithms, that make an small number of calls to cost-sensitive learner.
% \jcpnote{\@ michael can edit, don't want to make a mistake about agnostic learning.}
% However, there are special cases where learning can be computationally efficient. Furthermore,


Here, we frame a ``weak'' version of the problem where the learning need not be exact, but where the search is proper, in the sense that $\cscalg$ returns a hypothesis in $\cH$. This latter condition can easily also be relaxed without changing the overall results. However, we opt to keep it as is for the sake of simplifying the presentation.
The following proposition completes our reduction of auditing to supervised learning. 

\begin{proposition}
\proplabel{prop:csc_auditing}
Let $\cscalg$ be a cost-sensitive learner as per \definitionref{definition:csc}. Then, given access to RCT samples $(x, \yhat, \ys) \sim \rct$, we can solve the auditing problem outlined in \figureref{figure:auditing} using $2|\cL|$ many calls to $\cscalg$ with parameters $\rho  = \eps / (4\lmax |\cYh|)$.
\end{proposition}

\begin{proof}
By \lemmaref{lemma:ip_weighting} we have that the difference in performative risk between $\ps$ and $\pt$,
\begin{align*}
	  \E_{\substack{x \sim \cD \\ \yt \sim \pt(x,h(x))}}[\ell(x, h(x),\yt)] - \E_{\substack{x \sim \cD \\ \ys \sim \ps(x,h(x))}}[\ell(x, h(x),\ys)],
\end{align*}
is equal to:
\begin{align*}
|\cYh| \cdot \E_{\substack{x \sim \calD \\ \yhat \sim \Unif(\calYhat) \\ \yt \sim \pt(x, \yhat) ,\ys \sim \ps(x,\yhat)}} \left[\ind \{h(x) =\yhat\}(\ell(x, h(x),\yt) - \ell(x, h(x),\ys))\right].
\end{align*}
Now, we note that terms inside the expectation can be written as entries in a cost vector $c$ where for every sample $(x,\yhat, \ys, \yt)$ we define the corresponding vector $c$ to be, 
\begin{align*}
	c_{\sigma}(h(x)) = \begin{cases}
		\sigma\cdot (\ell(x, h(x),\yt) - \ell(x, h(x),\ys)) &\text{ if } h(x) = \yhat \\ 
		0 &\text{ o.w}
	\end{cases},
\end{align*}
Here, $\sigma \in \{\pm 1\}$
and we set $\sigma=1$ to get the desired equality. Hence, for a fixed loss $\ell$, we can transform RCT samples, $x\sim \cD, \yhat \sim \unif(\cYh), \ys \sim \ps(x,\yhat)$ to a cost sensitive classification problem such that for every $h \in \cH$, 
\begin{align*}
\E_{\substack{x \sim \cD'}} [c_{+1}(h(x))]  = |\cYh| \E_{\substack{x \sim \calD \\ \yhat \sim \Unif(\calYhat) \\ \yt \sim \pt(x, \yhat) ,\ys \sim \ps(x,\yhat)}} [\ind \{h(x) =\yhat\}(\ell(x, h(x),\yt) - \ell(x, h(x),\ys))].
\end{align*}
To solve the auditing problem outlined in \figureref{figure:auditing}, we need to check whether the absolute value of the difference is larger than $\epsilon$. To do this, it therefore to suffices to run $\cscalg$ twice (once with $\sigma=1$ and once with $\sigma=-1$) for every loss $\ell \in \cL$ to check if there exists a decision rule $h \in \cH$ such that:
\begin{align*}
	\E_{\substack{x \sim \cD'}} [c_{+1}(h(x))] \leq -\eps \text{ or } \E_{\substack{x \sim \cD'}} [c_{-1}(h(x))] \leq -\eps.
\end{align*}
Because we normalize the cost vectors to have entries in $[-1,1]$ in \definitionref{definition:csc}, we can scale the vectors $c_\sigma$ by $1/ (4|\cYh|\lmax)$ and divide the tolerance parameter $\eps$ by the corresponding amount to match the desired interface.
\end{proof}

\subsection{End-to-End Analysis}

Having now presented these reductions showing how omniprediction can be reduced to cost sensitive classification, we now summarize our results so far and establish end-to-end bounds on the runtime and sample complexities of achieving omniprediction. 

% \jcpnote{technically the runtime depends on the complexity of the functions $h$ and $\ell$?}
\begin{corollary}
\corollarylabel{cor:end}
Assume that $h \in \Hcal$ and $\ell \in \cL$ can be evaluated in time $\poly(\log(|\cH|))$ and $\poly(\log(|\cL|))$, respectively.
Let $\cscalg$ be a $\rho$-cost-sensitive weak learner for $\cH$ as per \definitionref{definition:csc}.
Assume that for any distribution $\cD_{\mathrm{csc}}$ over pairs $(x,c) \in \cX \times [-1,1]^k$, $\cscalg$ runs in time $\poly(\log(|\cH|), 1/\rho)$ and uses at most $\poly(\log(|\cH|), 1 / \rho)$ many samples drawn from $\cD_{\mathrm{csc}}$.\footnote{Here, we have avoided discussion on the failure probability parameter $\delta$ for the $\cscalg$. However, it is clear that the relevant complexity bounds should depend only on $\log(1/\delta)$ and that applying a simple union bound would not change the nature of the resulting analysis. We therefore assume that the algorithms succeed with probability 1 for the sake of simplicity.}
If the learner has access to samples drawn according $(x,\yhat, \ys) \sim \rct$, then, the POI-Boost algorithm:
\begin{itemize}
	\item runs in time $\mathcal{O}\left(|\cL| \cdot \poly\left(1/\eps,\; \lmax, \;|\cYh|, \;\log|\cL|,\;\log|\cH|\right) \right) $
	\item uses at most $\cO\left( \poly\left(1/\eps, \;\lmax, \;|\cYh|,\;\log|\cL|,\; \log|\cH|\right)\right)$ many samples
\end{itemize}
\end{corollary}
\begin{proof}
To bound the runtime, we note that by \propref{prop:iteration_bound}, the maximum number of iterations for POI-Boost is at most $\lmax^2 |\cYh| / \eps^2$. In each iteration, we solve the auditing via two subroutines. One to check for the POI guarantee (condition $a$ in \figureref{fig:algorithm}) and another routine to check the DOI guarantee (condition $b$ in \figureref{fig:algorithm}).
To audit for the POI guarantee, we call the cost-sensitive learner $2|\cL|$ times with parameters $\rho  = \eps / (4\lmax |\cYh|)$ as per \propref{prop:csc_auditing}, using labels derived from calculating each $\ell \in \cL$ and evaluating $p^{(t)}(x,\yhat)$ in at most $\poly(\log(\card{\cL})) + \poly(\log(\card{\cH}),1/\eps,\lmax,\card{\Ych})$ time. With the labels calculated, each of these calls has run time and sample complexity at most $\poly(\log(|\cH|, 1/\epsilon, \lmax, |\cYh|))$.


To audit for the DOI guarantee over the $(h,\ell) \in \{(f_{\ell,t}, \ell): \ell \in \cL\}$, at each iteration, we use the naive strategy outlined in \sectionref{subsec:csc} where we enumerate over all $|\cL|$ losses and evaluate the performative risk of each pair $(f_{\ell,t}, \ell)$ on a single dataset of RCT samples of size $\cO(\lmax^2  / \eps^2 |\cYh|^2 \log(|\cL|))$ as per \corollaryref{corollary:concentration}. Each auditing step for DOI therefore runs in time $|\cL| \cdot \poly(1/\epsilon, \lmax, |\cYh|)$ and uses $\poly(1/\epsilon, \lmax, |\cYh|, \log(|\cL|))$ many samples. All calls to the intermediate predictors $p^{(t)}$ also run in polynomial time as per \theoremref{theorem:circuit_size}. The final guarantees come from multiplying the sample and run time complexity of each iteration of the POI-boost algorithm by the bound on the total number of iterations.
\end{proof}

The main take away from this result is that if the cost-sensitive classification problem can be solved efficiently, in the sense that the the relevant statistical and computational complexities scale as $\polylog|\cH|$, then the overall POI-Boost algorithm runs in time linear in $|\cL|$, poly-logarithmically in the size of $\cH$ and with at most $\polylog |\cH| |\cL|$ many samples. Therefore, we can hope to develop efficient omnipredictors that are optimal for exponentially many decision rules, and polynomially many losses.

Note that, because of the result outlined in \propref{prop:adaptability},  this theorem also bounds the statistical and computational complexity of achieving universally adaptable omnipredictors. 
More specifically, the number of samples and the runtime for achieving universally adaptable omnipredictors are also bounded by the quantities in \corollaryref{cor:end} where we now replace the class $\cL$ by augment collection $\cL_\Wcal$ as defined in \propref{prop:adaptability}. The main difference is that the relevant runtime and sample complexity bounds replace dependence on $|\cL|$ by dependence on $|\cL||\cW|$ and replace dependence on $\lmax$ by $\lmax \omax$. Here, $\omax$ is the the worst case density ratio for the class $\cW$.
\begin{align*}
	   \max_{\omega \in \cW} \max_{x \in \supp(\D_\omega)}  \omega(x) = \frac{\D_\omega(x)}{\D(x)}.
\end{align*}
This complexity measure capture the intuition that if individuals $x$ are poorly represented over the distribution $\cD$ we are learning over, then we need more samples (and consequently runtime), to learn universally adaptable omnipredictors. 
We think of these complexity parameters like $\omax$ as a first step. It is an interesting question for future work to provide sharper notions of problem complexity and to find ways of designing omnipredictors for exponentially large collections of importance weights $\cW$. 


























==> arxiv 2/macros.tex <==
\newcommand\hmmax{0}
\newcommand\bmmax{0}
% packages
\usepackage{diagbox}
\usepackage{makecell}
\usepackage{booktabs}
\usepackage{tikz,tikz-3dplot}
\usepackage{amsmath}
\usepackage{bbm}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{url,ifthen}
% \usepackage[sort]{natbib}
\usepackage[shortlabels]{enumitem}
%\usepackage[shortlabele]{enumitem}
\usepackage{srcltx}
\usepackage{dsfont}
\usepackage{multirow}
\usepackage{boxedminipage}
\usepackage[margin=1.1in]{geometry}
\usepackage{nicefrac}
\usepackage{xspace}
\usepackage{graphicx}
\usepackage{color}
\usepackage{subfigure}
\usepackage{colortbl}
\usepackage{setspace}
\usepackage{pgfplots}
\pgfplotsset{compat=1.12}
\usepackage{algorithm,algorithmic}
\usepackage[algo2e]{algorithm2e}


\usepackage{xcolor}
\definecolor{DarkGreen}{rgb}{0.1,0.5,0.1}
\definecolor{DarkRed}{rgb}{0.5,0.1,0.1}
\definecolor{DarkBlue}{rgb}{0.1,0.1,0.5}
\definecolor{Gray}{rgb}{0.2,0.2,0.2}

\definecolor{c1}{RGB}{38, 70, 83}
\definecolor{c2}{RGB}{42, 157, 143}
\definecolor{c3}{RGB}{233, 196, 106}
\definecolor{c5}{RGB}{231, 111, 81}
\definecolor{c4}{RGB}{244, 162, 97}





\definecolor{c1}{RGB}{38, 70, 83}
\definecolor{c2}{RGB}{42, 157, 143}
\definecolor{c3}{RGB}{233, 196, 106}
\definecolor{c5}{RGB}{231, 111, 81}
\definecolor{c4}{RGB}{244, 162, 97}
\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

\renewcommand{\ttdefault}{pcr}
\usepackage{listings}
\lstdefinestyle{mystyle}{
    commentstyle=\color{DarkBlue},
    keywordstyle=\color{DarkRed},
    numberstyle=\tiny\color{Gray},
    stringstyle=\color{DarkGreen},
    basicstyle=\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2
}
\lstset{style=mystyle}


\usepackage[small]{caption}
\usepackage[pdftex]{hyperref}
\hypersetup{
    unicode=false,          % non-Latin characters in AcrobatÂ¿s bookmarks
    pdftoolbar=true,        % show Acrobat toolbar?
    pdfmenubar=true,        % show Acrobat menu?
    pdffitwindow=false,      % page fit to window when opened
    pdfnewwindow=true,      % links in new window
    colorlinks=true,       % false: boxed links; true: colored links
    linkcolor=DarkBlue,          % color of internal links
    citecolor=DarkGreen,        % color of links to bibliography
    filecolor=DarkRed,      % color of file links
    urlcolor=DarkBlue,          % color of external links
    %
    % paper specific, please update
    %
    pdftitle={},
    pdfauthor={},
}


% 1 for working draft
% will show author notes
\def\draft{1}

% 1 for submission version
% set to zero after submission
% use \forsubmit{visible during submission}
% and \forreals{visible after submission}
\def\submit{0}

\ifnum\draft=1 % show authors' note if draft
    \def\ShowAuthNotes{1}
\else
    \def\ShowAuthNotes{0}
\fi

\ifnum\submit=1
\newcommand{\forsubmit}[1]{#1}
\newcommand{\forreals}[1]{}
\else
\newcommand{\forreals}[1]{#1}
\newcommand{\forsubmit}[1]{}
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Author's notes
\ifnum\ShowAuthNotes=1
\newcommand{\authnote}[2]{{ \footnotesize \bf{\color{DarkRed}[#1's Note:
{\color{DarkBlue}#2}]}}}
\else
\newcommand{\authnote}[2]{}
\fi

\newcommand{\jcpnote}[1]{{\color{purple}Juanky: #1}}

%
% theorem environments
%

\newtheorem{theorem}{Theorem}[section]
\newtheorem{remark}[theorem]{Remark}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{claim}[theorem]{Claim}%[section]
\newtheorem{fact}[theorem]{Fact}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{assumption}[theorem]{Assumption}

\newtheorem{definition}[theorem]{Definition}%[section]
% \newtheorem{question}{Question}[section]
% \newtheorem{openQ}[theorem]{Open Question}

\newtheorem*{definition*}{Definition}
\newtheorem*{proposition*}{Proposition}
\newtheorem{result}{Theorem}


\theoremstyle{definition}
\newtheorem*{example*}{Example}
\newtheorem{example}[theorem]{Example}

% option to continue an example
\newtheoremstyle{example_contd}
{\topsep} {\topsep}%
{}% Body font
{}% Indent amount (empty = no indent, \parindent = para indent)
{\bfseries}% Thm head font
{.}% Punctuation after thm head
{1em}% Space after thm head (\newline = linebreak)
{\thmname{#1} \thmnumber{ #2}\thmnote{#3} (continued)}% Thm head spec

\theoremstyle{example_contd}
\newtheorem*{example_contd}{Example}

%
% nice refs
%
\newcommand{\chapterlabel}[1]{\label{ch:#1}}
\newcommand{\chapterref}[1]{\hyperref[ch:#1]{Chapter~\ref{ch:#1}}}
\newcommand{\claimlabel}[1]{\label{claim:#1}}
\newcommand{\claimref}[1]{\hyperref[claim:#1]{Claim~\ref{claim:#1}}}
\newcommand{\corollarylabel}[1]{\label{cor:#1}}
\newcommand{\corollaryref}[1]{\hyperref[cor:#1]{Corollary~\ref{cor:#1}}}
\newcommand{\definitionlabel}[1]{\label{def:#1}}
\newcommand{\definitionref}[1]{\hyperref[def:#1]{Definition~\ref{def:#1}}}
\newcommand{\equationlabel}[1]{\label{eq:#1}}
\newcommand{\equationref}[1]{\hyperref[eq:#1]{Equation~\ref{eq:#1}}}
\newcommand{\factlabel}[1]{\label{fact:#1}}
\newcommand{\factref}[1]{\hyperref[fact:#1]{Fact~\ref{fact:#1}}}
\newcommand{\figurelabel}[1]{\label{fig:#1}}
\newcommand{\figureref}[1]{\hyperref[fig:#1]{Figure~\ref{fig:#1}}}
\newcommand{\tablelabel}[1]{\label{tab:#1}}
\newcommand{\tableref}[1]{\hyperref[tab:#1]{Table~\ref{tab:#1}}}
\newcommand{\itemlabel}[1]{\label{item:#1}}
\newcommand{\itemref}[1]{\hyperref[item:#1]{Item~(\ref{item:#1})}}
\newcommand{\lemmalabel}[1]{\label{lem:#1}}
\newcommand{\lemmaref}[1]{\hyperref[lem:#1]{Lemma~\ref{lem:#1}}}
\newcommand{\proplabel}[1]{\label{prop:#1}}
\newcommand{\propref}[1]{\hyperref[prop:#1]{Proposition~\ref{prop:#1}}}
\newcommand{\propositionlabel}[1]{\label{prop:#1}}
\newcommand{\propositionref}[1]{\hyperref[prop:#1]{Proposition~\ref{prop:#1}}}
\newcommand{\remarklabel}[1]{\label{rem:#1}}
\newcommand{\remarkref}[1]{\hyperref[rem:#1]{Remark~\ref{rem:#1}}}
\newcommand{\sectionlabel}[1]{\label{sec:#1}}
\newcommand{\sectionref}[1]{\hyperref[sec:#1]{Section~\ref{sec:#1}}}
\newcommand{\theoremlabel}[1]{\label{thm:#1}}
\newcommand{\theoremref}[1]{\hyperref[thm:#1]{Theorem~\ref{thm:#1}}}


%
% nice fonts
%
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{kpfonts}
\usepackage{microtype}

% Expectation, Probability, Variance
\newcommand{\Esymb}{\mathbb{E}}
\newcommand{\Psymb}{\mathbb{P}}
\newcommand{\Vsymb}{\mathbb{V}}
\DeclareMathOperator*{\E}{\Esymb}
\DeclareMathOperator*{\Var}{\Vsymb}
\DeclareMathOperator*{\ProbOp}{\Psymb r}
\renewcommand{\Pr}{\ProbOp}
\newcommand{\prob}[1]{\Pr\big\{ #1 \big\}}
\newcommand{\Prob}[1]{\Pr\left\{ #1 \right\}}
\newcommand{\varprob}[1]{\Pr\big( #1 \big)}
\newcommand{\varProb}[1]{\Pr\left( #1 \right)}
\newcommand{\ex}[1]{\E\big[#1\big]}
\newcommand{\Ex}[1]{\E\left[#1\right]}
\newcommand{\varex}[1]{\E\paren{#1}}
\newcommand{\varEx}[1]{\E\Paren{#1}}
\newcommand{\widebar}[1]{\overline{#1}}
\newcommand{\tv}{\text{TV}}

% nice fractions
\newcommand{\flatfrac}[2]{#1/#2}
\newcommand{\nfrac}{\nicefrac}
\newcommand{\half}{\nfrac12}
\newcommand{\quarter}{\nfrac14}

% punctuation at the end of a displayed formula
\newcommand{\mper}{\,.}
\newcommand{\mcom}{\,,}

\renewcommand{\hat}{\widehat}

% cally fonts
\newcommand{\cA}{{\cal A}}
\newcommand{\cB}{{\cal B}}
\newcommand{\cC}{{\cal C}}
\newcommand{\cD}{{\cal D}}
\newcommand{\cE}{{\cal E}}
\newcommand{\cF}{{\cal F}}
\newcommand{\cG}{{\cal G}}
\newcommand{\cH}{{\cal H}}
\newcommand{\cI}{{\cal I}}
\newcommand{\cJ}{{\cal J}}
\newcommand{\cK}{{\cal K}}
\newcommand{\cL}{{\cal L}}
\newcommand{\cM}{{\cal M}}
\newcommand{\cN}{{\cal N}}
\newcommand{\cO}{{\cal O}}
\newcommand{\cP}{{\cal P}}
\newcommand{\cQ}{{\cal Q}}
\newcommand{\cR}{{\cal R}}
\newcommand{\cS}{{\cal S}}
\newcommand{\cT}{{\cal T}}
\newcommand{\cU}{{\cal U}}
\newcommand{\cV}{{\cal V}}
\newcommand{\cW}{{\cal W}}
\newcommand{\cX}{{\cal X}}
\newcommand{\cY}{{\cal Y}}
\newcommand{\cZ}{{\cal Z}}

% binary relations
\newcommand{\defeq}{\stackrel{\small \mathrm{def}}{=}}
\renewcommand{\leq}{\leqslant}
\renewcommand{\le}{\leqslant}
\renewcommand{\geq}{\geqslant}
\renewcommand{\ge}{\geqslant}
% parentheses
\newcommand{\paren}[1]{(#1 )}
\newcommand{\Paren}[1]{\left(#1 \right )}
% brackets
\newcommand{\brac}[1]{[#1 ]}
\newcommand{\Brac}[1]{\left[#1 \right]}
% set braces
\newcommand{\set}[1]{\{#1\}}
\newcommand{\bigset}[1]{\bigl\{#1\bigr\}}
\newcommand{\Set}[1]{\left\{#1\right\}}
% absolute value sign
\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\Abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\Bigabs}[1]{\Bigl\lvert#1\Bigr\rvert}
\newcommand{\card}[1]{\lvert#1\rvert}
\newcommand{\Card}[1]{\left\lvert#1\right\rvert}
% norm
\newcommand{\norm}[1]{\lVert#1\rVert_2}
\newcommand{\Norm}[1]{\left\lVert#1\right\rVert}
% declare function f as $f \from X \to Y$
\newcommand{\from}{\colon}
% differential as in "\int x\rd x"
\newcommand\rd{\,\mathrm{d}}
% sets
\newcommand{\bits}{\{0,1\}}
\newcommand{\signs}{\{-1,1\}}
\renewcommand{\Re}{\mathbb{R}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb Z}
\renewcommand{\D}{\mathcal D}
\newcommand{\C}{\mathbb C}
\newcommand{\N}{\mathbb N}
\newcommand{\varR}{\Re}
\newcommand{\Rnn}{\R_+}
\newcommand{\varRnn}{\varR_+}
% qed symbol
\renewcommand{\qedsymbol}{{$\blacksquare$}}
% bold vector notation
\usepackage{bm}
\renewcommand{\vec}[1]{{\bm{#1}}}

% linear algebra
\DeclareMathOperator*{\range}{range}
\newcommand{\Mid}{\ensuremath{~\Big|~}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\trans}{\top}
\newcommand{\pinv}{\dagger}
\newcommand{\iprod}[1]{\langle #1\rangle}
\newcommand{\isqur}[1]{\langle #1,#1\rangle}
\newcommand{\trsp}[1]{#1^\dagger}
\newcommand{\vartrsp}[1]{#1^T}
\newcommand{\varvartsp}[1]{#1^{\mathsf{T}}}
\newcommand{\smallrmtrsp}[1]{#1^{\scriptscriptstyle \mathrm{T}}}
\newcommand{\oprod}[2]{\trsp{#1} #2}
\newcommand{\osqur}[1]{\oprod{#1}{#1}}
% transposed of a vector
\newcommand{\trspvec}[1]{{\trsp{\vec{#1}}}}
% norm
\newcommand{\snorm}[1]{\norm{#1}^2}
% L2 norm
\newcommand{\normt}[1]{\norm{#1}_{\scriptstyle 2}}
\newcommand{\varnormt}[1]{\norm{#1}_{\scriptscriptstyle 2}}
\newcommand{\snormt}[1]{\normt{#1}^2}
% L1 norm
\newcommand{\normo}[1]{\norm{#1}_{\scriptstyle 1}}
\newcommand{\Normo}[1]{\Norm{#1}_{\scriptstyle 1}}
\newcommand{\varnormo}[1]{\norm{#1}_{\scriptscriptstyle 1}}
% Linfty norm
\newcommand{\normi}[1]{\norm{#1}_{\scriptstyle \infty}}
\newcommand{\varnormi}[1]{\norm{#1}_{\scriptscriptstyle \infty}}

% super set with parentheses
\newcommand{\super}[2]{#1^{\paren{#2}}}
\newcommand{\varsuper}[2]{#1^{\scriptscriptstyle\paren{#2}}}

% Indictator function
\newcommand{\Ind}{\mathbb I}

%Independence symbol
\newcommand{\indep}{\!\perp\!\!\!\perp}
%\newcommand{\notindep}{ \perp  \not \!\!\! \perp}
\newcommand{\notindep}{\not\!\perp\!\!\!\perp }


% common abbrevs
\newcommand{\ignore}[1]{}
\newcommand{\OPT}{\mathrm{OPT}}
\newcommand{\opt}{\mathrm{opt}}
\newcommand{\KL}{\mathrm{KL}}
\newcommand{\sign}{\mathrm{sign}}
\newcommand{\polylog}{{\rm polylog}}
\newcommand{\poly}{{\rm poly}}
\newcommand{\vol}{\mathrm{vol}}
\newcommand{\supp}{\mathrm{supp}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\reg}{\text{reg}}

% epsilon wars
\renewcommand{\epsilon}{\varepsilon}
\newcommand{\e}{\epsilon}
\newcommand{\eps}{\epsilon}

% distributions
\newcommand{\Laplace}{\mathrm{Lap}}
\newcommand{\Lap}{\Laplace}
\newcommand{\Bin}{\mathrm{Bin}}
\newcommand{\Unif}{\mathrm{Unif}}


% remove text
\newcommand{\remove}[1]{}

%
% draftbox
%
\newcommand{\draftbox}{\begin{center}
  \fbox{%
    \begin{minipage}{2in}%
      \begin{center}%
        \begin{Large}%
          \textsc{Working Draft}%
        \end{Large}\\
        Please do not distribute%
      \end{center}%
    \end{minipage}%
  }%
\end{center}
\vspace{0.2cm}}

% compact itemize and enumerate
\renewcommand{\labelitemi}{--}
\newenvironment{itm}
{\begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]}
{\end{itemize}}
\newenvironment{enum}
{\begin{enumerate}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]}
{\end{enumerate}}

% control white space of list and display environments
%
%\newcommand{\listoptions}{\labelsep0mm\topsep-0mm\itemindent-6mm\itemsep0mm}
%\newcommand{\displayoptions}[1]{\abovedisplayshortskip#1mm\belowdisplayshortskip#1mm\abovedisplayskip#1mm\belowdisplayskip#1mm}

%
%  PAPER SPECIFIC MACROS
%  add them below this
%


\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calYhat}{\hat{\calY}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calL}{\mathcal{L}}

\newenvironment{oneshot}[1]{\@begintheorem{#1}{\unskip}}{\@endtheorem}

\newcommand{\mtilde}{\tilde{m}}


\newcommand{\model}{M}
\newcommand{\score}{R}
\newcommand{\K}{\mathcal K}
\newcommand{\lgrad}[2]{\E_{z \sim \D(#1)}\nabla_\theta \ell(z; #2)}
\newcommand{\ploss}[2]{\E_{z \sim \D(#1)}\ell(z; #2)}
\newcommand{\plossemp}[3]{\E_{z \sim \D^{#2}(#1)}\ell(z; #3)}
\newcommand{\glgrad}[2]{\E_{z \sim \D(#1)}\nabla_\theta \ell(z; G(#2))}
\newcommand{\elgrad}[2]{\E_{z \sim {#1}}\nabla_\theta \ell(z; #2)}

\newcommand{\gd}{G_{\text{gd}}}
\newcommand{\pregloss}[2]{\E_{z \sim \D({#1})}\ell^{\reg}(z; #2)}

\newcommand{\PR}{\mathrm{PR}}
\newcommand{\thetaSL}{{\theta_{\mathrm{SL}}}}
\newcommand{\thetaPO}{{\theta_{\mathrm{PO}}}}
\newcommand{\thetaPS}{{\theta_{\mathrm{PS}}}}
\newcommand{\thetaSE}{{\theta_{\mathrm{SE}}}}
\newcommand{\map}{{\mathrm{DPR}}}

\newcommand{\varlipc}{L}
\newcommand{\bigexp}[1]{\E \big[ #1 \big]}
\newcommand{\tgamma}{\tilde{\gamma}}


% Project Specific Macros
\newcommand{\yhat}{\hat{y}}
\newcommand{\qt}{\tilde{q}}
\newcommand{\ptilde}{\tilde{p}}
\newcommand{\amo}{\mathsf{AMO}}

\newcommand{\ellvec}{\ell_{\mathsf{vec}}}
\newcommand{\cscalg}{\cA_{\mathrm{csc}}}

\newcommand{\omax}{\omega_{\max}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\purple}[1]{\textcolor{purple}{#1}}

%% Michael's
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Xcal}{\cX}
\newcommand{\Ych}{\cYh}
\newcommand{\1}{\ind}

\newcommand{\Wcal}{\mathcal{W}}

\newcommand{\rct}{\D_\mathrm{rct}}














==> arxiv 2/mc.tex <==









% \begin{definition}[Performative Multicalibration]
% A predictor $\pt:\Xcal \times \Ych \to [0,1]$ is $(\Hcal,\alpha)$-multicalibrated under performativity if for all $h \in \Hcal$, $\yhat \in \Ych$, and all $v \in \supp(\pt)$,
% \begin{gather*}
%     \card{\E_{\substack{x \sim \D\\\ys \sim \ps(x,\yhat)}}[h(x) \cdot \1[\pt(x,\yhat) = v] \cdot (\ys - v)]} \le \alpha.
% \end{gather*}
% \end{definition}


\begin{definition}[Performative Multicalibration]
For a hypothesis class $\Hcal$ and approximation parameter $\alpha \ge 0$, a predictor $\pt$ is $(\Hcal, \alpha)$-multicalibrated under performativity if for all $h \in \Hcal$ and all $v \in \supp(\pt)$
% \begin{gather*}
%     \E_{\substack{x \sim \D\\\ys \sim \ps(x,\yhat)}}[h(x) \cdot \omega(\pt(x,\yhat)) \cdot (\ys - \pt(x,\yhat))] \in [-\alpha,\alpha].
% \end{gather*}
\begin{gather*}
    \E_{\substack{x \sim \D\\\ys \sim \ps(x,h(x))}}[h(x) \cdot \1_v[\pt(x,h(x))] \cdot (\ys - \pt(x,h(x)))] \approx_\alpha 0.
\end{gather*}
\end{definition}


Useful:  assume that $\Hcal$ contains all constant hypotheses.
That is, we obtain some version of calibration from multicalibration:  for all $\yhat \in \Ych$
\begin{gather*}
    \E_{\substack{x \sim \D\\\ys \sim \ps(x,\yhat)}}[\1_v[\pt(x,\yhat)] \cdot (\ys - \pt(x,\yhat)] \approx_\alpha 0
\end{gather*}



\paragraph{Proof of Convex Omniprediction:}
\begin{proof}
Assumptions:  $\pt$ is a predictor that satisfies
\begin{itemize}
    \item Bounded support size $\card{\supp(\pt)} = s$
    \item $\alpha/s$-calibrated
    \item $(\Hcal,\alpha/s)$-multicalibrated
\end{itemize}
For any convex loss $\ell$, we need to show the following inequality holds:
\begin{gather*}
    \E_{\substack{x \sim \D\\\ys \sim \ps(x,f_\ell(x))}}[\ell(f_\ell(x),\ys)] \le \E_{\substack{x \sim \D\\\ys \sim \ps(x,h(x))}}[\ell(h(x),\ys)] + \eps
\end{gather*}
for $\eps \le 10\alpha$.
We go step by step.

First, we switch our view from a loss over $\ys$ to one over $\yt$.  In particular, (\ref{eqn:yt:calibration}) follows under calibration.
\begin{gather}\label{eqn:yt:calibration}
    \E_{\substack{x \sim \D\\\ys \sim \ps(x,f_\ell(x))}}[\ell(f_\ell(x),\ys)]
    \approx_\alpha \E_{\substack{x \sim \D\\\yt \sim \pt(x,f_\ell(x))}}[\ell(f_\ell(x),\yt)]
\end{gather}
Then, by the optimality of $f_\ell$, we can switch our view to any predictor that could also be derived from $\pt$.
Specifically, consider the function $h_\ell$ defined as
\begin{gather*}
    h_\ell(v) = \argmin_{\yhat \in \Ych} \E_{y_v\sim \Ber\left(\E[h(x) \vert \pt(x,\yhat) = v]\right)}[\ell(\yhat,y_v)]
\end{gather*}
\mpk{A bit suspect, but maybe not wrong?
The point is that we want to ensure that the policy we come up with is constant on the level sets of $\pt$.
In this case, calibration should save us?
Importantly, $y$-performativity is decomposable across units, so we can mix and match the calibration constraints for each $v \in \supp(\pt)$ regardless of what $\yhat$ is actually chosen.
}

\end{proof}





% Different weight classes correspond to specific multi-group notions.
% \begin{itemize}
%     \item $\Wcal = \set{1}$:  $(\Hcal,\alpha)$-multiaccuracy
%     \begin{gather*}
%     \E_{\substack{x \sim \D\\\ys \sim \ps(x,\yhat)}}[h(x) \cdot (\ys - \pt(x,\yhat))] \approx_\alpha 0
%     \end{gather*}
%     \item $\Wcal = \set{1,\mathrm{id}}$:  ``Degree-2'' $(\Hcal,\alpha)$-multicalibration
%     \begin{gather*}
%     \E_{\substack{x \sim \D\\\ys \sim \ps(x,\yhat)}}[h(x) \cdot \pt(x,\yhat) \cdot (\ys - \pt(x,\yhat))] \approx_\alpha 0
%     \end{gather*}
%     \item $\Wcal = \set{\1[\cdot = v] : v \in \supp(\pt)}$:  ``Full'' $(\Hcal,\alpha)$-multicalibration
%     \begin{gather*}
%     \E_{\substack{x \sim \D\\\ys \sim \ps(x,\yhat)}}[h(x) \cdot \1[\pt(x,\yhat) = v] \cdot (\ys - \pt(x,\yhat))] \approx_\alpha 0
%     \end{gather*}
%     for all $v \in \supp(\pt)$.
% \end{itemize}



\subsection{Technical Overview}

\begin{itemize}
    \item Performative Optimality:
    \begin{itemize}
        \item Frame it as agnostic PAC optimality (rather than parameter recovery/optimization)
        \item Challenges of optimality:  the optimal predictor on a set of labels will not be the optimal predictor after deploying the predictor
        \item Retraining known to converge to a stable point
        \item Key insight:  model the prediction as an ``input'' to the predictive model.  Train with the prediction in mind.  (Prediction?  Decision?  Action?)
        \item \mpk{Do we want to highlight the direct RCT / agnostic learning strategy?}
    \end{itemize}
    \item Performative Omniprediction:
    \begin{itemize}
        \item Often when we deploy a prediction system, we don't know exactly what loss we want to minimize.
        \item Ideally, would have a single predictor that could be used, meaningfully, by different clients with different objectives
        \item Concretely, when predictions are performative, it may be useful to have predictions that are equally good at estimating expected outcomes as it is for estimating the success of steering by intervention.
        \item Can we get a single predictor for such a task?
        \item Omniprediction:  developed in the literature on multicalibration.
        \item So a natural starting point for performative omnipredictor would be an analogue of performative multicalibration.
    \end{itemize}
    \item Performative Calibration vs.\ Static Calibration
    \begin{itemize}
        \item Calibration says: expected outcome, given predicted probability $v$ is $v$
        \item But what is the modeled probability under performativity?  It is a function of the choice of \emph{action}.
        \begin{gather*}
            \E_{\ys \sim \ps(x,\yhat)}[\ys \vert \pt(x,\yhat) = v] = v
        \end{gather*}
        \item In other words, even for a binary outcome, calibration becomes a vector-valued set of constraints.  The number of constraints scales \emph{exponentially} in the number of actions!
        \item But do we really care about all of the actions?  Could apply ``decision calibration'' to only focus on optimal decisions, but not obvious it helps. Also, clunky.
    \end{itemize}
    \item Performative Outcome Indistinguishability
    \begin{itemize}
        \item Idea:  develop $\pt$ to mimic $\ps$.  According to relevant tests.
        \item Avoid multicalibration and calibration.  Only focus on loss-based tests, for the predictions relevant to the losses and predictors relevant.
        \item Pro and con:  by explicitly accounting for losses, we can handle ``steering'' losses, in addition to standard convex losses.
    \end{itemize}
\end{itemize}


\clearpage

\paragraph{Outline of results.}
\begin{itemize}
    \item Performative optimality via OI
    \begin{itemize}
        \item \textbf{Def:} Performative OI in terms of a single loss function $\ell$
        \item \textbf{Def:} Decision OI for single loss function $\ell$
        \item \textbf{Thm:} $(\ell,\Hcal,\alpha)$-Performative OI implies $(\ell,\Hcal,\alpha)$-Performative optimality
        \item \textbf{Pf:}  three liner
    \end{itemize}
    \item Performative Omniprediction
    \begin{itemize}
        \item In fact, can get Performative OI and Decision OI for many losses simultaneously
        \item \textbf{Cor:}  Can get Performative Omniprediction for $\cL$ by auditing for each $\ell \in \cL$ explicitly.
    \end{itemize}
    \item Omniprediction for losses that only depend on $\yhat$
    \begin{itemize}
        \item Consider $\cL_1$ the class of all bounded losses that only depend on $x$ through $h(x)$.
        \item \textbf{Def:}  Multiaccuracy
        \item \textbf{Def:}  Decision Calibration
        \item \textbf{Lem:}  $(\Hcal,\alpha)$-Multiaccuracy implies $(\cL_1,\Hcal,2\alpha)$-Performative OI
        \item \textbf{Lem:}  $\alpha$-Decision calibration implies $(\cL_1,\alpha)$-Decision OI
        \item \textbf{Cor:}  $(\Hcal,\alpha)$-MA + $\alpha$-Dec Calibration implies $(\cL_1,\Hcal,3\alpha)$-Performative Omniprediction.
        \item That is, we get a loss-independent approach for omniprediction for all losses.
        \item Note:  can also mix-and-match, e.g., multiaccuracy + $\cL$-decision OI for your favorite $\cL$.
    \end{itemize}
    \item Learning Performative OI predictors:
    \begin{itemize}
        \item Explicit search
        \item Reduction to learning (particularly for multiaccuracy / decision calibration)
        \item Bounded sample complexity!
        \item \textbf{Thm:}  There exists an oracle-efficient, sample-efficient learning algorithm that returns a Performative Omnipredictor.
        \item Open questions about auditing
    \end{itemize}
    \item Universal Adaptability:
    \begin{itemize}
        \item Impossible to get $X$-performativity without modeling the distribution of $X$ explicitly
        \item Short of this, next best thing is that optimality would hold even under covariate shift
        \item \textbf{Cor:}  With the right loss class, you get universal adpaptability too!
        \item Interesting question of how to execute the search reduction to learning effectively.
    \end{itemize}
\end{itemize}








\clearpage
Let $\mathcal{L}_1 = \set{\ell:\Ych \times \set{0,1} \to [-1,1]}$ be the class of all bounded loss functions.



\begin{definition}[Decision OI]
Fix a class of loss functions $\cL$.
A predictor $\pt:\Xcal \times \Ych \to [0,1]$ is $(\cL,\alpha)$-decision outcome indistinguishable if for all $\ell \in \cL$
\begin{gather*}
    \E_{\ys \sim \ps(x,f_\ell(x))}[\ell(f_\ell(x),\ys)] \approx_\alpha \E_{\yt \sim \pt(x,f_\ell(x))}[\ell(f_\ell(x),\yt)].
\end{gather*}
\end{definition}


\begin{definition}[Decision Calibration]
A predictor $\pt:\Xcal \times \Ych \to [0,1]$ is $(\cL,\alpha)$-decision calibrated if for every bounded loss $\ell \in \cL_1$, for all $\yhat \in \Ych$
\begin{gather*}
    \E_{\ys \sim \ps(x,f_\ell(x))}[\ys \vert f_\ell(x) = \yhat] \approx_\alpha \E_{\yt \sim \pt(x,f_\ell(x))}[\yt \vert f_\ell(x) = \yhat]
\end{gather*}
\end{definition}

\mpk{
Note:  decision calibration is equivalent to the following technical condition.

Does there exist a $\yhat \in \Ych, w_0,w_1 \in [-1,1]$ such that:
\begin{gather*}
    \E_x[\pt(x,\yhat) - \ps(x,\yhat) ~\vert~ \argmin_{a \in \Ych}\set{ w_1 \cdot \pt(x,a) + w_0 \cdot (1-\pt(x,a))} = \yhat] > \alpha
\end{gather*}
i.e., does there exist some $\ell \in \cL_1$ and $\yhat \in \Ych$ such that conditioning on the event that $f_\ell(x) = \yhat$ maintains accurate expectations of probabilities.

Note:  this means we can probably run explicit searches over $\poly(1/\alpha)$ many choices of $w_0,w_1$, then compute the minimizers, and evaluate the conditional expectations for $\card{\Ych}$ choices of $\yhat$.

So, auditing is reasonably efficient.  e.g., linear in $\card{\Ych}$, not exponential!

}

\begin{definition}[Multiaccuracy]
Fix a hypothesis class $\Hcal$.
A predictor $\pt:\Xcal \times \Ych \to [0,1]$ is $(\Hcal,\alpha)$-multiaccurate under outcome performativity if for all $h \in \Hcal$
\begin{gather*}
    \E_{\ys \sim \ps(x,h(x))}[\ys \vert h(x) = \yhat] \approx_\alpha \E_{\yt \sim \pt(x,h(x))}[\yt \vert h(x) = \yhat].
\end{gather*}
\end{definition}
\mpk{some sloppiness in approximation here.  Do we want it to be weighted by $\Pr[h(x) = \yhat]$?}

\begin{definition}[Performative OI]
Fix a hypothesis class $\Hcal$.
A predictor $\pt:\Xcal \times \Ych \to [0,1]$ is $(\Hcal,\alpha)$-performative outcome indistinguishable if for all $\ell \in \mathcal{L}_1$ and all $h \in \Hcal$,
\begin{gather*}
    \E_{\yt \sim \pt(x,h(x))}[\ell(h(x),\yt)] \approx_\alpha \E_{\ys \sim \ps(x,h(x))}[\ell(h(x),\ys)].
\end{gather*}
\end{definition}

\begin{lemma}
If $\pt:\Xcal \times \Ych \to [0,1]$ is $(\Hcal,\alpha)$-multiaccurate, then $\pt$ is $(\Hcal,2\alpha)$-performative OI.
\end{lemma}
\begin{proof}
We show an approximate equality between the loss $\ell \in \mathcal{L}_1$ of any $h \in \Hcal$ under $\yt \sim \pt(x,h(x))$ and $\ys \sim \ps(x,h(x))$.
\begin{align*}
\E_{\yt \sim \pt(x,h(x))}[\ell(h(x),\yt)]
&= \sum_{\yhat \in \Ych} \Pr[h(x) = \yhat] \cdot \E_{\yt \sim \pt(x,h(x))}[\ell(\yhat,\yt) ~\vert~ h(x) = \yhat]\\
&= \sum_{\yhat \in \Ych} \Pr[h(x) = \yhat] \cdot \E_{\yt \sim \pt(x,h(x))}\left[\yt \cdot \ell(\yhat,1) + (1-\yt) \cdot \ell(\yhat,0) ~\vert~ h(x) = \yhat\right]\\
&\approx_{2\alpha} \sum_{\yhat \in \Ych} \Pr[h(x) = \yhat] \cdot \E_{\ys \sim \ps(x,h(x))}\left[\ys \cdot \ell(\yhat,1) + (1-\ys) \cdot \ell(\yhat,0) ~\vert~ h(x) = \yhat\right]\\
&= \sum_{\yhat \in \Ych} \Pr[h(x) = \yhat] \cdot \E_{\ys \sim \ps(x,h(x))}[\ell(\yhat,\ys) ~\vert~ h(x) = \yhat]\\
&=\E_{\ys \sim \ps(x,h(x))}[\ell(h(x),\ys)]
\end{align*}
The approximate equality follows under the assumption that $\pt$ is $(\Hcal,\alpha)$-multiaccurate and the bound on the magnitude of $\card{\ell(\yhat,b)} \le 1$ for all $\yhat \in \Ych$ and $b \in \set{0,1}$.
\end{proof}


% \begin{proposition}
% Suppose $\Hcal$ is a class of boolean functions.
% If $\pt:\Xcal \to [0,1]$ is $\C$-multiaccurate and calibrated, then for \emph{any} loss $\ell$, the optimal post-processing $f_\ell$ is an $(\ell,\C)$-agnostic learner.
% \end{proposition}
% \begin{proof}
% Fix a loss $\ell$.
% For a given performative probability $q:\Ych \to [0,1]$, we define $\tilde{\ell}(q)$ to be the optimal loss achievable to predict $y \sim q$.
% \begin{align*}
% \tilde{\ell}(q)
% &= \min_{\yhat}\set{q(\yhat)\cdot \ell(\yhat,1) + (1-q(\yhat)) \cdot \ell(\yhat,0)}
% \end{align*}
% First, we consider the loss experienced by $f_\ell$.
% \begin{align*}
% \E_{\ys \sim \ps(x,f_\ell(x))}[\ell(f_\ell(x),\ys)]
% &= \E_{\yt \sim \ps(x,f_\ell(x))}[\ell(f_\ell(x),\yt)]
% \end{align*}
% by Decision OI.
% Then,
% \begin{align*}
% &= \sum_{\yhat} \Pr[f_\ell(x) = \yhat] \cdot \sum_{v} \Pr[\pt(x,\yhat) = v \vert f_\ell(x) = \yhat] \cdot \E_{\yt \sim \pt(x,\yhat)}[\ell(\yhat,\yt) \vert \pt(x,\yhat) = v, f_\ell(x) = \yhat]\\
% &= \sum_{\yhat} \Pr[f_\ell(x) = \yhat] \cdot \sum_{v} \Pr[\pt(x,\yhat) = v \vert f_\ell(x) = \yhat] \cdot \left(v\cdot \ell(\yhat,1) + (1-v) \cdot \ell(\yhat,0)\right)
% \end{align*}
% where the final equality follows by the definition of $f_\ell$ and the assumption that $\pt$ is calibrated.
% Expanding $\tilde{\ell}(v)$, we upper bound the loss of $f_\ell \circ \pt$ by the loss of any $c \in \C$ as follows.
% \begin{align*}
% % \sum_{v} \Pr[\pt(x) = v] \cdot \tilde{\ell}(v)
% &=  \sum_{v} \Pr[\pt(x) = v] \cdot \min_{a_v}\set{v \cdot \ell(a_v,1) + (1-v) \cdot \ell(a_v,0)}\\
% &\le \sum_{b \in \set{0,1}} \Pr[c(x) = b] \cdot \sum_{v} \Pr[\pt(x) = v \vert c(x) = b] \cdot \min_{a_v}\set{v \cdot \ell(a_v,1) + (1-v) \cdot \ell(a_v,0)}\\
% &\le \sum_{b \in \set{0,1}} \Pr[c(x) = b] \cdot \min_{a}\set{\sum_{v}\Pr[\pt(x) = v \vert c(x) = b] \cdot \left(v \cdot \ell(a,1) + (1-v) \cdot \ell(a,0)\right)}\\
% &= \sum_{b \in \set{0,1}} \Pr[c(x) = b] \cdot \min_{a} \set{\Pr[y = 1 \vert c(x) = b] \cdot \ell(a,1) + \Pr[y = 0 \vert c(x) = b] \cdot \ell(a,0)}\\
% &\le \sum_{b \in \set{0,1}} \Pr[c(x) = b] \cdot \E[\ell(b,y) \vert c(x) = b]\\
% &= \E[\ell(c(x),y)]
% \end{align*}
% where (\ref{eq:multiaccurate}) follows by multiaccuracy of $\pt$.  Specifically, under multiaccuracy, we assume for each $b \in \set{0,1}$, we have the following equalities.
% \begin{align*}
% \sum_{v} \Pr[\pt(x) = v \vert c(x) = b] \cdot v
% &= \sum_{v} \Pr[\pt(x) = v \vert c(x) = b] \cdot \E[\pt(x) \vert c(x) = b \land \pt(x) = v]\\
% &= \E[\pt(x) \vert c(x) = b]\\
% &= \E[y \vert c(x) = b]\\
% &= \Pr[y = 1 \vert c(x) = b]
% \end{align*}
% Thus, for any $\ell$, the post-processed predictor $f_\ell$ is an $(\ell,\C)$-agnostic learner.


% \mpk{This summation seems wrong.  When we sum over $\yhat$, it's no longer the expectation we want.  This should hold for each $\yhat$.}
% \begin{align*}
% \sum_{v} \Pr[\pt(x,\yhat) = v] \cdot v
% &= \sum_{\yhat}\sum_{v} \Pr[h(x) = \yhat] \cdot \Pr[\pt(x,\yhat) = v \vert h(x) = \yhat] \cdot v\\
% &= \sum_{\yhat} \Pr[h(x) = \yhat] \cdot  \E_{\ys \sim \ps(x,h(x))}[\ys \vert h(x) = \yhat]\\
% &= \E_{\ys \sim \ps(x,h(x))}[\ys]
% \end{align*}


% \begin{align*}
% \sum_{v} v \cdot \Pr[\pt(x,\yhat) = v \vert h(x) = \yhat]
% &= \E[\pt(x,\yhat) \vert h(x) = \yhat]\\
% &= \E_{\yt \sim \pt(x,h(x))}[\yt \vert h(x) = \yhat]\\
% &= \E_{\ys \sim \ps(x,h(x))}[\ys \vert h(x) = \yhat]
% \end{align*}

% \end{proof}










==> arxiv 2/omni.tex <==
\section{Omniprediction}

Having introduced performative outcome indistinguishability, we now move on to discuss how naive post-processing of models which satisfy this condition lead
to decision rules which are optimal for a wide variety of losses.

\begin{definition}[Performative Omnipredictor]
Suppose $\cL$ is a collection of loss functions and $\cH$ is a hypothesis class.
For $\eps \geq 0$, a predictor $\pt:\cX \times \cYh \to \Delta(\cY)$ is an $(\cL,\cH, \eps)$-omnipredictor under performativity if for all $\ell \in \cL$,
\begin{align}
    \E_{\substack{x \sim \cD \\ \ys \sim \ps(x,\ft_{\ell}(x))}}[\ell(x, \ft_{\ell}(x),\ys)] \leq \min_{h \in \cH} \E_{\substack{x \sim \cD \\ \ys \sim \ps(x,h(x))}}[\ell(x, h(x),\ys)] + \eps
\end{align}
\end{definition}

The following theorem is the main result of this section. 
\begin{theorem}
\theoremlabel{thm:omniprediction}
Let $\cL$ be a set of loss functions and $\cH$ a hypothesis class. If $\pt$ is
$(\cL, \cH, \epsilon)$-reflexitvely POI, then $\pt$ is an $(\cL, \cH, 2\epsilon)$-omnipredictor under performativity.
\end{theorem}
\begin{proof}
The proof is straightforward. In fact, we only need one side of the POI  inequality:
\begin{align}
\E_{\substack{x \sim \D \\ \ys \sim \ps(x,\ft_{\ell}(x))}}[\ell(x, \ft_{\ell}(x),\ys)]
&\le \E_{\substack{x \sim \D\\\yt \sim \pt(x,\ft_{\ell}(x))}} [\ell(x, f_{\ell, \pt}(x),\yt)] +\epsilon \label{ineq:calibration}\\
&\le \E_{\substack{x \sim \D\\\yt \sim \pt(x,h(x))}}[\ell(x, h(x),\yt)] + \epsilon \label{ineq:def:fell}\\
&\le \E_{\substack{x \sim \D\\\ys \sim \ps(x,h(x))}}[\ell(x, h(x),\ys)] + 2\epsilon \label{ineq:multiaccuracy}.
\end{align}
Here, (\ref{ineq:calibration}) follows by the definition of POI; (\ref{ineq:def:fell}) follows by the definition of $f_{\ell, \pt}$ as the (pointwise) minimizer of the expected loss of outcomes sampled as $\yt \sim \pt(x,\yhat)$; and (\ref{ineq:multiaccuracy}) again follows by the reflexive POI guarantee.
\end{proof}

We can in fact strengthen this past result. A predictor that is reflexively-POI for a class $\cL$ is an omnipredictor not just for the functions in $\cL$, it is also an omnipredictor for any linear combination of functions in $\cL$. 
This follows from the fact that the POI definition is closed under linear combinations of loss functions. More formally,
\begin{lemma}
\lemmalabel{lemma:linear combinations}
Let $\beta > 0$ be some positive constant and $\cL$ be a collection of loss functions. Now define, 
\begin{align*}
	\mathsf{Lin}(\cL, \beta) \defeq \left\{\sum_{i=1}^k \lambda_i \ell_i : \sum_i |\lambda_i| \leq \beta, \; \ell_i \in \cL \right\}.
\end{align*}
If $\pt$ is $(\cL,\cH,\eps)$-POI, then it is also $(\mathsf{Lin}(\cL, \beta),\cH,\beta \eps)$-POI. 
\end{lemma}

\begin{proof}
Using the triangle inequality and the definition of loss calibration,
\begin{align*}
\card{\E_{\substack{x \sim \D\\\yt \sim \pt(x,h(x))}}\sum_i \lambda_i\ell_i(x,h(x),\yt) - \E_{\substack{x \sim \D\\\ys \sim \ps(x,h(x))}} \sum_{i} \lambda_i \ell_i(x, h(x),\ys)} 
\end{align*}
is upper bounded by,
\begin{align*}
\sum_i |\lambda_i |\cdot  \card{\E_{\substack{x \sim \D\\\yt \sim \pt(x,h(x))}}[\ell_i(x,h(x),\yt)] - \E_{\substack{x \sim \D\\\ys \sim \ps(x,h(x))}} [\ell_i(x, h(x),\ys)]} \leq \sum |\lambda_i| \epsilon \leq \beta \epsilon.
\end{align*}
\end{proof}

This observation is particularly relevant in the context of omniprediction. 
It shows how given a predictor $\pt$ which is $(\cL, \cH, \epsilon)$-reflexively POI for a small number of ``basis'' functions $\cL$, we get an omniprediction guarantee with regards to a much richer class of function formed via linear combinations of functions $\cL$. 
We make this formal via the following corollary:


\begin{corollary}
A predictor $\pt$ which is a $(\cL, \cH, \epsilon)$-reflexively POI is a $(\mathsf{Lin}(\cL, \beta), \cH, \beta \epsilon)$-omnipredictor  under performativity.  
\end{corollary}

We illustrate the value of this closure property via following example.
\begin{example}
Assume that both predictions and outcomes are binary, $\cYh = \cY = \{\pm 1\}$. If $\pt$ is performatively outcome indistinguishable for 
\begin{align*}
	\ell_1(\yhat, y) = \yhat, \quad \ell_2(\yhat, y) = y,\quad \ell_3(\yhat, y) = \yhat \cdot y, 
\end{align*}
then it is also performatively outcome indistinguishable for any norm bounded polynomial in these variables. In particular, if $\pt$ is $(\cL_b, \cH, \epsilon)$-reflexively POI for $\cL_b= \{\ell_1, \ell_2, \ell_3\}$, then it is a $(\cL_{\mathrm{poly}}, \cH, 2\epsilon)-$ omnipredictor for the set of losses:
\begin{align*}
	\cL_{\mathrm{poly}} = \left\{ \sum_{j,k=1}^\infty a_{j,k} (\yhat)^j (y)^k: \sum_{j,k} |a_{j,k}| \leq 1 \right\}.
\end{align*}
\end{example}





==> arxiv 2/performative-omni.tex <==

\section{Performative Omniprediction}
\label{sec:omni}

Introduced in the supervised learning setting by \cite{omni},
an omnipredictor is an outcome probability model that suggests an optimal decision rule for any loss within a class of loss functions.
To discuss this concept more formally, we first review the definition optimality with respect to a fixed loss function, under our setting of outcome performativity.
\begin{definition}[Performative Optimality]
For input distribution $\D$, loss function $\ell$, hypothesis class $\Hcal$, and $\eps \ge 0$, a decision rule $f:\Xcal \to \Ych$ is $(\ell,\Hcal,\eps)$-performatively optimal over $\D$ if 
\begin{gather*}
\E_{\substack{x \sim \D\\\ys \sim \ps(x,f(x))}}[\ell(x, f(x),\ys)] \le \min_{h \in \Hcal}\E_{\substack{x \sim \D\\\ys \sim \ps(x,h(x))}}[\ell(x, h(x),\ys)] + \eps.
\end{gather*}
\end{definition}
That is, a decision rule $f$ is performative optimal if $f$ obtains expected loss under the induced outcome distribution (i.e. performative risk) competitive with the best hypothesis in some reference class $h \in \Hcal$.
\footnote{To review, as in \cite{performative} we refer to  $\E_{x \sim \D,\ys \sim \ps(x,h(x))}[\ell(x, h(x),\ys)]$ as the performative risk of $h$ on $\ell$.}
A simple, but key observation is that if we knew the model that generates outcomes for each individual perfectly, then performative optimality is straightforward to achieve.
Given an outcome model $\ps$ that specifies, for a given individual $x \in \Xcal$ and decision $\yhat \in \Ych$, the probability of outcome $y \sim \ps(x,\yhat)$, the optimal decision rule for any loss function can be determined by a simple optimization over the choice of decisions $\yhat$, as follows.
\begin{fact}[Optimal Decision Rule]
\label{fact:opt}
Fix an outcome model $\ps:\Xcal \times \Ych \to [0,1]$.
For a loss $\ell:\Xcal \times \Ych \times \cY \to \R_{\ge 0}$, there exists a globally optimal decision rule $f_{\ell}^*:\Xcal \to \Ych$ for $\ell$ under $\ps$, given by the pointwise loss-minimizer,
\begin{gather}
\equationlabel{eq:optimal_rule}
    f^*_{\ell}(x) = \argmin_{\yhat \in \Ych}\E_{\ys \sim \ps(x,\yhat)}[\ell(x,\yhat,\ys)].
\end{gather}
\end{fact}
For instance, when $\Ych$ is discrete and finite, then the optimal prediction can be computed by linearly enumerating over $\cYh$, and computing a finite sum of two terms each time.
% \jcpnote{Add comment on the argmin being a linear time operation in the size of $\cYh$}
We will often consider the optimal decision rule $\ft_{\ell}$ after post-processing an approximate outcome model, or predictor, denoted as $\pt$. 

With these definitions of performative optimality and optimal decision rule in place, we are ready to define performative omniprediction.
An omnipredictor is an outcome model $\pt$ where for \emph{every} loss $\ell \in \cL$ within some collection, the optimal decision rule derived from $\pt$ is performatively optimal with respect to some class of hypothesis $\calH$.
% More formally:
\begin{definition}[Performative Omniprediction]
For input distribution $\D$, collection of loss functions $\cL$, hypothesis class $\Hcal$, and $\eps \ge 0$, a predictor $\pt:\Xcal \times \Ych \to [0,1]$ is an $(\cL,\Hcal,\eps)$-performative omnipredictor over $\D$ if for all $\ell \in \cL$, the optimal decision rule
$\ft_\ell$ is $(\ell,\Hcal,\eps)$-performative optimal.
\end{definition}
Omniprediction is a very strong solution concept.
Whereas the optimal decision rule typically depends intimately on the chosen loss, an omnipredictor needs to encode the optimal decision rule for every loss in $\cL$, even if these losses encode very different preferences over predictions.
It is not hard to see that the optimal predictor is an omnipredictor for any hypothesis and loss class.
\begin{corollary}
For any input distribution $\D$, collection of loss functions $\cL$, and hypothesis class $\Hcal$, the optimal predictor $p^*:\Xcal \times \Ych \to [0,1]$ is an $(\cL,\Hcal,0)$-performative omnipredictor over $\D$.
\end{corollary}
This corollary follows directly from Fact~\ref{fact:opt}, because the optimal predictor $p^*$ gives the true probability law governing the performative outcome distribution. 
Still, the optimal predictor may be of arbitrary complexity and is generally inaccessible.
The question remains whether \emph{efficient} performative omnipredictors exist, and if so, how to learn them.
To attack this question, we introduce a generalization of the outcome indistinguishability framework to the outcome performativity setting.

% While omniprediction is already a very strong guarantee in supervised learning, it becomes even more valuable in performative prediction. In classic supervised learning, most notions of accuracy are, at least qualitatively speaking, very similar.
% Consequently, the optimal decision rules for different loss functions that measure predictive accuracy, while not identical, are still qualitatively similar.
% In performative prediction however, there is a much larger design space. Losses do not just encode predictive accuracy, but also other concerns like the desire to steer outcomes towards more desirable states. Therefore, omnipredictors must simultaneously encode decision rules that have very different behavior. \jcpnote{mpk, thoughts on the example?}

% \begin{example}
% Consider the following highly stylized model for predicting whether an individual will default on a loan. There is a single feature $x=1$. Outcomes are $\cY= \{\pm1\}$ with 1 indicating that $x$ defaults on their loan and -1 denoting that $x$ has successfully repaid. Predictions $\cYh=\{\pm1\}$ are also binary, where predicting $\yhat = 1$ suggest that $x$ is likely to default. Assume that $\ps(x,\yhat) = 3/4 + 1/4 \cdot \yhat$, capturing the idea that predictions are self-fulfilling prophecies. 

% For $\cH = \{\pm \sign(x)\}$, if the goal is to be accurate $\ell(x, \yhat, \ys) = \ind\{\yhat \neq y\}$, then the optimal decision rule is $\sign(x) =1$. On the other hand, if the goal is to also nudge individuals to pay their loan $\ell(x, \yhat, \ys) = \ind\{\yhat \neq y\} + \ys+ 1$, then $-\sign(x)$ is optimal. 
% \end{example}




\subsection{Performative Outcome Indistinguishability}
Outcome Indistinguishability (OI) was introduced by \cite{oi} as an alternative paradigm for supervised learning.
Rather than focusing on loss minimization, OI formalizes learning as a computational indistinguishability condition.
In this view, a predictor should produce outcomes that are indistinguishable from Nature's outcome distribution.
While OI can encode classic learning goals like loss minimization, the abstraction is quite generic and amenable to modern supervised learning desiderata, like fairness \cite{hkrr} and distributional robustness \cite{ua}. 

Here, we propose an indistinguishability definition for the performative world.\footnote{In its original formulation, OI is a hierarchy of related notions. We generalize the framework to our setting, focusing on notions of performative OI that will imply performative omniprediction.  Understanding a full generalization of the OI framework to the performative setting is an interesting question for future investigations.}
This definition extends what \cite{gopalan2022loss} refer to as Hypothesis OI in the supervised setting.
%To define a distribution on outcomes, we need to specify a probability outcome model $\pt:\Xcal \times \Ych \to [0,1]$ as well as a decision rule $h:\Xcal \to \Ych$.
%Informally, a predictor $\pt$ satisifes OI if the expected risk of every decision rule $h\in \cH$ for every loss $\ell$ in a class $\cL$ is the same if $\yt \sim \pt(x,h(x))$ or if $\ys \sim \ps(x,h(x))$,
%%\jcpnote{this point needs to shine, it's the main point of departure from previous conceptions of OI. TBD whether this is best explained here or in the intro.}
%%\mpk{I agree. But let's hammer this home in the intro.}
%Performative OI requires this condition, not simply for a fixed decision rule, but simultaneously for each decision rule from a hypothesis class $\Hcal$.
\begin{definition}[Performative OI]
For input distribution $\D$, collection of losses $\cL$, hypothesis class $\Hcal$, and $\epsilon \ge 0$, a predictor $\pt:\Xcal \times \Ych \to [0,1]$ is $(\cL,\Hcal,\epsilon)$-performative outcome indistinguishable (POI) over $\D$ if for all $\ell \in \cL$ and all $h \in \Hcal$,
\begin{gather*}
   \big| \E_{\substack{x \sim \D\\\ys \sim \ps(x,h(x))}}[\ell(x,h(x),\ys)] -  \E_{\substack{x \sim \D\\\yt \sim \pt(x,h(x))}}[\ell(x,h(x),\yt)] \big| \leq \epsilon
\end{gather*}
\end{definition}
In this definition, we fix our collection of distinguishers to be parameterized by a collection of loss functions and a hypothesis class.
The POI condition states that, even when the outcome distribution can depend nontrivially on the hypothesis value $h(x)$, the outcomes $\ys$ and $\yt$ are indistinguishable, as measured by the expected loss of each hypothesis.
Note that the distinguishers take as input the individual $x$, the decision $h(x)$, and either Nature's outcome $\ys$ or the modeled outcome $\yt$.
In particular, these distinguishers do not receive access to the predictions $\pt(x,h(x))$ themselves.\footnote{In the language of \cite{oi}, this notion corresponds to the ``No-Access'' level of the OI hierarchy.  In principle, we could also extend the upper levels to the performative setting as well.  We comment this issue further within our discussion of performative calibration in Section~\ref{sec:calibration}.}

As a step towards obtaining omniprediction, we require indistinguishability between $\pt$ and $\ps$ not just under the reference decision rules $h$, but also under the optimal decision rules $\ft_{\ell}$ derived from $\pt$.
This motivates the notion of Performative Decision OI, which extends the idea of decision calibration, introduced in \cite{zhao2021calibrating}, and decision OI, introduced in \cite{gopalan2022loss}, to the performative setting.
\begin{definition}[Performative Decision OI]
For input distribution $\D$, collection of loss functions $\cL$, and $\epsilon \ge 0$, a predictor $\pt:\Xcal \times \Ych \to [0,1]$ is $(\cL,\epsilon)$-performative decision outcome indistinguishable (DOI) over $\D$ if for all $\ell \in \cL$,
\begin{gather*}
    \big| \E_{\substack{x \sim \D\\\ys \sim \ps(x,\ft_\ell(x))}}[\ell(x,\ft_\ell(x),\ys)] - \E_{\substack{x \sim \D\\\yt \sim \pt(x,\ft_\ell(x))}}[\ell(x,\ft_\ell(x),\yt)] \big| \leq \epsilon.
\end{gather*}
\end{definition}
Operationally, DOI allows us to sample outcomes $\yt \sim \pt(x,\ft_\ell(x))$ from our model of Nature, evaluate the expected loss of $\ell(x,\ft_\ell(x),\yt)$, and be confident that it is close to the loss on outcomes sampled from Nature $\ys \sim \ps(x,\ft_\ell(x))$.

Note that, technically, the indistinguishability conditions in Performative OI and Performative Decision OI look the same, but just refer to different hypothesis classes; that is, $(\cL, \eps)$-Performative Decision OI can be phrased as $(\cL, \set{\ft_\ell : \ell \in \cL}, \eps)$-Performative OI.
We make a distinction between these notions because, semantically, the hypothesis class $\set{\ft_\ell : \ell \in \cL}$ is derived from the predictor $\pt$, whereas $h \in \Hcal$ is independent of $\pt$.
As we will see later, this semantic difference manifests as a concrete difference in the computational complexity of achieving each notion of indistinguishability.

% Note that a model $\pt$ is $(\cL, \alpha)$-Performative Decision OI if and only if is $(\cL, \tilde{\cH}, \alpha)$-performative OI for the hypothesis class: $\tilde{\cH} = \{\ft_{\ell}: \ell \in \cL\}$. Nevertheless, we make this formal distinction because, as we will see later, there are meaningful differences in 
% the computational complexity of achieving indistinguishability for typical sets of hypothesis $\cH$ (e.g. decision trees) versus $\tilde{\cH}$.


\subsection{Performative Omniprediction via OI}
With these definitions in place, we can prove our first main result: performative omniprediction from performative outcome indistinguishability.
One of the main benefits of studying the problem from the indistinguishability lens is that it enables an especially clean and simple analysis.
The proof strategy we employ here follows the proof of omniprediction in the supervised learning world by \cite{gopalan2022loss}.
Curiously, the proof only needs one direction of the indistinguishability inequalities.
\begin{theorem}
\theoremlabel{thm:omni}
Fix an input distribution $\D$, collection of losses $\cL$, hypothesis class $\Hcal$, and $\epsilon \ge 0$.
Suppose that $\pt:\Xcal \times \Ych \to [0,1]$ is $(\cL,\epsilon)$-performative decision OI and $(\cL,\Hcal,\epsilon)$-performative OI.
Then, $\pt$ is a $(\cL,\Hcal,2\epsilon)$-performative omnipredictor.
\end{theorem}

\begin{proof}
The proof exploits the fact that for each loss $\ell \in \cL$, $\ft_\ell$ is the optimal decision rule for $\ell$ under $\pt$.
Fix a loss $\ell \in \cL$.
First, we upper bound the loss achieved by $\ft_\ell$ on real outcomes $\ys$ in terms of the loss on modeled outcomes $\yt$. Under  $(\cL, \epsilon)$-performative decision OI,
\begin{align*}
\E_{\substack{x \sim \D \\ \ys \sim \ps(x,\ft_{\ell}(x))}}[\ell(x, \ft_{\ell}(x),\ys)]
&\le \E_{\substack{x \sim \D\\\yt \sim \pt(x,\ft_{\ell}(x))}} [\ell(x, \ft_\ell(x),\yt)] + \epsilon. \label{ineq:calibration}
\end{align*}
Next, we relate the expected loss achieved by $\ft_\ell$ on modeled outcomes $\yt \sim \pt(x,\ft_\ell(x))$ versus that of other decision rules $h$.
By its definition, $\ft_\ell(x)$ is the optimal decision over any $\yhat \in \Ych$ for the loss $\ell(x,\yhat,\yt)$ under $\yt \sim \pt(x,\yhat)$.
So, averaging over the distribution on inputs $x \sim \D$, the loss of $\ft_\ell$ is upper bounded by the loss of any other decision rule $h$, and in particular those in $\Hcal$:
\begin{align*}
\E_{\substack{x \sim \D\\\yt \sim \pt(x,\ft_{\ell}(x))}} [\ell(x, \ft_\ell(x),\yt)] &\le \E_{\substack{x \sim \D\\\yt \sim \pt(x,h(x))}}[\ell(x, h(x),\yt)]. 
\end{align*}
Finally, by $(\cL,\Hcal,\eps)$-POI, we upper bound the loss achieved by $h$ on real outcomes $\ys$ by that achieved on modeled outcomes $\yt$.
\begin{align*}
\E_{\substack{x \sim \D\\\yt \sim \pt(x,h(x))}}[\ell(x, h(x),\yt)] &\le \E_{\substack{x \sim \D\\\ys \sim \ps(x,h(x))}}[\ell(x, h(x),\ys)] + \epsilon.
\end{align*}
Combining these three inequalities, 
\begin{gather*}
    \E_{\substack{x \sim \D \\ \ys \sim \ps(x,\ft_{\ell}(x))}}[\ell(x, \ft_{\ell}(x),\ys)] \le \E_{\substack{x \sim \D\\\ys \sim \ps(x,h(x))}}[\ell(x, h(x),\ys)] + 2\epsilon,
\end{gather*}
so $\pt$ is a $(\cL,\Hcal, 2\eps)$-performative omnipredictor.
\end{proof}




==> arxiv 2/predict_then_optimize.tex <==





==> arxiv 2/prelims.tex <==


%\section{Outcome Performativity}
%\label{sec:prelims}
%
%\paragraph{Outcome Performativity} Throughout our presentation, we will assume that features $x \in \calX$ are static and distributed according to some distribution $\calD$. Distributions are \emph{outcome} performative, and follows the data generating process:
%
%\begin{enumerate}
%	\item Sample $x \sim \calD$
%	\item Having observed $x$, declare prediction $\yhat \in \calYhat$
%	\item Sample $y \sim \ps(x, \yhat)$, where $\ps$ is conditional distribution of $y \in \calY$, given $x$ and $\yhat$.
%\end{enumerate}
%
%Outcome performativity can be described by the following causal graph:
%\begin{center}
%\begin{tikzpicture}[scale=0.2]
%\tikzstyle{every node}+=[inner sep=0pt]
%\draw [black] (30.7,-27.5) circle (3);
%\draw (30.7,-27.5) node {$\cX$};
%\draw [black] (38.7,-18.7) circle (3);
%\draw (38.7,-18.7) node {$\cYh$};
%\draw [black] (46.2,-27.5) circle (3);
%\draw (46.2,-27.5) node {$\cY$};
%\draw [black] (32.72,-25.28) -- (36.68,-20.92);
%\fill [black] (36.68,-20.92) -- (35.77,-21.18) -- (36.51,-21.85);
%\draw [black] (33.7,-27.5) -- (43.2,-27.5);
%\fill [black] (43.2,-27.5) -- (42.4,-27) -- (42.4,-28);
%\draw [black] (40.6,-21.3) -- (44.19,-25.27);
%\fill [black] (44.19,-25.27) -- (44.02,-24.34) -- (43.28,-25.02);
%\end{tikzpicture}
%\end{center}

 
 
 

==> arxiv 2/search.tex <==

\begin{figure}[t]
\setlength{\fboxsep}{2mm}
\begin{boxedminipage}{\textwidth}
\begin{center}
\underline{$\mathrm{Audit}(\cH, \cL, \alpha)$}
\end{center}
\vspace{2mm}
\textbf{If:} there exists $h \in \cH$ and $\ell \in \cL$ such that
	\begin{align*}
		\card{     \E_{\substack{x \sim \cD \\ \yt \sim \pt(x,h(x))}}[\ell(x, h(x),\yt)] - \E_{\substack{x \sim \cD \\ \ys \sim \ps(x,h(x))}}[\ell(x, h(x),\ys)]} \geq \alpha
	\end{align*}
\textbf{Then:} return  $h,l$  \\

\textbf{Else:} return $\mathsf{False} $
\end{boxedminipage}
\caption{The key step in the loss calibration procedure.}
\figurelabel{fig:search_template}
\end{figure}

\section{A Closer Look at Auditing}
\sectionlabel{sec:search}
The Indistinguishability Boosting algorithm is oracle-efficient. 
That is, it is guaranteed to work assuming there exists a statistically and computationally efficient algorithm for solving the auditing step defined in \equationref{eq:constraint}. 
Recall, the goal of the auditing problem is to 
determine whether there exists $h \in \cH$ and $\ell \in \cL$ such that the difference between nature's performative risk and the learner's performative risk under $\pt$ is large:
	\begin{align*}
		\card{     \E_{\substack{x \sim \cD \\ \yt \sim \pt(x,h(x))}}[\ell(x, h(x),\yt)] - \E_{\substack{x \sim \cD \\ \ys \sim \ps(x,h(x))}}[\ell(x, h(x),\ys)]} \geq \alpha.
	\end{align*}
So far, we've established how this problem can be naively solved by simply enumerating over all $h, \ell$ and non-adaptively computing their empirical risks on a single dataset of size $n \geq \mathcal{O}(\lmax |\cYh| \log(|\cH| |\cL| / \delta)\;/\; \alpha^2)$ at each iteration. However, this algorithm runs in time linear in $|\cH| |\cL|$ which may be prohibitively expensive for reasonable hypothesis classes.

In this section, we pay closer attention to the intricacies of implementing this auditing step and establish connections between this question and well-studied learning primitives. 

\subsection{Auditing via Cost-Sensitive Classification}

\jcpnote{The punchline is a reduction to cost sensitive learning which runs in time $|\cL| \cdot \mathrm{Time}(CSL)$}
To do so, we start by defining a generalization of this auditing problem. Let $\cH \subseteq \cX \rightarrow [k]$ be a hypothesis class and let $\cD$ be a distribution over $\cX \times [-1,1]^k$. If $(x,c) \sim \cD$ we refer to $c$ as the cost-vector where $c(j)$ is the $j$-entry of $c$.  


\begin{definition}(weak, agnostic cost-sensitive learning)
An algorithm $\cA$ is a $(\alpha, \gamma)$-??? if for any distribution $\cD$ over $\cX \times [-1,1]$, whenever it is promised that there is an $h \in \cH$ such that $\E c(h(x)) \geq \alpha$, $\cA$ returns a function $g: \cX \rightarrow [k]$ such that $\E c(h(x)) \geq \gamma$. 
\end{definition}

\begin{enumerate}
	\item this is weaker than cost sensitive classification
	\item cost sensitive classification is a well studied problem
	\item both in the theory (cite the MSR papers) and in practice vowpall wabbit
	\item In the binary case $\cYh = \{\pm 1\}$, this reduces to weak agnostic learning as defined in Michael's thesis. 
\end{enumerate} 

\subsection{Auditing via Weak Agnostic Learning}

\jcpnote{this isn't quite great either, you still end up running in time $\cH, \cL \cdot \mathrm{WeakLearn}(\cW)$ }




%\begin{figure}[t]
%\setlength{\fboxsep}{2mm}
%\begin{boxedminipage}{\textwidth}
%$$\underline{\mathrm{LinearSearch}(\cH, \cL, \alpha, n)}$$
%Collect dataset $S = \{(x, \yhat, \ys, \yt)_i\}_{i=1}^n$ of $n$ samples drawn i.i.d according to:
%$$x \sim \D,\; \yhat \sim \unif(\cYh),\; \ys \sim \ps(x,\yhat),\; \yt \sim \pt(x, \yhat)$$
%\textbf{For:} $(h,l) \in \cH' \times \cL$ where $\cH' = \cH \cup \{f_{\ell, p^{(t)}}: \ell \in \cL \}$
%\begin{itemize}
%	\item Compute empirical means:
%	\begin{align*}
%		\widetilde{\PR}(h,l) = \frac{|\cYh|}{n} \sum_{(x,\yhat, \yt) \in S} \ell(x, \yhat, \yt) \ind\{h(x) = \yt\}, \quad 
%		\hat{\PR}(h,l) = \frac{|\cYh|}{n} \sum_{(x,\yhat, \ys) \in S} \ell(x, \yhat, \ys) \ind\{h(x) = \ys\}
%	\end{align*}
%	\item \textbf{If: } $|\widetilde{\PR}(h,l) - \hat{\PR}(h,l)| \geq \alpha$ 
%	\textbf{Then: } return $h,l$\\
%\end{itemize}
%	
%Return $\mathsf{False} $
%\end{boxedminipage}
%\caption{Baseline implementation of the search step}
%\figurelabel{fig:linear_search}
%\end{figure}




==> arxiv 2/universality.tex <==

\section{Universal Adaptability}
\label{sec:ua}

In addition to minimizing expected risk, performative omniprediction can also be viewed as a guarantee of robustness.
So far, we've seen how a performative omnipredictor induces optimal predictions $\yhat$ even if these predictions lead to endogenous shifts in the distribution over outcomes $\ys$. 
In this section, we argue that with little additional work, the OI framework can be adapted to yield performative omnipredictors that are robust to exogenous shifts in the marginal distribution over individuals $x$.\footnote{By endogenous we mean that the distribution shift is caused by the act of prediction itself, which is considered in the outcome performativity framework. Exogeneous shifts are not influence by predictions. They refer to changes in the data distribution caused by factors like a change in external environment, or the passage of time.}

The results here build on the recent work of \cite{ua}, who introduced a notion of \emph{universal adaptability} in the context of statistical inference problems.
In our context, universal adaptability may be interpreted as a guarantee that the performative omnipredictor properties hold, not only on the original input distribution $\D$, but also on a broad family of shifts of this input distribution $\cD$.
In particular, we show that by augmenting the class of loss functions, we can learn an outcome prediction model $\pt$ that can handle exogenous shifts in the input distribution, while still maintaining performative optimality.

We parameterize universal adaptability  by a class of importance weight functions $\cW \subseteq \set{\Xcal \to \R_{\ge 0}}$.
For a base input distribution $\D$, we define a corresponding collection of shifted distributions $\D_{\cW}$ to be the set of distributions reachable after reweighting the probabilities in $\cD$ by some $\omega \in \cW$.
% \mpk{What assumptions do we need on $\D_{\cW}$?  Positivity?  Boundedness?  Making sure that $\omega$ actually yields a distribution?  Somehow, the error we incur should depend on the partition function or something.}
\begin{gather*}
    \D_{\cW} = \set{\D_\omega : \omega \in \cW, \; \supp(\D_\omega) \subseteq \supp(\cD) }, 
    \textrm{ where } \forall x \in \supp(\D_\omega),~~ \D_\omega(x) = \omega(x) \cdot \D(x) 
\end{gather*}
Note that to yield a valid probability distribution $\D_\omega$ it is necessary and sufficient that the importance weight function $\omega$ have unit weight over $\D$; that is, for any $\omega \in \cW$, $\E_{x \sim \D}[\omega(x)] = 1$.\footnote{Other properties of $\cW$ will affect whether universal adaptability is feasible, but not its definition.
We discuss these issues further in Section~\ref{sec:learning}.}
Given an importance weight class $\cW$, we say that an omnipredictor is universally adaptable if it is an omnipredictor over any $\D_\omega \in \D_{\cW}$.
% \mpk{do we hate this notation?  is there notation we hate less?}
\begin{definition}[Universal Adaptability]
For input distribution $\D$, weight class $\cW$, collection of losses $\cL$, hypothesis class $\Hcal$, and $\eps \ge 0$, a performative omnipredictor is $\cW$-universally adaptable over $\D$ if $\pt$ is an $(\cL, \Hcal, \eps)$-performative omnipredictor over every $\D_\omega \in \D_{\cW}$.
\end{definition}
Note that universal adaptability guarantees robustness under \emph{exogeneous} shifts in the marginal distribution over $\cX$, not under \emph{endogeneous} shifts in the input distribution induced by the act of prediction.
The distributional robustness is with respect to shifts that are defined in advance, independent of the chosen decision rule.
Under the guarantees of universal adaptability, the prevalence of various individuals may vary, but the response of any specific individual $x$ to a prediction $\yhat$, as measured by the distribution $\ps$ governing the outcome $\ys$, remains the same.
Intuitively, this type of robustness is the best that we can hope for without explicitly modeling how the predictions $\yhat \in \Ych$ change the distribution over individuals $x \in \Xcal$, which $\pt$ does not model. If predictions $\yhat$ affect both $x$ and $\ys$, it is not at all obvious to us what invariant property of Nature we should choose to model. We believe these are important questions for future work.
%\newcommand{\lamvec}{}

 One consequence of this adaptability definition is that any model $\pt$ that is an omnipredictor for a class of distributions $\D_{\cW}$ must also be an omnipredictor for any mixture distribution with components drawn from this class.  We say that a distribution $\cD_{m}$ is a mixture distribution if for all $x \in \cX$, 
\begin{align*}
	\Pr_{\cD_m}[X=x] = \sum_{\omega} \lambda_\omega \Pr_{\cD_\omega}[X=x]  \text{ where } \cD_\omega \in \cD_{\cW},\; \lambda_\omega \geq 0 \text{ for all } \omega \text{ and } \sum_\omega \lambda_\omega=1.
\end{align*}
We denote by $\mathsf{mixt}(\cD_{\cW})$ the set of all such mixture distributions $\D_m$.
 
 
\begin{proposition}
\propositionlabel{prop:mixtures}
Let $\cD_\cW$ be a set of distributions over $\cX$. If $\pt$ is a $(\cL, \cH, \epsilon)$-performative omnipredictor over every $\cD_\omega \in \cD_{\cW}$, then it is also a $(\cL, \cH, \epsilon)$-performative omnipredictor over every $\cD_m$ in $\mathsf{mixt}(\cD_{\cW})$.
\end{proposition}
\begin{proof}
Fix a loss $\ell \in \cL$, a hypothesis $h \in \cH$ and a distribution $\cD_m$ in $\mathsf{mixt}(\cD_{\cW})$. Then,
\begin{align*}
\E_{\substack{x \sim \D_m \\ \ys \sim \ps(x,\ft_{\ell}(x))}}[\ell(x, \ft_{\ell}(x),\ys)] &= \sum_\omega \lambda_\omega \cdot \E_{\substack{x \sim \cD_i \\ \ys \sim \ps(x,\ft_{\ell}(x))}}[\ell(x, \ft_{\ell}(x),\ys)]  \\ 
& \leq \sum_\omega \lambda_\omega \cdot \E_{\substack{x \sim \cD_\omega \\ \ys \sim \ps(x,h(x))}}[\ell(x, h(x),\ys)] + \sum_\omega \lambda_\omega \epsilon \\
& = \E_{\substack{x \sim \D_m \\ \ys \sim \ps(x,h(x))}}[\ell(x, h(x),\ys)] + \epsilon
\end{align*}
The first line follows by expanding the definition of the mixture distribution and the second by the omniprediction guarantee on mixture components. In the last line we again applied the definition of a mixture and the fact that the $\lambda_\omega$ sum to 1. Because the inequalities hold for every $h\in \cH$, it must be the case that $\pt$ is an $(\cL, \cH, \epsilon)$-omnipredictor for every mixture distribution .
\end{proof}



% \begin{itemize}
%     \item Omniprediction:  shows that we can get optimality, under different rules of optimality, even when the distribution over outcomes is effected by our decisions
%     \item In this sense, an omnipredictor is robust to shifts in the outcome distribution cause by our predictions
%     \item Here, we argue that the OI framework can be adapted to yield omnipredictors that are robust to shifts in the input distribution as well.
%     \item This builds on recent work of \cite{ua}, who introduced a notion of \emph{universal adaptability} in the context of statistical estimation.
%     \item In our context of omniprediction, we argue that by augmenting the loss class, we can anticipate shifts in the distribution, and still maintain performative optimality.
%     \item Note, this comes short of handling performativity in the input distribution.  The shifts we are robust to must be defined in advance, independent of the predictions we choose.
%     \item This is the best we can hope for, without explicitly modeling the shift in the distribution over $\Xcal$, which our outcome predictor $\pt$ does not model.
% \end{itemize}

We establish universal adaptability for performative omnipredictors by augmenting the loss class $\cL$ using the weight class $\cW$.
Specifically, we define the augmented loss class $\cL_\cW$ as the class of losses $\ell \in \cL$ reweighted by importance weight functions $\omega \in \cW$.
\begin{gather*}
    \cL_{\cW} = \set{\ell_\omega : \ell \in \cL,\ \omega \in \cW}\\
    \textrm{where }\forall x \in \Xcal,\yhat \in \Ych,y \in \cY:~~~ \ell_\omega(x,\yhat,y) = \omega(x) \cdot \ell(x,\yhat,y)
\end{gather*}
With this class of losses in place, we argue that universally-adaptable performative omniprediction is, again, a consequence of performative outcome indistinguishability.
\begin{proposition}
\proplabel{prop:adaptability}
For a base input distribution $\D$, weight class $\cW$, collection of losses $\cL$, hypothesis class $\Hcal$, and $\eps \ge 0$, if a predictor $\pt$ is $(\cL_{\cW},\Hcal,\eps)$-performative OI and $(\cL_\cW,\eps)$-performative decision OI over $\D$, then $\pt$ is an $(\cL,\Hcal,2 \eps)$-performative omnipredictor that is $\cW$-universally adaptable over $\D$.
\end{proposition}
\begin{proof}
The proposition follows as a corollary of \theoremref{thm:omni}.
The key observation is that multiplying by the importance weight $\omega(x)$ allows us to switch from an expectation over $\D$ to an expectation over $\D_\omega$.
By the definition of $\D_\omega$, we have that for supported $x \in \Xcal$, $\omega$ is the odds ratio,
\begin{gather*}
    \omega(x) = \frac{\D_\omega(x)}{\D(x)}.
\end{gather*}
Further, by the definition of $\ell_\omega$, for any $h:\Xcal \to \Ych$ and any outcome probability model $p$, the following equality of expectations holds
\begin{gather}
\equationlabel{eqn:reweight}
    \E_{\substack{x \sim \D\\y \sim p(x,h(x))}}[\ell_\omega(x,h(x),y)]
    = \E_{\substack{x \sim \D\\y \sim p(x,h(x))}}[\omega(x) \cdot \ell(x,h(x),y)]
    = \E_{\substack{x \sim \D_\omega\\y \sim p(x,h(x))}}[\ell(x,h(x),y)],
\end{gather}
where we rely on the identity that for any function $g:\Xcal \to \R$,
\begin{gather*}
    \E_\D[g(x) \cdot \omega(x)] = \E_\D[g(x) \cdot \D_\omega(x)/\D(x)] = \E_{\D_\omega}[g(x)].
\end{gather*}
The equality in \equationref{eqn:reweight} immediately implies that if $\pt$ is $(\cL_\cW,\Hcal,\eps)$-POI over $\D$, then $\pt$ is $(\cL,\Hcal,\eps)$-POI over every $\D_\omega \in \D_\cW$.
That is, by applying the identity to the expectation under Nature's outcomes $\ys \sim \ps(x,h(x))$ and separately to the expectation under the modeled outcomes $\yt \sim \pt(x,h(x))$, $(\cL_\cW,\Hcal,\eps)$-performative OI imples that we obtain indistinguishability for all $\ell \in \cL, h \in \Hcal$ and $\D_\omega \in \D_\cW$:
\begin{gather*}
\big|\E_{\substack{x \sim \D_\omega\\\ys \sim \ps(x,h(x))}}[\ell(x,h(x),\ys)]
-
\E_{\substack{x \sim \D_\omega\\\yt \sim \pt(x,h(x))}}[\ell(x,h(x),\yt)] \big| \leq \epsilon.
\end{gather*} 
The corresponding statement for performative decision OI is a bit more subtle.
Whereas above, the decision rules $h \in \Hcal$ do not depend in any way on $\omega$, the optimal decision rule $\ft_{\ell_\omega}$ based on $\pt$, is allowed to depend on the specified loss and, thus, on $\omega$.
Still, we argue that for any $\omega$, $\ft_{\ell_\omega} = \ft_\ell$.
This equality follows by the fact that the optimal decision rule is chosen pointwise, for each $x \in \Xcal$.
In particular, for all $x \in \Xcal$, scaling the loss by $\omega(x)$ changes the scale of the optimization, but not the minimizer:
\begin{gather*}
    \ft_{\ell_\omega}(x) = \argmin_{\yhat \in \Ych} \E_{y \sim \pt(x,\yhat)}[\omega(x) \cdot \ell(\yhat,y)] = \argmin_{\yhat \in \Ych} \E_{y \sim \pt(x,\yhat)}[\ell(\yhat,y)] = \ft_{\ell}(x).
\end{gather*}
Thus, the same identities from above can be applied to prove that if $\pt$ is $(\cL_\omega,\eps)$-DOI for a fixed distribution $\cD$, then it is also $(\cL, \epsilon)$-DOI for every $\D_\omega \in \D_\cW$.
The proposition follows by applying \theoremref{thm:omni} separately over each $\D_\omega \in \D_\cW$.
\end{proof}

Before moving on, we highlight that designing omnipredictors requires the learner to account for possible shifts in the distribution at \emph{training} time, not at test time. At test time, the learner simply chooses predictions $\yhat$ according to the function $\ft_\ell$, without needing to first infer what the underlying distribution $\cD$ may be. The decision rule $\ft_\ell$ is simultaneously optimal for all of them. 
This design choice shifts the burden of technical sophistication and expertise from the user of the system to its designer. The user is free to focus on the choice of loss function $\ell$ to balance between forecasting and steering knowing that naive usage of $\ft_\ell$ is guaranteed to work.


% The proof follows directly from the observation regarding importance weighting in \eqref{eq:ip_weights} and the relationship between performative outcome indistinguishability and omniprediction outlined in Theorem \ref{thm:omni}. If $\pt$ is $(\cL_\omega, \cH, \epsilon)$-POI and $(\cL_\omega, \epsilon)$-DOI over $\cD$, then by the previous theorem, for all $\ell_\omega \in \cL_\omega$, 
% \begin{align}
% \label{eq:universality_proofeq}
%     \E_{\substack{x \sim \cD \\ \ys \sim \ps(x,\ft_{\ell}(x))}}[\ell_\omega(x, \ft_{\ell}(x),\ys)] \leq \min_{h \in \cH} \E_{\substack{x \sim \cD \\ \ys \sim \ps(x,h(x))}}[\ell_\omega(x, h(x),\ys)] + 2\eps.
% \end{align}
% Here, we used the fact that $\ft_{\ell} = f_{\ell_\omega, \pt}$ for all $\omega$ since the post-processing is unaffected by the reweighting.

% By definition of $\cL_\omega$, for any distribution $\cD' \in \cS(\cW; \cD)$ and loss $\ell \in \cL$, there exists a function $\ell_\omega \in \cL_\omega$ such that for any $h: \cX \rightarrow \cYh$ (not necessarily belonging to $\cH$) and predictors $p$, 
% \begin{align*}
% \E_{\substack{x \sim \cD \\ y \sim p(x,h(x))}}[\ell_\omega(x, h(x),y)] = \E_{\substack{x \sim \cD \\ y \sim p(x,h(x))}}[\ell(x, h(x), y) \omega(x)]  = \E_{\substack{x \sim \cD' \\ y \sim p(x,h(x))}}[\ell(x, h(x), y)]. 
% \end{align*}
% Applying this identity to both sides of Equation \ref{eq:universality_proofeq}, we get that for any distribution $\cD'$ and loss $\ell$,
% \begin{align*}
%     \E_{\substack{x \sim \cD' \\ \ys \sim \ps(x,f_{\ell_{\omega}, \pt}(x))}}[\ell(x, f_{\ell_{\omega}, \pt}(x),\ys)] \leq \min_{h \in \cH} \E_{\substack{x \sim \cD' \\ \ys \sim \ps(x,h(x))}}[\ell(x, h(x),\ys)] + 2\eps.
% \end{align*}
% \end{proof}
















% These robustness to covariate shift can be derived from the following simple observation. Let $\cD$ and $\cD'$ be two discrete distributions over a finite set $\cX$. It's a well-known fact that given a function $\omega:  \cX \rightarrow \R_{\geq 0}$ such that $\supp(\cD') \subseteq \supp(\cD)$ and for which,
% \begin{align*}
% 	\omega(x) = \frac{\Pr_{\cD'}[X=x]}{\Pr_{\cD}[X=x]},
% \end{align*}
% for all $x \in \supp(\cD)$, it holds that for any loss function  $\ell: \cX \rightarrow \R$,
% \begin{align}
% \label{eq:ip_weights}
% 	\E_{x \sim \cD} g(x) \omega(x) = \E_{x \sim \cD'} g(x).  
% \end{align} 
% By ensuring that our model of nature $\pt$ is indistinguishable from nature even if we include these ``importance weights'' $\omega$ as part of the set of test functions, we can prove that our omnipredictors are universally usable across contexts where the marginal distribution over $\cD$ may vary.

% To prove this formally, for a collection of importance weights $\cW \subseteq \cX \rightarrow \R$ and base distribution $\cD$, we define the corresponding set of represented distributions $\cS(\cW;\cD)$ as 
% \begin{align}
% \label{eq:induced_dists}
% 	\cS(\cW; \cD) \defeq \{\cD': \exists \omega \in \cW \text{ s.t for all } x\in \supp(\cD), \omega(x) = p_{\cD'}(x) / p_{\cD}(x) \}.
% \end{align}
% Next, we define the concept of a universal omnipredictor:

% \begin{definition}[Universal Omnipredictor]
% Let $\cL$ be a collection of loss functions, $\cH$ a hypothesis class, and $\cP$ a set of distributions over $\cX$.
% For $\eps \geq 0$, a predictor $\pt$ is an $(\cP,\cL,\cH, \eps)$-universal performative omnipredictor if for every distribution
% $\D$ and all $\ell \in \cL$, the optimal decision rule
% $\ft_\ell$ is $(\ell,\Hcal,\eps)$-performative optimal over $\cD$:
% \begin{align*}
%     \E_{\substack{x \sim \cD \\ \ys \sim \ps(x,\ft_{\ell}(x))}}[\ell(x, \ft_{\ell}(x),\ys)] \leq \min_{h \in \cH} \E_{\substack{x \sim \cD \\ \ys \sim \ps(x,h(x))}}[\ell(x, h(x),\ys)] + \eps.
% \end{align*}
% \end{definition}
% Using these definitions, we can formalize the intuition from \eqref{eq:ip_weights} and show to achieve universal omniprediction by augmenting the set of losses for which $\pt$ is performatively outcome indistinguishable. 
% %However, before presenting our main result for this section, we first establish the following lemma showing how these  
% \begin{corollary}
% 	Let $\cW$ be a class of importance weight functions, $\cL$ be a set of losses, and $\cH$ a hypothesis class. Define $\cL_\omega$ to be the set of losses
% \begin{align}
% \label{eq:lomega_def}
% 	\cL_{\omega} \defeq \{ \ell_{\omega}: \exists (\ell, \omega) \in \cL \times \cW \text{ s.t }\ell_{\omega}(x, \yhat, y) = \ell(x, \yhat, y) \cdot \omega(x) \text{ for all } x, \yhat, y \}.
% \end{align}
% If $\pt$ is $(\cL_\omega, \cH, \epsilon)$-performative OI and $(\cL_\omega, \epsilon)$-performative decision OI over a fixed distribution $\cD$, then $\pt$ is a $(\cS(\cW,\cD),\cL,\cH, 2\eps)$-universal omnipredictor. 
% \end{corollary}





%This universality result can in fact be made even stronger without any additional assumptions by leveraging the fact that











%The overarching goal of our work is to simple, yet powerful, approaches for algorithmic decision making under outcome performativity. 
%Omniprediction takes a step towards this direction by enabling decision-makes to act optimally for a loss function of their own choosing. 
%Here we take an additional step and show how, with only minor additional work, the same technical machinery presented so far can be used to guarantee that the decision rules $\ft$ are optimal not just for a fixed distribution over individuals, $\calD$, but for many. 

%If we think of the elements $\cD_j$ as distributions over individuals in particular communities, like say states in the US, this result says that any predictor which satisfies the POI (and DOI) conditions for each state separately, is an omnipredictor for any population composed of a mixture of individuals from different states.
%By establishing these indistinguishability guarantees for a small number of reference distributions, one ends up with universal omnipredictor a for a much richer class of marginal distributions. 

%A couple of other points are worth noting. First, we use universality to indicate that these omniprediction guarantees are robust to covariate shift. However, while the marginal distribution over features $\cX$ may change, the conditional distribution of $\cY$ given $x$ and $\yhat$ is assumed to be invariant. Intuitively, this corresponds to the assumption that  while the prevalence of various individuals may vary, the response (as measured by $\ys$) of any specific individual $x$ to a prediction $\yhat$ is the same across communities. 



%As a final note, one might hope that the closure property discussed in \lemmaref{lemma:linear combinations} could lead to a strengthening of the omniprediction result from the previous section. This is unfortunately not true. While the POI condition is closed under linear combination, performative decision OI is not since adding new losses may introduce new decision rules $\ft_\ell$. See \textcolor{red}{???} for more discussion. 

%\jcpnote{these previous paragraphs will need to be updated depending on what's in the intro}














==> indistinguishability.tex <==


\newpage


\begin{figure}[t]
\setlength{\fboxsep}{2mm}
\begin{boxedminipage}{\textwidth}
\begin{center}
{\centering{\underline{Indistinguishability Boosting}}}
\end{center}

\vspace{2mm}
{\bf Input:} Set of losses $\cL$, hypotheses $\cH$, distribution $\cD$, tolerance $\alpha > 0$\\
\vspace{-2mm}

{\bf Initialize:} $p^{(1)}(x,\yhat) \in \Delta(\cY)$ for all $x$ and $\yhat$ \\

{\bf For:} $t = 1,2, \ldots$
\begin{itemize}
	\item {\bf If:} there exists $\bar{h} \in \cH \cup \{f_{\ell, t}: \ell \in \cL \}$ and $\bar{\ell} \in \cL$ such that
	\begin{align}
	\equationlabel{eq:constraint}
		| \underbrace{\E_{\substack{x \sim \cD \\ \yt \sim \pt(x,\bar{h}(x))}}[\bar{\ell}(x, \bar{h}(x),\yt)] - \E_{\substack{x \sim \cD \\ \ys \sim \ps(x,\bar{h}(x))}}[\bar{\ell}(x, \bar{h}(x),\ys)]}_{\nabla} | \geq \alpha
	\end{align}
	{\bf Then:} update the model $p^{(t)}$, for all $x, \yhat$
	\begin{align}
	\label{eq:predictor_update_rule}
		p^{(t+1)}(x,\yhat) \leftarrow \Pi \left( p^{(t)}(x,\yhat) - \eta^{(t)} \left[\bar{\ell}(x, \bar{h}(x), 1) - \bar{\ell}(x, \bar{h}(x),0) \right] \ind\{h(x) = \yhat\} \right)
	\end{align}
% TO INCLUDE general categorical case update rule

%	\begin{align}
%	\label{eq:predictor_update_rule_2}
%		p^{(t+1)}(x,\yhat) \leftarrow p^{(t)}(x,\yhat) - \eta^{(t)} \begin{bmatrix}
%			\ell(x, h(x), y_1) \\ 
%			\dots\\
%		    \ell(x, h(x), y_k)
%		\end{bmatrix} \ind\{h(x) = \yhat\}
%	\end{align}
	where $\eta_t = - \sign(\nabla) \; / \; \lmax$

	\item {\bf Else:} terminate and return $p^{(t)}$
\end{itemize}
\vspace*{2mm}
\end{boxedminipage}

\caption{\label{fig:algorithms} Algorithm for generating performatively outcome indistinguishable predictors. Correctness and runtime are analyzed in \propref{prop:loss_calibration_analysis}. For the sake of clarity, here we present the simplest version of the algorithm where $\cYh = \{0,1\}$ is binary and the search outlined in \equationref{eq:constraint} is proper. Both of these conditions can be relaxed as we explore in \sectionref{sec:search}.}
\end{figure}














\section{Performative Outcome Indistinguishability}

Our approach towards achieving decision rules which are simultaneously optimal for a wide variety of losses and marginal distributions over features is centered around achieving the following indistinguishability definition. 

Performative outcome indistinguishability, as we define it below, is a property of a model of nature $\pt$, which captures the probabilities of outcomes in $\cY$, for every individual $x$ and (performative) prediction $\yhat$. 
Intuitively, the condition asserts that, when viewed from the perspective of a particular set of test functions and decision rules, the expected values of these functions under nature and the learner's model of nature are approximately indistinguishable.

\begin{definition}[Performative Outcome Indistinguishability]
Suppose $\cL$ is a collection of loss functions and $\cH$ is a hypothesis class.
For a given tolerance $\eps \geq 0$, a predictor $\pt$ is $(\cL,\cH,\eps)$-performatively outcome indistinguishable (or POI for short) if for all $\ell \in \cL$ and for all $h \in \cH$,
\begin{align}
    \card{\E_{\substack{x \sim \D\\\yt \sim \pt(x,h(x))}}[\ell(x, h(x),\yt)] - \E_{\substack{x \sim \D\\\ys \sim \ps(x,h(x))}}[\ell(x, h(x),\ys)]} \le \eps.
\end{align}
Furthermore, we say that $\pt$ is $(\cL,\cH,\eps)$-reflexively POI if it is $(\cL,\cH',\eps)$
-calibrated for 
\begin{align}
\cH' = \cH \cup \{\ft_{\ell}: \ell \in \cL \}.
\end{align}
\end{definition}

Relative to initial work on outcome indistinguishability (OI) in supervised learning which defines indistinguishability in terms of an abstract class of binary-valued distinguishers, our definition of performative outcome indistinguishability is somewhat more pragmatic. 
It ensures that nature and the learner's model are close in terms of the downstream metrics (the expected risks for a choice of loss and hypothesis) which will ultimately decide whether a predictor is useful or not for a particular application.

Like previous definitions however, this indistinguishability condition can be efficiently achieved assuming the learner can solve a particular search problem, closely related to weak agnostic learning. 
As we now show, one can extend the algorithm from [??? \jcpnote{@mpk}], to nonparametrically construct a predictor $\pt$ which achieves this definition. 
For the sake of simplifying the exposition, we again focus on the case where $\cY$ is binary. Extensions to the general case where $\cY$ is categorical are straightforward (see Appendix ???).

\begin{proposition}
\proplabel{prop:loss_calibration_analysis}
The Indistinguishability Boosting algorithm described in Figure 1 terminates in at most $  \lmax^2 |\cYh| \;/\; \alpha^2$ many iterations and returns a predictor $\pt$ that is
$(\cL, \cH, \alpha)$-self-calibrated. 
\end{proposition}
\begin{proof}
The fact that $\pt$ is reflexively-POI follows directly from the termination criteria. 
To prove the algorithm terminates, the key insight is that if the indistinguishability constraint is violated for any $l$ or $h$, then we will have made nontrivial progress on a common potential function. 
Since this potential is bounded from above and below, and bounded progress is guaranteed with every update, the total number of updates must be bounded. 
We now make this argument formal.
First, note that for any predictor $p$, loss $\ell$, and hypothesis $h$,
\begin{align*}
	\E_{\substack{x \sim \D\\ y \sim p(x,h(x))}} \ell(x, h(x), y) &= \E_{x} \E_{y\mid x} \ell(x, h(x), y) \\
	&= \E_x \ell(x, h(x), 1)p(x,h(x)) + \ell(x, h(x),0)(1 - p(x, h(x))) \\ 
	&= \E_{x}\ell(x, h(x),0) + \left(\ell(x, h(x), 1) - \ell(x, h(x), 1)\right) p(x,h(x)).
\end{align*}
Hence, the difference between any two predictors $p$ and $p'$ (and in particular for $p^{(t)}$ and $\ps$) can be expanded as:
\begin{align*}
	\E_{\substack{x \sim \D\\ \yt \sim \pt(x,h(x))}} \ell(x, h(x), \tilde{y}) - \E_{\substack{x \sim \D\\ \ys \sim \ps(x,h(x))}} \ell(x, h(x), y_*) &= \E_{x} \left(\ell(x, h(x),1) - \ell(x, h(x), 0)\right)\left(\pt(x, h(x)) - \ps(x, h(x))\right) \\ 
	& = \underbrace{\sum_{\yhat} \E_x \left(\ell(x,\yhat,1) - \ell(x,\yhat', 0)\right)\left(\pt(x, \yhat) - \ps(x, \yhat)\right) \ind\{h(x) = \yhat\}}_{\defeq \nabla_t} 
\end{align*}
Now, consider the potential:
\begin{align*}
 \sum_{\yhat} \E_x \left(p^{(t+1)}(x,\yhat) - \ps(x,\yhat)\right)^2 = 	\sum_{\yhat} \E_x \left(\Pi \left(p^{(t)}(x,\yhat)  - \eta \left[\ell(x, h(x), 1) - \ell(x, h(x),0) \right] \ind\{h(x) = \yhat\} \right) -
 \ps(x,\yhat)\right)^2.
\end{align*}
Because projection can only decrease the distance to $\ps$, if an update is performed, the difference between potentials at adjacent time steps,
\begin{align*}
	\sum_{\yhat} \E_x \left(p^{(t+1)}(x,\yhat) - \ps(x,\yhat)\right)^2 - \sum_{\yhat} \E_x \left(p^{(t)}(x,\yhat) - \ps(x,\yhat)\right)^2,
\end{align*}
is upper bounded by 
\begin{align*}
-2 \eta \underbrace{\sum_{\yhat}\E_x(\ell(x,\yhat, 1) - \ell(x, \yhat, 0))  \left(p^{t}(x,\yhat) - \ps(x, \yhat)\right) \ind\{h(x) = \yhat\}}_{\nabla_t} + \eta^2 \underbrace{ \sum_{\yhat}\E_x(\ell(x,\yhat, 1) - \ell(x, \yhat, 0))^2 \ind\{h(x) = \yhat\}}_{\defeq B}.
\end{align*}
From this rewriting, since $\nabla_t \geq \alpha$ by the search criterion in \equationref{eq:constraint} and $|B| \leq \lmax^2$, the difference between potentials satisfies:
\begin{align*}
	\sum_{\yhat} \E_x \left(p^{(t+1)}(x,\yhat) - \ps(x,\yhat)\right)^2 - \sum_{\yhat} \E_x \left(p^{(t)}(x,\yhat) - \ps(x,\yhat)\right)^2 = -2 \eta_t \Delta_t + \eta^2 B \leq -\alpha^2 / \lmax^2
\end{align*}
Hence, the potential must decrease by at least $\alpha^2 / \lmax^2
$ per iteration. Since the potential is lower bounded by 0, upper bounded by $|\cYh|$, and we improve by $\alpha^2 / \lmax^2$ each time, the algorithm is guaranteed to terminate in at most $\lmax^2 |\cYh| / \alpha^2$ many iterations.
\end{proof}

\subsection{Statistical Complexity of Performative Outcome Indistinguishability}

The previous proposition shows that one can efficiently construct a POI predictor $\pt$ with at most a moderately small number of calls to an algorithm which implements the search step outlined in \equationref{eq:constraint}. This begs the question, what are the statistical and computational complexities of solving this search problem? 

Here, we focus on the statistical considerations and delay the discussion on computation for \sectionref{sec:search}. Interestingly, this weak learning problem can be solved using a single exploratory dataset in which predictions are chosen randomly for every $x$:

\begin{proposition}
There exists an algorithm  which given $n \geq \mathcal{O}(\lmax |\cYh|\log(|\cH| |\cL| / \delta)/ \alpha^2)$ samples drawn according to $x\sim \cD, \yhat \sim \unif(\cYh), \ys \sim \ps(x,\yhat)$
implements the search step outlined in \equationref{eq:constraint} with probability $1-\delta$  and runs in time $\mathcal{O}(|\cH| |\cL| n)$.
\end{proposition}

\begin{proof}
The algorithm just runs a for loop and computes the empirical mean of the performative risk for each $h$ and $\ell$. 
Crucially, this can be done off of a single exploratory dataset.
By \lemmaref{lemma:static}, for any hypothesis $h$ and loss $\ell$, the performative risk of $h$ over $\ell$ can be written as the expected risk of a modified objective over distribution that is independent of $h$:
\begin{align*}
\E_{\substack{x \sim \calD_x \\ \ys \sim \ps(x,h(x))}} \ell(x, h(x), \ys) = |\calYhat| \E_{\substack{x \sim \calD_x \\ \yhat \sim \Unif(\calYhat) \\ \ys \sim \ps(x,\yhat)}} \ell(x, \yhat, \ys )\ind \{h(x) = \yhat\}.
\end{align*}	
Since $|\cYh| \cdot \ell(x, \yhat, y)$ is uniformly bounded by $|\cYh| \cdot \lmax$, Hoeffding's inequality guarantees that given $n \geq |\cYh| \cdot  \infn{\cL} / (2\alpha^2) \log(2 /\delta)$ many samples, the empirical mean of the right hand side (over $n$ samples) is $\alpha$ close to its expectation. To get uniform convergence over all $\ell \in \cL$ and $h \in \cH$ it suffices to apply a union bound.
\end{proof}

From this result, we see that at least naively, a total of $\mathcal{O}(\lmax^3 |\cYh|^2 \log(|\cH| |\cL| / \delta)\;/\; \alpha^4)$ many ``RCT'' samples, where $\yhat \sim \unif(\cYh)$ for every $x$, are sufficient to compute a predictor $\pt$ which is $(\cL, \cH, \epsilon)$ performatively outcome indistinguishable. 

\jcpnote{There are of course better ways of getting this concentration analysis to go through (e.g Bernstein's, VC dimension, etc.). Getting the sharpest concentration result doesn't seem to me the main focus on this paper, but we should make a remark to that end.}





==> mc.tex <==









% \begin{definition}[Performative Multicalibration]
% A predictor $\pt:\Xcal \times \Ych \to [0,1]$ is $(\Hcal,\alpha)$-multicalibrated under performativity if for all $h \in \Hcal$, $\yhat \in \Ych$, and all $v \in \supp(\pt)$,
% \begin{gather*}
%     \card{\E_{\substack{x \sim \D\\\ys \sim \ps(x,\yhat)}}[h(x) \cdot \1[\pt(x,\yhat) = v] \cdot (\ys - v)]} \le \alpha.
% \end{gather*}
% \end{definition}


\begin{definition}[Performative Multicalibration]
For a hypothesis class $\Hcal$ and approximation parameter $\alpha \ge 0$, a predictor $\pt$ is $(\Hcal, \alpha)$-multicalibrated under performativity if for all $h \in \Hcal$ and all $v \in \supp(\pt)$
% \begin{gather*}
%     \E_{\substack{x \sim \D\\\ys \sim \ps(x,\yhat)}}[h(x) \cdot \omega(\pt(x,\yhat)) \cdot (\ys - \pt(x,\yhat))] \in [-\alpha,\alpha].
% \end{gather*}
\begin{gather*}
    \E_{\substack{x \sim \D\\\ys \sim \ps(x,h(x))}}[h(x) \cdot \1_v[\pt(x,h(x))] \cdot (\ys - \pt(x,h(x)))] \approx_\alpha 0.
\end{gather*}
\end{definition}


Useful:  assume that $\Hcal$ contains all constant hypotheses.
That is, we obtain some version of calibration from multicalibration:  for all $\yhat \in \Ych$
\begin{gather*}
    \E_{\substack{x \sim \D\\\ys \sim \ps(x,\yhat)}}[\1_v[\pt(x,\yhat)] \cdot (\ys - \pt(x,\yhat)] \approx_\alpha 0
\end{gather*}



\paragraph{Proof of Convex Omniprediction:}
\begin{proof}
Assumptions:  $\pt$ is a predictor that satisfies
\begin{itemize}
    \item Bounded support size $\card{\supp(\pt)} = s$
    \item $\alpha/s$-calibrated
    \item $(\Hcal,\alpha/s)$-multicalibrated
\end{itemize}
For any convex loss $\ell$, we need to show the following inequality holds:
\begin{gather*}
    \E_{\substack{x \sim \D\\\ys \sim \ps(x,f_\ell(x))}}[\ell(f_\ell(x),\ys)] \le \E_{\substack{x \sim \D\\\ys \sim \ps(x,h(x))}}[\ell(h(x),\ys)] + \eps
\end{gather*}
for $\eps \le 10\alpha$.
We go step by step.

First, we switch our view from a loss over $\ys$ to one over $\yt$.  In particular, (\ref{eqn:yt:calibration}) follows under calibration.
\begin{gather}\label{eqn:yt:calibration}
    \E_{\substack{x \sim \D\\\ys \sim \ps(x,f_\ell(x))}}[\ell(f_\ell(x),\ys)]
    \approx_\alpha \E_{\substack{x \sim \D\\\yt \sim \pt(x,f_\ell(x))}}[\ell(f_\ell(x),\yt)]
\end{gather}
Then, by the optimality of $f_\ell$, we can switch our view to any predictor that could also be derived from $\pt$.
Specifically, consider the function $h_\ell$ defined as
\begin{gather*}
    h_\ell(v) = \argmin_{\yhat \in \Ych} \E_{y_v\sim \Ber\left(\E[h(x) \vert \pt(x,\yhat) = v]\right)}[\ell(\yhat,y_v)]
\end{gather*}
\mpk{A bit suspect, but maybe not wrong?
The point is that we want to ensure that the policy we come up with is constant on the level sets of $\pt$.
In this case, calibration should save us?
Importantly, $y$-performativity is decomposable across units, so we can mix and match the calibration constraints for each $v \in \supp(\pt)$ regardless of what $\yhat$ is actually chosen.
}

\end{proof}





% Different weight classes correspond to specific multi-group notions.
% \begin{itemize}
%     \item $\Wcal = \set{1}$:  $(\Hcal,\alpha)$-multiaccuracy
%     \begin{gather*}
%     \E_{\substack{x \sim \D\\\ys \sim \ps(x,\yhat)}}[h(x) \cdot (\ys - \pt(x,\yhat))] \approx_\alpha 0
%     \end{gather*}
%     \item $\Wcal = \set{1,\mathrm{id}}$:  ``Degree-2'' $(\Hcal,\alpha)$-multicalibration
%     \begin{gather*}
%     \E_{\substack{x \sim \D\\\ys \sim \ps(x,\yhat)}}[h(x) \cdot \pt(x,\yhat) \cdot (\ys - \pt(x,\yhat))] \approx_\alpha 0
%     \end{gather*}
%     \item $\Wcal = \set{\1[\cdot = v] : v \in \supp(\pt)}$:  ``Full'' $(\Hcal,\alpha)$-multicalibration
%     \begin{gather*}
%     \E_{\substack{x \sim \D\\\ys \sim \ps(x,\yhat)}}[h(x) \cdot \1[\pt(x,\yhat) = v] \cdot (\ys - \pt(x,\yhat))] \approx_\alpha 0
%     \end{gather*}
%     for all $v \in \supp(\pt)$.
% \end{itemize}



\subsection{Technical Overview}

\begin{itemize}
    \item Performative Optimality:
    \begin{itemize}
        \item Frame it as agnostic PAC optimality (rather than parameter recovery/optimization)
        \item Challenges of optimality:  the optimal predictor on a set of labels will not be the optimal predictor after deploying the predictor
        \item Retraining known to converge to a stable point
        \item Key insight:  model the prediction as an ``input'' to the predictive model.  Train with the prediction in mind.  (Prediction?  Decision?  Action?)
        \item \mpk{Do we want to highlight the direct RCT / agnostic learning strategy?}
    \end{itemize}
    \item Performative Omniprediction:
    \begin{itemize}
        \item Often when we deploy a prediction system, we don't know exactly what loss we want to minimize.
        \item Ideally, would have a single predictor that could be used, meaningfully, by different clients with different objectives
        \item Concretely, when predictions are performative, it may be useful to have predictions that are equally good at estimating expected outcomes as it is for estimating the success of steering by intervention.
        \item Can we get a single predictor for such a task?
        \item Omniprediction:  developed in the literature on multicalibration.
        \item So a natural starting point for performative omnipredictor would be an analogue of performative multicalibration.
    \end{itemize}
    \item Performative Calibration vs.\ Static Calibration
    \begin{itemize}
        \item Calibration says: expected outcome, given predicted probability $v$ is $v$
        \item But what is the modeled probability under performativity?  It is a function of the choice of \emph{action}.
        \begin{gather*}
            \E_{\ys \sim \ps(x,\yhat)}[\ys \vert \pt(x,\yhat) = v] = v
        \end{gather*}
        \item In other words, even for a binary outcome, calibration becomes a vector-valued set of constraints.  The number of constraints scales \emph{exponentially} in the number of actions!
        \item But do we really care about all of the actions?  Could apply ``decision calibration'' to only focus on optimal decisions, but not obvious it helps. Also, clunky.
    \end{itemize}
    \item Performative Outcome Indistinguishability
    \begin{itemize}
        \item Idea:  develop $\pt$ to mimic $\ps$.  According to relevant tests.
        \item Avoid multicalibration and calibration.  Only focus on loss-based tests, for the predictions relevant to the losses and predictors relevant.
        \item Pro and con:  by explicitly accounting for losses, we can handle ``steering'' losses, in addition to standard convex losses.
    \end{itemize}
\end{itemize}


\clearpage

\paragraph{Outline of results.}
\begin{itemize}
    \item Performative optimality via OI
    \begin{itemize}
        \item \textbf{Def:} Performative OI in terms of a single loss function $\ell$
        \item \textbf{Def:} Decision OI for single loss function $\ell$
        \item \textbf{Thm:} $(\ell,\Hcal,\alpha)$-Performative OI implies $(\ell,\Hcal,\alpha)$-Performative optimality
        \item \textbf{Pf:}  three liner
    \end{itemize}
    \item Performative Omniprediction
    \begin{itemize}
        \item In fact, can get Performative OI and Decision OI for many losses simultaneously
        \item \textbf{Cor:}  Can get Performative Omniprediction for $\cL$ by auditing for each $\ell \in \cL$ explicitly.
    \end{itemize}
    \item Omniprediction for losses that only depend on $\yhat$
    \begin{itemize}
        \item Consider $\cL_1$ the class of all bounded losses that only depend on $x$ through $h(x)$.
        \item \textbf{Def:}  Multiaccuracy
        \item \textbf{Def:}  Decision Calibration
        \item \textbf{Lem:}  $(\Hcal,\alpha)$-Multiaccuracy implies $(\cL_1,\Hcal,2\alpha)$-Performative OI
        \item \textbf{Lem:}  $\alpha$-Decision calibration implies $(\cL_1,\alpha)$-Decision OI
        \item \textbf{Cor:}  $(\Hcal,\alpha)$-MA + $\alpha$-Dec Calibration implies $(\cL_1,\Hcal,3\alpha)$-Performative Omniprediction.
        \item That is, we get a loss-independent approach for omniprediction for all losses.
        \item Note:  can also mix-and-match, e.g., multiaccuracy + $\cL$-decision OI for your favorite $\cL$.
    \end{itemize}
    \item Learning Performative OI predictors:
    \begin{itemize}
        \item Explicit search
        \item Reduction to learning (particularly for multiaccuracy / decision calibration)
        \item Bounded sample complexity!
        \item \textbf{Thm:}  There exists an oracle-efficient, sample-efficient learning algorithm that returns a Performative Omnipredictor.
        \item Open questions about auditing
    \end{itemize}
    \item Universal Adaptability:
    \begin{itemize}
        \item Impossible to get $X$-performativity without modeling the distribution of $X$ explicitly
        \item Short of this, next best thing is that optimality would hold even under covariate shift
        \item \textbf{Cor:}  With the right loss class, you get universal adpaptability too!
        \item Interesting question of how to execute the search reduction to learning effectively.
    \end{itemize}
\end{itemize}








\clearpage
Let $\mathcal{L}_1 = \set{\ell:\Ych \times \set{0,1} \to [-1,1]}$ be the class of all bounded loss functions.



\begin{definition}[Decision OI]
Fix a class of loss functions $\cL$.
A predictor $\pt:\Xcal \times \Ych \to [0,1]$ is $(\cL,\alpha)$-decision outcome indistinguishable if for all $\ell \in \cL$
\begin{gather*}
    \E_{\ys \sim \ps(x,f_\ell(x))}[\ell(f_\ell(x),\ys)] \approx_\alpha \E_{\yt \sim \pt(x,f_\ell(x))}[\ell(f_\ell(x),\yt)].
\end{gather*}
\end{definition}


\begin{definition}[Decision Calibration]
A predictor $\pt:\Xcal \times \Ych \to [0,1]$ is $(\cL,\alpha)$-decision calibrated if for every bounded loss $\ell \in \cL_1$, for all $\yhat \in \Ych$
\begin{gather*}
    \E_{\ys \sim \ps(x,f_\ell(x))}[\ys \vert f_\ell(x) = \yhat] \approx_\alpha \E_{\yt \sim \pt(x,f_\ell(x))}[\yt \vert f_\ell(x) = \yhat]
\end{gather*}
\end{definition}

\mpk{
Note:  decision calibration is equivalent to the following technical condition.

Does there exist a $\yhat \in \Ych, w_0,w_1 \in [-1,1]$ such that:
\begin{gather*}
    \E_x[\pt(x,\yhat) - \ps(x,\yhat) ~\vert~ \argmin_{a \in \Ych}\set{ w_1 \cdot \pt(x,a) + w_0 \cdot (1-\pt(x,a))} = \yhat] > \alpha
\end{gather*}
i.e., does there exist some $\ell \in \cL_1$ and $\yhat \in \Ych$ such that conditioning on the event that $f_\ell(x) = \yhat$ maintains accurate expectations of probabilities.

Note:  this means we can probably run explicit searches over $\poly(1/\alpha)$ many choices of $w_0,w_1$, then compute the minimizers, and evaluate the conditional expectations for $\card{\Ych}$ choices of $\yhat$.

So, auditing is reasonably efficient.  e.g., linear in $\card{\Ych}$, not exponential!

}

\begin{definition}[Multiaccuracy]
Fix a hypothesis class $\Hcal$.
A predictor $\pt:\Xcal \times \Ych \to [0,1]$ is $(\Hcal,\alpha)$-multiaccurate under outcome performativity if for all $h \in \Hcal$
\begin{gather*}
    \E_{\ys \sim \ps(x,h(x))}[\ys \vert h(x) = \yhat] \approx_\alpha \E_{\yt \sim \pt(x,h(x))}[\yt \vert h(x) = \yhat].
\end{gather*}
\end{definition}
\mpk{some sloppiness in approximation here.  Do we want it to be weighted by $\Pr[h(x) = \yhat]$?}

\begin{definition}[Performative OI]
Fix a hypothesis class $\Hcal$.
A predictor $\pt:\Xcal \times \Ych \to [0,1]$ is $(\Hcal,\alpha)$-performative outcome indistinguishable if for all $\ell \in \mathcal{L}_1$ and all $h \in \Hcal$,
\begin{gather*}
    \E_{\yt \sim \pt(x,h(x))}[\ell(h(x),\yt)] \approx_\alpha \E_{\ys \sim \ps(x,h(x))}[\ell(h(x),\ys)].
\end{gather*}
\end{definition}

\begin{lemma}
If $\pt:\Xcal \times \Ych \to [0,1]$ is $(\Hcal,\alpha)$-multiaccurate, then $\pt$ is $(\Hcal,2\alpha)$-performative OI.
\end{lemma}
\begin{proof}
We show an approximate equality between the loss $\ell \in \mathcal{L}_1$ of any $h \in \Hcal$ under $\yt \sim \pt(x,h(x))$ and $\ys \sim \ps(x,h(x))$.
\begin{align*}
\E_{\yt \sim \pt(x,h(x))}[\ell(h(x),\yt)]
&= \sum_{\yhat \in \Ych} \Pr[h(x) = \yhat] \cdot \E_{\yt \sim \pt(x,h(x))}[\ell(\yhat,\yt) ~\vert~ h(x) = \yhat]\\
&= \sum_{\yhat \in \Ych} \Pr[h(x) = \yhat] \cdot \E_{\yt \sim \pt(x,h(x))}\left[\yt \cdot \ell(\yhat,1) + (1-\yt) \cdot \ell(\yhat,0) ~\vert~ h(x) = \yhat\right]\\
&\approx_{2\alpha} \sum_{\yhat \in \Ych} \Pr[h(x) = \yhat] \cdot \E_{\ys \sim \ps(x,h(x))}\left[\ys \cdot \ell(\yhat,1) + (1-\ys) \cdot \ell(\yhat,0) ~\vert~ h(x) = \yhat\right]\\
&= \sum_{\yhat \in \Ych} \Pr[h(x) = \yhat] \cdot \E_{\ys \sim \ps(x,h(x))}[\ell(\yhat,\ys) ~\vert~ h(x) = \yhat]\\
&=\E_{\ys \sim \ps(x,h(x))}[\ell(h(x),\ys)]
\end{align*}
The approximate equality follows under the assumption that $\pt$ is $(\Hcal,\alpha)$-multiaccurate and the bound on the magnitude of $\card{\ell(\yhat,b)} \le 1$ for all $\yhat \in \Ych$ and $b \in \set{0,1}$.
\end{proof}


% \begin{proposition}
% Suppose $\Hcal$ is a class of boolean functions.
% If $\pt:\Xcal \to [0,1]$ is $\C$-multiaccurate and calibrated, then for \emph{any} loss $\ell$, the optimal post-processing $f_\ell$ is an $(\ell,\C)$-agnostic learner.
% \end{proposition}
% \begin{proof}
% Fix a loss $\ell$.
% For a given performative probability $q:\Ych \to [0,1]$, we define $\tilde{\ell}(q)$ to be the optimal loss achievable to predict $y \sim q$.
% \begin{align*}
% \tilde{\ell}(q)
% &= \min_{\yhat}\set{q(\yhat)\cdot \ell(\yhat,1) + (1-q(\yhat)) \cdot \ell(\yhat,0)}
% \end{align*}
% First, we consider the loss experienced by $f_\ell$.
% \begin{align*}
% \E_{\ys \sim \ps(x,f_\ell(x))}[\ell(f_\ell(x),\ys)]
% &= \E_{\yt \sim \ps(x,f_\ell(x))}[\ell(f_\ell(x),\yt)]
% \end{align*}
% by Decision OI.
% Then,
% \begin{align*}
% &= \sum_{\yhat} \Pr[f_\ell(x) = \yhat] \cdot \sum_{v} \Pr[\pt(x,\yhat) = v \vert f_\ell(x) = \yhat] \cdot \E_{\yt \sim \pt(x,\yhat)}[\ell(\yhat,\yt) \vert \pt(x,\yhat) = v, f_\ell(x) = \yhat]\\
% &= \sum_{\yhat} \Pr[f_\ell(x) = \yhat] \cdot \sum_{v} \Pr[\pt(x,\yhat) = v \vert f_\ell(x) = \yhat] \cdot \left(v\cdot \ell(\yhat,1) + (1-v) \cdot \ell(\yhat,0)\right)
% \end{align*}
% where the final equality follows by the definition of $f_\ell$ and the assumption that $\pt$ is calibrated.
% Expanding $\tilde{\ell}(v)$, we upper bound the loss of $f_\ell \circ \pt$ by the loss of any $c \in \C$ as follows.
% \begin{align*}
% % \sum_{v} \Pr[\pt(x) = v] \cdot \tilde{\ell}(v)
% &=  \sum_{v} \Pr[\pt(x) = v] \cdot \min_{a_v}\set{v \cdot \ell(a_v,1) + (1-v) \cdot \ell(a_v,0)}\\
% &\le \sum_{b \in \set{0,1}} \Pr[c(x) = b] \cdot \sum_{v} \Pr[\pt(x) = v \vert c(x) = b] \cdot \min_{a_v}\set{v \cdot \ell(a_v,1) + (1-v) \cdot \ell(a_v,0)}\\
% &\le \sum_{b \in \set{0,1}} \Pr[c(x) = b] \cdot \min_{a}\set{\sum_{v}\Pr[\pt(x) = v \vert c(x) = b] \cdot \left(v \cdot \ell(a,1) + (1-v) \cdot \ell(a,0)\right)}\\
% &= \sum_{b \in \set{0,1}} \Pr[c(x) = b] \cdot \min_{a} \set{\Pr[y = 1 \vert c(x) = b] \cdot \ell(a,1) + \Pr[y = 0 \vert c(x) = b] \cdot \ell(a,0)}\\
% &\le \sum_{b \in \set{0,1}} \Pr[c(x) = b] \cdot \E[\ell(b,y) \vert c(x) = b]\\
% &= \E[\ell(c(x),y)]
% \end{align*}
% where (\ref{eq:multiaccurate}) follows by multiaccuracy of $\pt$.  Specifically, under multiaccuracy, we assume for each $b \in \set{0,1}$, we have the following equalities.
% \begin{align*}
% \sum_{v} \Pr[\pt(x) = v \vert c(x) = b] \cdot v
% &= \sum_{v} \Pr[\pt(x) = v \vert c(x) = b] \cdot \E[\pt(x) \vert c(x) = b \land \pt(x) = v]\\
% &= \E[\pt(x) \vert c(x) = b]\\
% &= \E[y \vert c(x) = b]\\
% &= \Pr[y = 1 \vert c(x) = b]
% \end{align*}
% Thus, for any $\ell$, the post-processed predictor $f_\ell$ is an $(\ell,\C)$-agnostic learner.


% \mpk{This summation seems wrong.  When we sum over $\yhat$, it's no longer the expectation we want.  This should hold for each $\yhat$.}
% \begin{align*}
% \sum_{v} \Pr[\pt(x,\yhat) = v] \cdot v
% &= \sum_{\yhat}\sum_{v} \Pr[h(x) = \yhat] \cdot \Pr[\pt(x,\yhat) = v \vert h(x) = \yhat] \cdot v\\
% &= \sum_{\yhat} \Pr[h(x) = \yhat] \cdot  \E_{\ys \sim \ps(x,h(x))}[\ys \vert h(x) = \yhat]\\
% &= \E_{\ys \sim \ps(x,h(x))}[\ys]
% \end{align*}


% \begin{align*}
% \sum_{v} v \cdot \Pr[\pt(x,\yhat) = v \vert h(x) = \yhat]
% &= \E[\pt(x,\yhat) \vert h(x) = \yhat]\\
% &= \E_{\yt \sim \pt(x,h(x))}[\yt \vert h(x) = \yhat]\\
% &= \E_{\ys \sim \ps(x,h(x))}[\ys \vert h(x) = \yhat]
% \end{align*}

% \end{proof}










==> omni.tex <==
\section{Omniprediction}

Having introduced performative outcome indistinguishability, we now move on to discuss how naive post-processing of models which satisfy this condition lead
to decision rules which are optimal for a wide variety of losses.

\begin{definition}[Performative Omnipredictor]
Suppose $\cL$ is a collection of loss functions and $\cH$ is a hypothesis class.
For $\eps \geq 0$, a predictor $\pt:\cX \times \cYh \to \Delta(\cY)$ is an $(\cL,\cH, \eps)$-omnipredictor under performativity if for all $\ell \in \cL$,
\begin{align}
    \E_{\substack{x \sim \cD \\ \ys \sim \ps(x,\ft_{\ell}(x))}}[\ell(x, \ft_{\ell}(x),\ys)] \leq \min_{h \in \cH} \E_{\substack{x \sim \cD \\ \ys \sim \ps(x,h(x))}}[\ell(x, h(x),\ys)] + \eps
\end{align}
\end{definition}

The following theorem is the main result of this section. 
\begin{theorem}
\theoremlabel{thm:omniprediction}
Let $\cL$ be a set of loss functions and $\cH$ a hypothesis class. If $\pt$ is
$(\cL, \cH, \epsilon)$-reflexitvely POI, then $\pt$ is an $(\cL, \cH, 2\epsilon)$-omnipredictor under performativity.
\end{theorem}
\begin{proof}
The proof is straightforward. In fact, we only need one side of the POI  inequality:
\begin{align}
\E_{\substack{x \sim \D \\ \ys \sim \ps(x,\ft_{\ell}(x))}}[\ell(x, \ft_{\ell}(x),\ys)]
&\le \E_{\substack{x \sim \D\\\yt \sim \pt(x,\ft_{\ell}(x))}} [\ell(x, f_{\ell, \pt}(x),\yt)] +\epsilon \label{ineq:calibration}\\
&\le \E_{\substack{x \sim \D\\\yt \sim \pt(x,h(x))}}[\ell(x, h(x),\yt)] + \epsilon \label{ineq:def:fell}\\
&\le \E_{\substack{x \sim \D\\\ys \sim \ps(x,h(x))}}[\ell(x, h(x),\ys)] + 2\epsilon \label{ineq:multiaccuracy}.
\end{align}
Here, (\ref{ineq:calibration}) follows by the definition of POI; (\ref{ineq:def:fell}) follows by the definition of $f_{\ell, \pt}$ as the (pointwise) minimizer of the expected loss of outcomes sampled as $\yt \sim \pt(x,\yhat)$; and (\ref{ineq:multiaccuracy}) again follows by the reflexive POI guarantee.
\end{proof}

We can in fact strengthen this past result. A predictor that is reflexively-POI for a class $\cL$ is an omnipredictor not just for the functions in $\cL$, it is also an omnipredictor for any linear combination of functions in $\cL$. 
This follows from the fact that the POI definition is closed under linear combinations of loss functions. More formally,
\begin{lemma}
\lemmalabel{lemma:linear combinations}
Let $\beta > 0$ be some positive constant and $\cL$ be a collection of loss functions. Now define, 
\begin{align*}
	\mathsf{Lin}(\cL, \beta) \defeq \left\{\sum_{i=1}^k \lambda_i \ell_i : \sum_i |\lambda_i| \leq \beta, \; \ell_i \in \cL \right\}.
\end{align*}
If $\pt$ is $(\cL,\cH,\eps)$-POI, then it is also $(\mathsf{Lin}(\cL, \beta),\cH,\beta \eps)$-POI. 
\end{lemma}

\begin{proof}
Using the triangle inequality and the definition of loss calibration,
\begin{align*}
\card{\E_{\substack{x \sim \D\\\yt \sim \pt(x,h(x))}}\sum_i \lambda_i\ell_i(x,h(x),\yt) - \E_{\substack{x \sim \D\\\ys \sim \ps(x,h(x))}} \sum_{i} \lambda_i \ell_i(x, h(x),\ys)} 
\end{align*}
is upper bounded by,
\begin{align*}
\sum_i |\lambda_i |\cdot  \card{\E_{\substack{x \sim \D\\\yt \sim \pt(x,h(x))}}[\ell_i(x,h(x),\yt)] - \E_{\substack{x \sim \D\\\ys \sim \ps(x,h(x))}} [\ell_i(x, h(x),\ys)]} \leq \sum |\lambda_i| \epsilon \leq \beta \epsilon.
\end{align*}
\end{proof}

This observation is particularly relevant in the context of omniprediction. 
It shows how given a predictor $\pt$ which is $(\cL, \cH, \epsilon)$-reflexively POI for a small number of ``basis'' functions $\cL$, we get an omniprediction guarantee with regards to a much richer class of function formed via linear combinations of functions $\cL$. 
We make this formal via the following corollary:


\begin{corollary}
A predictor $\pt$ which is a $(\cL, \cH, \epsilon)$-reflexively POI is a $(\mathsf{Lin}(\cL, \beta), \cH, \beta \epsilon)$-omnipredictor  under performativity.  
\end{corollary}

We illustrate the value of this closure property via following example.
\begin{example}
Assume that both predictions and outcomes are binary, $\cYh = \cY = \{\pm 1\}$. If $\pt$ is performatively outcome indistinguishable for 
\begin{align*}
	\ell_1(\yhat, y) = \yhat, \quad \ell_2(\yhat, y) = y,\quad \ell_3(\yhat, y) = \yhat \cdot y, 
\end{align*}
then it is also performatively outcome indistinguishable for any norm bounded polynomial in these variables. In particular, if $\pt$ is $(\cL_b, \cH, \epsilon)$-reflexively POI for $\cL_b= \{\ell_1, \ell_2, \ell_3\}$, then it is a $(\cL_{\mathrm{poly}}, \cH, 2\epsilon)-$ omnipredictor for the set of losses:
\begin{align*}
	\cL_{\mathrm{poly}} = \left\{ \sum_{j,k=1}^\infty a_{j,k} (\yhat)^j (y)^k: \sum_{j,k} |a_{j,k}| \leq 1 \right\}.
\end{align*}
\end{example}





==> predict_then_optimize.tex <==





==> prelims.tex <==


%\section{Outcome Performativity}
%\label{sec:prelims}
%
%\paragraph{Outcome Performativity} Throughout our presentation, we will assume that features $x \in \calX$ are static and distributed according to some distribution $\calD$. Distributions are \emph{outcome} performative, and follows the data generating process:
%
%\begin{enumerate}
%	\item Sample $x \sim \calD$
%	\item Having observed $x$, declare prediction $\yhat \in \calYhat$
%	\item Sample $y \sim \ps(x, \yhat)$, where $\ps$ is conditional distribution of $y \in \calY$, given $x$ and $\yhat$.
%\end{enumerate}
%
%Outcome performativity can be described by the following causal graph:
%\begin{center}
%\begin{tikzpicture}[scale=0.2]
%\tikzstyle{every node}+=[inner sep=0pt]
%\draw [black] (30.7,-27.5) circle (3);
%\draw (30.7,-27.5) node {$\cX$};
%\draw [black] (38.7,-18.7) circle (3);
%\draw (38.7,-18.7) node {$\cYh$};
%\draw [black] (46.2,-27.5) circle (3);
%\draw (46.2,-27.5) node {$\cY$};
%\draw [black] (32.72,-25.28) -- (36.68,-20.92);
%\fill [black] (36.68,-20.92) -- (35.77,-21.18) -- (36.51,-21.85);
%\draw [black] (33.7,-27.5) -- (43.2,-27.5);
%\fill [black] (43.2,-27.5) -- (42.4,-27) -- (42.4,-28);
%\draw [black] (40.6,-21.3) -- (44.19,-25.27);
%\fill [black] (44.19,-25.27) -- (44.02,-24.34) -- (43.28,-25.02);
%\end{tikzpicture}
%\end{center}

 
 
 

==> search.tex <==

\begin{figure}[t]
\setlength{\fboxsep}{2mm}
\begin{boxedminipage}{\textwidth}
\begin{center}
\underline{$\mathrm{Audit}(\cH, \cL, \alpha)$}
\end{center}
\vspace{2mm}
\textbf{If:} there exists $h \in \cH$ and $\ell \in \cL$ such that
	\begin{align*}
		\card{     \E_{\substack{x \sim \cD \\ \yt \sim \pt(x,h(x))}}[\ell(x, h(x),\yt)] - \E_{\substack{x \sim \cD \\ \ys \sim \ps(x,h(x))}}[\ell(x, h(x),\ys)]} \geq \alpha
	\end{align*}
\textbf{Then:} return  $h,l$  \\

\textbf{Else:} return $\mathsf{False} $
\end{boxedminipage}
\caption{The key step in the loss calibration procedure.}
\figurelabel{fig:search_template}
\end{figure}

\section{A Closer Look at Auditing}
\sectionlabel{sec:search}
The Indistinguishability Boosting algorithm is oracle-efficient. 
That is, it is guaranteed to work assuming there exists a statistically and computationally efficient algorithm for solving the auditing step defined in \equationref{eq:constraint}. 
Recall, the goal of the auditing problem is to 
determine whether there exists $h \in \cH$ and $\ell \in \cL$ such that the difference between nature's performative risk and the learner's performative risk under $\pt$ is large:
	\begin{align*}
		\card{     \E_{\substack{x \sim \cD \\ \yt \sim \pt(x,h(x))}}[\ell(x, h(x),\yt)] - \E_{\substack{x \sim \cD \\ \ys \sim \ps(x,h(x))}}[\ell(x, h(x),\ys)]} \geq \alpha.
	\end{align*}
So far, we've established how this problem can be naively solved by simply enumerating over all $h, \ell$ and non-adaptively computing their empirical risks on a single dataset of size $n \geq \mathcal{O}(\lmax |\cYh| \log(|\cH| |\cL| / \delta)\;/\; \alpha^2)$ at each iteration. However, this algorithm runs in time linear in $|\cH| |\cL|$ which may be prohibitively expensive for reasonable hypothesis classes.

In this section, we pay closer attention to the intricacies of implementing this auditing step and establish connections between this question and well-studied learning primitives. 

\subsection{Auditing via Cost-Sensitive Classification}

\jcpnote{The punchline is a reduction to cost sensitive learning which runs in time $|\cL| \cdot \mathrm{Time}(CSL)$}
To do so, we start by defining a generalization of this auditing problem. Let $\cH \subseteq \cX \rightarrow [k]$ be a hypothesis class and let $\cD$ be a distribution over $\cX \times [-1,1]^k$. If $(x,c) \sim \cD$ we refer to $c$ as the cost-vector where $c(j)$ is the $j$-entry of $c$.  


\begin{definition}(weak, agnostic cost-sensitive learning)
An algorithm $\cA$ is a $(\alpha, \gamma)$-??? if for any distribution $\cD$ over $\cX \times [-1,1]$, whenever it is promised that there is an $h \in \cH$ such that $\E c(h(x)) \geq \alpha$, $\cA$ returns a function $g: \cX \rightarrow [k]$ such that $\E c(h(x)) \geq \gamma$. 
\end{definition}

\begin{enumerate}
	\item this is weaker than cost sensitive classification
	\item cost sensitive classification is a well studied problem
	\item both in the theory (cite the MSR papers) and in practice vowpall wabbit
	\item In the binary case $\cYh = \{\pm 1\}$, this reduces to weak agnostic learning as defined in Michael's thesis. 
\end{enumerate} 

\subsection{Auditing via Weak Agnostic Learning}

\jcpnote{this isn't quite great either, you still end up running in time $\cH, \cL \cdot \mathrm{WeakLearn}(\cW)$ }




%\begin{figure}[t]
%\setlength{\fboxsep}{2mm}
%\begin{boxedminipage}{\textwidth}
%$$\underline{\mathrm{LinearSearch}(\cH, \cL, \alpha, n)}$$
%Collect dataset $S = \{(x, \yhat, \ys, \yt)_i\}_{i=1}^n$ of $n$ samples drawn i.i.d according to:
%$$x \sim \D,\; \yhat \sim \unif(\cYh),\; \ys \sim \ps(x,\yhat),\; \yt \sim \pt(x, \yhat)$$
%\textbf{For:} $(h,l) \in \cH' \times \cL$ where $\cH' = \cH \cup \{f_{\ell, p^{(t)}}: \ell \in \cL \}$
%\begin{itemize}
%	\item Compute empirical means:
%	\begin{align*}
%		\widetilde{\PR}(h,l) = \frac{|\cYh|}{n} \sum_{(x,\yhat, \yt) \in S} \ell(x, \yhat, \yt) \ind\{h(x) = \yt\}, \quad 
%		\hat{\PR}(h,l) = \frac{|\cYh|}{n} \sum_{(x,\yhat, \ys) \in S} \ell(x, \yhat, \ys) \ind\{h(x) = \ys\}
%	\end{align*}
%	\item \textbf{If: } $|\widetilde{\PR}(h,l) - \hat{\PR}(h,l)| \geq \alpha$ 
%	\textbf{Then: } return $h,l$\\
%\end{itemize}
%	
%Return $\mathsf{False} $
%\end{boxedminipage}
%\caption{Baseline implementation of the search step}
%\figurelabel{fig:linear_search}
%\end{figure}



